Satellite Based Positioning Signal Acquisition at Higher Order Cycle Frequency

The acquisition of the signal from the satellite based positioning systems, such as GPS, Galileo, and Compass, encounters challenges in the urban streets, indoor. For improving the acquisition performance, the data accumulation is usually performed to improve the signal-to-noise ratio which is defined on the second order statistics. Different from the conventional approaches, the acquisition based on higher order cyclostatistics is proposed. Using the cyclostatistics, the estimation of the initial phase and Doppler shift of the signal is presented respectively. Afterwards, a joint estimator is introduced. The analysis in this paper is performed on GPS signal. Indeed, the proposed estimation method can be straightforwardly extended to acquire the signal from the other satellite positioning systems. The simulation and experiment results demonstrate that the proposed signal acquisition scheme achieves the detection probability of 0.9 at the CNR 28dBHz.

==> Background_Rayleigh.tex <==
\section{Background of Rayleigh Channel Generation}
\label{sec:background}

As a well known model, Rayleigh fading is used to describe the radio environment in which many objects scatter the signal before it arrives at the receiver. Furthermore, there is no light-of-sight component in Rayleigh fading. Due to the central limit theorem, the amplitude of the large amount of scattered signals is Gaussian distributed. The envelope of the two Gaussian variables $r_R^I$ and $r_R^Q$ is Rayleigh distributed. Therefore, to simulate a fading environment with Rayleigh fading, we need to generate two Gaussian variables first. 

%The envelope of two Gaussian variables is Rayleigh distributed. Let $r_R^I$ and $r_R^Q$ denote the variables which capture the statistical feature of the received signals at the In-phase and Quadrature channels of the receiver respectively.

In the scenario that the scattered signals arrive at the receiver at uniformly distributed incidence angles, $r_R^I$ and $r_R^Q$ are generated by (\ref{eq:Rayleigh fading chan gen-Q})~\cite{Jake1974},
%%%%%%%%%%%%%%%%%%%%%%%
\begin{equation}
\left\{
\begin{aligned}
r_{R}^{I}(t)&=\frac{1}{P}\sum_{p=1}^P\cos(2\pi f_{M}(cos(\alpha_p))t+\phi_p),\\
%\label{eq:Rayleigh fading chan gen-I} 
r_{R}^{Q}(t)&=\frac{1}{P}\sum_{p=1}^P\sin(2\pi f_{M}(cos(\alpha_p))t+\phi_p)
\end{aligned}
\right.,
\label{eq:Rayleigh fading chan gen-Q}
\end{equation}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
where $\alpha_p$ represents the incidence angle of the \textit{p}-th of the $P$ paths in the scattering environment, $\phi_p$ is the initial phase of the \textit{p}-th sinusoid which is uniformly distributed in the range $[0,\pi]$, and $f_M$ denotes the maximum Doppler
value. The square root of $r_{R}^{I}(t)$ and $r_{R}^{Q}(t)$ is the Rayleigh distributed variable with a \enquote{U} shape spectrum. 

%\begin{equation}
%r_R(t)=\sqrt{{[r_{R}^{I}(t)]}^2+{[r_{R}^{Q}(t)]}^2}.
%\label{eq:Rayleigh fading chan gen-square root}
%\end{equation}

As mentioned in last section, to obtain the Rayleigh channel via (\ref{eq:Rayleigh fading chan gen-Q}) , multiple lookup tables are needed to generate the $2\times P$ sinusoids~\cite{Alimohammad2006, Alimohammad2007, Ren2010}. Clearly, to ensure accuracy of the generated channel, large lookup tables and consequently large memories are required.  




==> README <==

March 5, 2007


IEEEtran is the official LaTeX class for authors of the Institute of
Electrical and Electronics Engineers (IEEE) transactions journals and
conferences. The latest version of the IEEEtran package can be found
at CTAN:

http://www.ctan.org/tex-archive/macros/latex/contrib/IEEEtran/

as well as within IEEE's site:

http://www.ieee.org/

For latest news, helpful tips, answers to frequently asked questions,
beta releases and other support, visit the IEEEtran home page at my
website:

http://www.michaelshell.org/tex/ieeetran/


Version 1.7a is a bug fix release that corrects the two column peer
review title page problem. This problem was not present in the 1.6 series.


V1.7 is a significant update over the 1.6 series with many important
changes. For a full list, please read the file changelog.txt. The most
notable changes include:

 1. New class option compsoc to support the IEEE Computer Society format.

 2. Several commands and environments have been deprecated in favor of
    replacements with IEEE prefixes to better avoid potential future name
    clashes with other packages. Legacy code retained to allow the use of
    the obsolete forms (for now), but with a warning message to the console
    during compilation:
    \IEEEauthorblockA, \IEEEauthorblockN, \IEEEauthorrefmark,
    \IEEEbiography, \IEEEbiographynophoto, \IEEEkeywords, \IEEEPARstart,
    \IEEEproof, \IEEEpubid, \IEEEpubidadjcol, \IEEEQED, \IEEEQEDclosed,
    \IEEEQEDopen, \IEEEspecialpapernotice. IEEEtran.cls now redefines
    \proof in way to avoid problems with the amsthm.sty package.
    For IED lists:
    \IEEEiedlabeljustifyc, \IEEEiedlabeljustifyl, \IEEEiedlabeljustifyr,
    \IEEEnocalcleftmargin, \IEEElabelindent, \IEEEsetlabelwidth,
    \IEEEusemathlabelsep
    These commands/lengths now require the IEEE prefix and do not have
    legacy support: \IEEEnormaljot.
    For IED lists: \ifIEEEnocalcleftmargin, \ifIEEEnolabelindentfactor,
    \IEEEiedlistdecl, \IEEElabelindentfactor

 3. New \CLASSINPUT, \CLASSOPTION and \CLASSINFO interface allows for more
    user control and conditional compilation.

 4. Several bug fixes and improved compatibility with other packages.


A note to those who create classes derived from IEEEtran.cls: Consider the
use of patch code, either in an example .tex file or as a .sty file,
rather than creating a new class. The IEEEtran.cls CLASSINPUT interface
allows IEEEtran.cls to be fully programmable with respect to document
margins, so there is no need for new class files just for altered margins.
In this way, authors can benefit from updates to IEEEtran.cls and the need
to maintain derivative classes and backport later IEEEtran.cls revisions
thereto is avoided. As always, developers who create classes derived from
IEEEtran.cls should use a different name for the derived class, so that it
cannot be confused with the official/base version here, as well as provide
authors with technical support for the derived class. It is generally a bad
idea to produce a new class that is not going to be maintained.


Best wishes for all your publication endeavors,

Michael Shell
http://www.michaelshell.org/


********************************** Files **********************************

README                 - This file.

IEEEtran.cls           - The IEEEtran LaTeX class file.

changelog.txt          - The revision history.

IEEEtran_HOWTO.pdf     - The IEEEtran LaTeX class user manual.

bare_conf.tex          - A bare bones starter file for conference papers.

bare_jrnl.tex          - A bare bones starter file for journal papers.

bare_jrnl_compsoc.tex  - A bare bones starter file for Computer Society
                         journal papers.

bare_adv.tex           - A bare bones starter file showing advanced
                         techniques such as conditional compilation,
                         hyperlinks, PDF thumbnails, etc. The illustrated
                         format is for a Computer Society journal paper.

***************************************************************************
Legal Notice:
This code is offered as-is without any warranty either expressed or
implied; without even the implied warranty of MERCHANTABILITY or
FITNESS FOR A PARTICULAR PURPOSE! 
User assumes all risk.
In no event shall IEEE or any contributor to this code be liable for
any damages or losses, including, but not limited to, incidental,
consequential, or any other damages, resulting from the use or misuse
of any information contained here.

All comments are the opinions of their respective authors and are not
necessarily endorsed by the IEEE.

This work is distributed under the LaTeX Project Public License (LPPL)
( http://www.latex-project.org/ ) version 1.3, and may be freely used,
distributed and modified. A copy of the LPPL, version 1.3, is included
in the base LaTeX documentation of all distributions of LaTeX released
2003/12/01 or later.
Retain all contribution notices and credits.
** Modified files should be clearly indicated as such, including  **
** renaming them and changing author support contact information. **

File list of work: IEEEtran.cls, IEEEtran_HOWTO.pdf, bare_adv.tex,
                   bare_conf.tex, bare_jrnl.tex, bare_jrnl_compsoc.tex
***************************************************************************


==> abstract.tex <==
\begin{abstract}

The cyclcostationary feature of the GPS signal is investigated in the acquisition in the severely fading environment.. The estimation schemes for the initial code phase and the Doppler shift is proposed. The scheme is built on the cyclostatistics of GPS signals. The simulation and experiment results demonstrate that the GPS signal acquisition scheme achieves the detection probability of 0.9 at the CNR 28dBHz.

\end{abstract}
%\thanks{This material is based upon work supported by the National Science Foundation under Grant Nos. 0958436, 1040429, and 1150215.}
%\let\thefootnote\relax\footnotetext{This material is based upon work supported by the National Science Foundation under Grant Nos. 0958436, 1040429, and 1150215.}


==> conclusion.tex <==
\section{Conclusion}
\label{sec:conclusion}
An efficient fading channel generator is proposed, which is based on the stable recursive computation structure and the time division usage on the structure. The dynamic feature of the data generation equation is analyzed which assists us to design the stable recursive structure. Simulation results demonstrate the advantages of the proposed generator in saving hardware sources.


%Section~\ref{sec:iterative_str_based_Rayleigh_gen} presents the structure for iteratively providing the sinusoids data. To save the hardware resource, we propose a novel structure which implementing the rotation based on bit shifting. However, as a computer based on the hardware platform, errors is inevitable due to the finite resolution or the change of environment. Indeed, the iterative structure is sensitive to the computation. To avoid the exaggerating the error, we propose a improved iterative structure which enables diminishing computation error in the iteration. The investigation in this improved structure has been presented in the previous two subsection. Fig.~\ref{fig: novel rotation str.} illustrates the block diagram of this novel structure.


==> csquotes.def.tex <==
% $Id: csquotes.def,v 5.1d 2011/10/22 19:17:39 lehman stable $

\ProvidesFile{csquotes.def}
[\csq@rcsid $Id: csquotes.def,v 5.1d 2011/10/22 19:17:39 lehman stable $
 csquotes generic definitions]

% Set defaults

\ExecuteQuoteOptions{autostyle=tryonce,autopunct,maxlevel=2,threshold=3,thresholdtype=lines}
\SetBlockEnvironment{quote}
\SetCiteCommand{\cite}

% Predefined backend styles

\DeclareQuoteStyle[quotes]{croatian}% verified
  {\quotedblbase}
  {\textquotedblright}
  [0.05em]% unsure
  {\quotesinglbase}
  {\textquoteright}
\DeclareQuoteStyle[guillemets]{croatian}% verified
  {\guillemotright}
  {\guillemotleft}
  [0.025em]
  {\quotesinglbase}
  {\textquoteright}
\DeclareQuoteStyle[guillemets*]{croatian}% verified
  {\guillemotleft}
  {\guillemotright}
  [0.025em]
  {\quotesinglbase}
  {\textquoteright}
\DeclareQuoteStyle[quotes]{danish}
  {\quotedblbase}
  {\textquotedblleft}
  [0.05em]
  {\textquoteright}% unsure
  {\textquoteright}% unsure
\DeclareQuoteStyle[guillemets]{danish}
  {\guillemotright}
  {\guillemotleft}
  {\textquoteright}% unsure
  {\textquoteright}% unsure
\DeclareQuoteStyle{dutch}
  {\quotedblbase}
  {\textquotedblright}
  [0.05em]
  {\quotesinglbase}% unsure
  {\textquoteright}% unsure
\DeclareQuoteStyle[american]{english}% verified
  {\textquotedblleft}
  {\textquotedblright}
  [0.05em]
  {\textquoteleft}
  {\textquoteright}
\DeclareQuoteStyle[british]{english}% verified
  {\textquoteleft}
  {\textquoteright}
  [0.05em]
  {\textquotedblleft}
  {\textquotedblright}
\DeclareQuoteStyle{finnish}% verified
  {\textquotedblright}
  {\textquotedblright}
  [0.05em]
  {\textquoteright}
  {\textquoteright}
\DeclareQuoteStyle[quotes]{french}
  {\mkfrenchopenquote{\guillemotleft}}
  {\mkfrenchclosequote{\guillemotright}}
  {\textquotedblleft}
  {\textquotedblright}
\DeclareQuoteStyle[quotes*]{french}
  {\mkfrenchopenquote{\guillemotleft}}
  {\mkfrenchclosequote{\guillemotright}}
  {\mkfrenchopenquote{\textquotedblleft}}
  {\mkfrenchclosequote{\textquotedblright}}
\DeclareQuoteStyle[guillemets]{french}
  [\initfrenchquotes]
  {\mkfrenchopenquote{\guillemotleft}}
  [\mkfrenchopenquote{\guillemotleft}]
  {\mkfrenchclosequote{\guillemotright}}
  {\mkfrenchopenquote{\guillemotleft}}
  [\mkfrenchopenquote{\guillemotleft}]
  {\mkfrenchclosequote{\guillemotright}}
\DeclareQuoteStyle[guillemets*]{french}
  [\initfrenchquotes]
  {\mkfrenchopenquote{\guillemotleft}}
  [\mkfrenchopenquote{\guillemotright}]
  {\mkfrenchclosequote{\guillemotright}}
  {\mkfrenchopenquote{\guillemotleft}}
  [\mkfrenchopenquote{\guillemotright}]
  {\mkfrenchclosequote{\guillemotright}}
\DeclareQuoteStyle[quotes]{german}% verified
  {\quotedblbase}
  {\textquotedblleft}
  [0.05em]
  {\quotesinglbase}
  {\fixligatures\textquoteleft}
\DeclareQuoteStyle[guillemets]{german}% verified
  {\guillemotright}
  {\guillemotleft}
  [0.025em]
  {\guilsinglright}
  {\guilsinglleft}
\DeclareQuoteStyle[swiss]{german}% verified
  {\guillemotleft}
  {\guillemotright}
  [0.025em]
  {\guilsinglleft}
  {\guilsinglright}
\DeclareQuoteStyle{greek}% verified
  {\guillemotleft}
  {\guillemotright}
  {\textquotedblleft} 
  {\textquotedblright}
\DeclareQuoteStyle[quotes]{italian}
  {\textquotedblleft}
  {\textquotedblright}
  [0.05em]
  {\textquoteleft}
  {\textquoteright}
\DeclareQuoteStyle[guillemets]{italian}
  {\guillemotleft}
  {\guillemotright}
  [0.025em]
  {\textquotedblleft}
  {\textquotedblright}
\DeclareQuoteStyle[guillemets]{norwegian}
  {\guillemotleft}
  {\guillemotright}
  [0.025em]
  {\guilsinglleft}
  {\guilsinglright}
\DeclareQuoteStyle[quotes]{norwegian}
  {\quotedblbase}
  {\textquotedblright}
  [0.05em]
  {\quotesinglbase}
  {\textquoteright}
\DeclareQuoteStyle[brazilian]{portuguese}% verified
  {\textquotedblleft}
  {\textquotedblright}
  [0.05em]
  {\textquoteleft}
  {\textquoteright}
\DeclareQuoteStyle[portuguese]{portuguese}% unsure
  {\guillemotleft}
  {\guillemotright}
  [0.05em]
  {\textquotedblleft}
  {\textquotedblright}
\DeclareQuoteStyle{russian}% verified
  {\guillemotleft}
  {\guillemotright}
  {\quotedblbase}
  {\textquotedblleft}
\DeclareQuoteStyle[mexican]{spanish}
  {\textquotedblleft}
  {\textquotedblright}
  [0.05em]
  {\textquoteleft}
  {\textquoteright}
\DeclareQuoteStyle[spanish]{spanish}% verified
  {\guillemotleft}
  [\guillemotright]
  {\guillemotright}
  [0.025em]
  {\textquotedblleft}
  [\textquotedblright]
  {\textquotedblright}
\DeclareQuoteStyle[quotes]{swedish}% verified
  {\textquotedblright}
  {\textquotedblright}
  [0.05em]
  {\textquoteright}
  {\textquoteright}
\DeclareQuoteStyle[guillemets]{swedish}% verified
  {\guillemotright}
  {\guillemotright}
  [0.025em]
  {\guilsinglright}
  {\guilsinglright}
\DeclareQuoteStyle[guillemets*]{swedish}% verified
  {\guillemotright}
  {\guillemotleft}
  [0.025em]
  {\guilsinglright}
  {\guilsinglleft}

% Plain style for PDF strings

\DeclarePlainStyle{"}{"}{'}{'}

% Default style

\DeclareQuoteAlias[american]{english}{default}

% Predefined aliases

\DeclareQuoteAlias[quotes]{croatian}{croatian}
\DeclareQuoteAlias[quotes]{danish}{danish}
\DeclareQuoteAlias[american]{english}{american}
\DeclareQuoteAlias[american]{english}{canadian}
\DeclareQuoteAlias[american]{english}{english}
\DeclareQuoteAlias[british]{english}{british}
\DeclareQuoteAlias[british]{english}{australian}% unsure
\DeclareQuoteAlias[british]{english}{newzealand}% unsure
\DeclareQuoteAlias[quotes]{french}{french}
\DeclareQuoteAlias[quotes]{german}{austrian}
\DeclareQuoteAlias[quotes]{german}{german}
\DeclareQuoteAlias[swiss]{german}{swiss}
\DeclareQuoteAlias[guillemets]{italian}{italian}
\DeclareQuoteAlias[guillemets]{norwegian}{norwegian}
\DeclareQuoteAlias[brazilian]{portuguese}{brazilian}
\DeclareQuoteAlias[portuguese]{portuguese}{portuguese}
\DeclareQuoteAlias[mexican]{spanish}{mexican}
\DeclareQuoteAlias[spanish]{spanish}{spanish}
\DeclareQuoteAlias[quotes]{swedish}{swedish}

% Babel aliases

\DeclareQuoteAlias{american}{USenglish}
\DeclareQuoteAlias{american}{usenglish}
\DeclareQuoteAlias{brazilian}{brazil}
\DeclareQuoteAlias{british}{UKenglish}
\DeclareQuoteAlias{british}{ukenglish}
\DeclareQuoteAlias{german}{ngerman}
\DeclareQuoteAlias{austrian}{naustrian}
\DeclareQuoteAlias{norwegian}{norsk}
\DeclareQuoteAlias{norwegian}{nynorsk}
\DeclareQuoteAlias{portuguese}{portuges}

% Language options

\DeclareQuoteOption{danish}
\DeclareQuoteOption{english}
\DeclareQuoteOption{french}
\DeclareQuoteOption{german}
\DeclareQuoteOption{italian}
\DeclareQuoteOption{norwegian}
\DeclareQuoteOption{spanish}
\DeclareQuoteOption{swedish}

% Register quotation marks (per output encoding)

\DeclareQuoteGlyph{OT1}{34}%  = \textquotedblright
\DeclareQuoteGlyph{OT1}{39}%  = \textquoteright
\DeclareQuoteGlyph{OT1}{92}%  = \textquotedblleft
\DeclareQuoteGlyph{OT1}{96}%  = \textquoteleft

\DeclareQuoteGlyph{OT2}{34}%  = \textquotedbl
\DeclareQuoteGlyph{OT2}{39}%  = \textquoteright
\DeclareQuoteGlyph{OT2}{60}%  = \guillemotleft
\DeclareQuoteGlyph{OT2}{62}%  = \guillemotright
\DeclareQuoteGlyph{OT2}{96}%  = \textquoteleft
%\DeclareQuoteGlyph{OT2}{91}% = [[ ligature = \guillemotleft
%\DeclareQuoteGlyph{OT2}{93}% = ]] ligature = \guillemotright

\DeclareQuoteGlyph{OT4}{34}%  = \textquotedblright
\DeclareQuoteGlyph{OT4}{39}%  = \textquoteright
\DeclareQuoteGlyph{OT4}{92}%  = \textquotedblleft
\DeclareQuoteGlyph{OT4}{96}%  = \textquoteleft
\DeclareQuoteGlyph{OT4}{174}% = \guillemotleft
\DeclareQuoteGlyph{OT4}{175}% = \guillemotright
\DeclareQuoteGlyph{OT4}{255}% = \quotedblbase

\DeclareQuoteGlyph{T1}{13}%   = \quotesinglbase
\DeclareQuoteGlyph{T1}{14}%   = \guilsinglleft
\DeclareQuoteGlyph{T1}{15}%   = \guilsinglright
\DeclareQuoteGlyph{T1}{16}%   = \textquotedblleft
\DeclareQuoteGlyph{T1}{17}%   = \textquotedblright
\DeclareQuoteGlyph{T1}{18}%   = \quotedblbase
\DeclareQuoteGlyph{T1}{19}%   = \guillemotleft
\DeclareQuoteGlyph{T1}{20}%   = \guillemotright
\DeclareQuoteGlyph{T1}{34}%   = \textquotedbl
\DeclareQuoteGlyph{T1}{39}%   = \textquoteright
\DeclareQuoteGlyph{T1}{96}%   = \textquoteleft
%\DeclareQuoteGlyph{T1}{60}%  = << ligature = \guillemotleft
%\DeclareQuoteGlyph{T1}{62}%  = >> ligature = \guillemotright

\DeclareQuoteGlyph{LY1}{34}%  = \textquotedbl
\DeclareQuoteGlyph{LY1}{39}%  = \textquoteright
\DeclareQuoteGlyph{LY1}{96}%  = \textquoteleft
\DeclareQuoteGlyph{LY1}{129}% = \textquotesingle
\DeclareQuoteGlyph{LY1}{130}% = \quotesinglbase
\DeclareQuoteGlyph{LY1}{132}% = \quotedblbase
\DeclareQuoteGlyph{LY1}{139}% = \guilsinglleft
\DeclareQuoteGlyph{LY1}{147}% = \textquotedblleft
\DeclareQuoteGlyph{LY1}{148}% = \textquotedblright
\DeclareQuoteGlyph{LY1}{155}% = \guilsinglright
\DeclareQuoteGlyph{LY1}{171}% = \guillemotleft
\DeclareQuoteGlyph{LY1}{187}% = \guillemotright

\DeclareQuoteGlyph{LGR}{28}%  = \textquoteleft
\DeclareQuoteGlyph{LGR}{29}%  = \textquoteright
\DeclareQuoteGlyph{LGR}{123}% = \guillemotleft
\DeclareQuoteGlyph{LGR}{125}% = \guillemotright

\DeclareQuoteGlyph{T2A}{16}%  = \textquotedblleft
\DeclareQuoteGlyph{T2A}{17}%  = \textquotedblright
\DeclareQuoteGlyph{T2A}{34}%  = \textquotedbl
\DeclareQuoteGlyph{T2A}{39}%  = \textquoteright
\DeclareQuoteGlyph{T2A}{96}%  = \textquoteleft
\DeclareQuoteGlyph{T2A}{189}% = \quotedblbase
\DeclareQuoteGlyph{T2A}{190}% = \guillemotleft
\DeclareQuoteGlyph{T2A}{191}% = \guillemotright
%\DeclareQuoteGlyph{T2A}{60}% = << ligature = \guillemotleft
%\DeclareQuoteGlyph{T2A}{62}% = >> ligature = \guillemotright

\DeclareQuoteGlyph{T2B}{16}%  = \textquotedblleft
\DeclareQuoteGlyph{T2B}{17}%  = \textquotedblright
\DeclareQuoteGlyph{T2B}{34}%  = \textquotedbl
\DeclareQuoteGlyph{T2B}{39}%  = \textquoteright
\DeclareQuoteGlyph{T2B}{96}%  = \textquoteleft
\DeclareQuoteGlyph{T2B}{189}% = \quotedblbase
\DeclareQuoteGlyph{T2B}{190}% = \guillemotleft
\DeclareQuoteGlyph{T2B}{191}% = \guillemotright
%\DeclareQuoteGlyph{T2B}{60}% = << ligature = \guillemotleft
%\DeclareQuoteGlyph{T2B}{62}% = >> ligature = \guillemotright

\DeclareQuoteGlyph{T2C}{16}%  = \textquotedblleft
\DeclareQuoteGlyph{T2C}{17}%  = \textquotedblright
\DeclareQuoteGlyph{T2C}{34}%  = \textquotedbl
\DeclareQuoteGlyph{T2C}{39}%  = \textquoteright
\DeclareQuoteGlyph{T2C}{96}%  = \textquoteleft
\DeclareQuoteGlyph{T2C}{189}% = \quotedblbase
\DeclareQuoteGlyph{T2C}{190}% = \guillemotleft
\DeclareQuoteGlyph{T2C}{191}% = \guillemotright
%\DeclareQuoteGlyph{T2C}{60}% = << ligature = \guillemotleft
%\DeclareQuoteGlyph{T2C}{62}% = >> ligature = \guillemotright

\DeclareQuoteGlyph{X2}{16}%   = \textquotedblleft
\DeclareQuoteGlyph{X2}{17}%   = \textquotedblright
\DeclareQuoteGlyph{X2}{34}%   = \textquotedbl
\DeclareQuoteGlyph{X2}{39}%   = \textquoteright
\DeclareQuoteGlyph{X2}{96}%   = \textquoteleft
\DeclareQuoteGlyph{X2}{189}%  = \quotedblbase
\DeclareQuoteGlyph{X2}{190}%  = \guillemotleft
\DeclareQuoteGlyph{X2}{191}%  = \guillemotright
%\DeclareQuoteGlyph{X2}{60}%  = << ligature = \guillemotleft
%\DeclareQuoteGlyph{X2}{62}%  = >> ligature = \guillemotright

\DeclareQuoteGlyph{LCY}{13}%  = \textquotesingle
\DeclareQuoteGlyph{LCY}{34}%  = \textquotedbl
\DeclareQuoteGlyph{LCY}{39}%  = \textquoteright
\DeclareQuoteGlyph{LCY}{96}%  = \textquoteleft
\DeclareQuoteGlyph{LCY}{253}% = \guillemotleft
\DeclareQuoteGlyph{LCY}{254}% = \guillemotright
\DeclareQuoteGlyph{LCY}{255}% = \quotedblbase
%\DeclareQuoteGlyph{LCY}{60}% = << ligature = \guillemotleft
%\DeclareQuoteGlyph{LCY}{62}% = >> ligature = \guillemotright

% Unicode (for XeTeX)
\DeclareQuoteGlyph{EU1}{"0022}% = neutral quot. mark, double              = \textquotedbl
\DeclareQuoteGlyph{EU1}{"0027}% = neutral quot. mark, single              = \textquotesingle
\DeclareQuoteGlyph{EU1}{"00AB}% = angle quot. mark, left-pointing double  = \guillemotleft
\DeclareQuoteGlyph{EU1}{"00BB}% = angle quot. mark, right-pointing double = \guillemotright
\DeclareQuoteGlyph{EU1}{"2018}% = comma quot. mark, single turned         = \textquoteleft
\DeclareQuoteGlyph{EU1}{"2019}% = comma quot. mark, single                = \textquoteright
\DeclareQuoteGlyph{EU1}{"201A}% = comma quot. mark, low single            = \quotesinglbase
\DeclareQuoteGlyph{EU1}{"201B}% = comma quot. mark, single reversed       = n/a
\DeclareQuoteGlyph{EU1}{"201C}% = comma quot. mark, double turned         = \textquotedblleft
\DeclareQuoteGlyph{EU1}{"201D}% = comma quot. mark, double                = \textquotedblright
\DeclareQuoteGlyph{EU1}{"201E}% = comma quot. mark, low double            = \quotedblbase
\DeclareQuoteGlyph{EU1}{"201F}% = comma quot. mark, double reversed       = n/a
\DeclareQuoteGlyph{EU1}{"2039}% = angle quot. mark, left-pointing single  = \guilsinglleft
\DeclareQuoteGlyph{EU1}{"203A}% = angle quot. mark, right-pointing single = \guilsinglright

% Unicode (for LuaTeX)
\DeclareQuoteGlyph{EU2}{"0022}% = neutral quot. mark, double              = \textquotedbl
\DeclareQuoteGlyph{EU2}{"0027}% = neutral quot. mark, single              = \textquotesingle
\DeclareQuoteGlyph{EU2}{"00AB}% = angle quot. mark, left-pointing double  = \guillemotleft
\DeclareQuoteGlyph{EU2}{"00BB}% = angle quot. mark, right-pointing double = \guillemotright
\DeclareQuoteGlyph{EU2}{"2018}% = comma quot. mark, single turned         = \textquoteleft
\DeclareQuoteGlyph{EU2}{"2019}% = comma quot. mark, single                = \textquoteright
\DeclareQuoteGlyph{EU2}{"201A}% = comma quot. mark, low single            = \quotesinglbase
\DeclareQuoteGlyph{EU2}{"201B}% = comma quot. mark, single reversed       = n/a
\DeclareQuoteGlyph{EU2}{"201C}% = comma quot. mark, double turned         = \textquotedblleft
\DeclareQuoteGlyph{EU2}{"201D}% = comma quot. mark, double                = \textquotedblright
\DeclareQuoteGlyph{EU2}{"201E}% = comma quot. mark, low double            = \quotedblbase
\DeclareQuoteGlyph{EU2}{"201F}% = comma quot. mark, double reversed       = n/a
\DeclareQuoteGlyph{EU2}{"2039}% = angle quot. mark, left-pointing single  = \guilsinglleft
\DeclareQuoteGlyph{EU2}{"203A}% = angle quot. mark, right-pointing single = \guilsinglright

\endinput

% Auxiliary commands for some styles

% The \fixligatures command used in the above styles is provided
% by csquotes.sty. It is used as follows:
%
%       \fixligatures\textquoteleft
%
% and will suppress the ligatures
%
%       ?` -> \textquestiondown
% and
%       !` -> \textexclamdown
%
% in T1 encoding.

% \initfrenchquotes is also provided by csquotes.sty. This command
% is intended for use in the 'outer initialization' argument of
% \DeclareQuoteStyle. It will enable a feature which replaces two
% adjoining marks at the end of a quotation by a single one. This is
% required by some styles which use the same quotation marks on both
% the outer and the inner level. If enabled, you get:
%
%        <<outer quote <<inner quote>>
%
% instead of
%
%        <<outer quote <<inner quote>> >>
%
% That is, if two nested quotations end simultaneously, the second
% closing mark is omitted.

% The commands \mkfrenchopenquote and \mkfrenchclosequote are
% intended for spaced-out quotation marks as used in French. They
% are employed as follows:
%
%       \mkfrenchopenquote{\guillemotleft}
%       \mkfrenchclosequote{\guillemotright}
%
% and will use a command called \@frenchquotespace to space out the
% quotation marks. The default spacing is:
%
%       \penalty\@M
%       \hskip 0.8\fontdimen2\font
%        plus  0.3\fontdimen3\font
%        minus 0.3\fontdimen4\font
%
% This is similar to what the \og and \fg commands of babel's
% french.ldf use. It yields a stretchable space whose natural size
% is the interword space of the current font multiplied by 0.8. The
% stretch component is the interword stretch of the current font
% multiplied by 0.3, and the shrink component is the interword
% shrink of the current font multiplied by 0.3.
%
% If you prefer a full interword space, redefine \@frenchquotespace
% as follows:
%
%       \renewcommand*{\@frenchquotespace}{%
%         \penalty\@M
%         \hskip\fontdimen2\font\relax}
%
% or:
%
%       \renewcommand*{\@frenchquotespace}{%
%         \penalty\@M\space}
%
% In either case, the difference to the default values is so subtle,
% you will hardly notice it in most cases.
%
% Don't forget to add the penalty if you redefine \@frenchquotespace!
% You certainly don't want to allow a linebreak at that point.

==> csquotes.sty.tex <==
% $Id: csquotes.sty,v 5.1d 2011/10/22 19:17:39 lehman stable $

% Copyright (c) 2003-2011 Philipp Lehman.
%
% Permission is granted to copy, distribute and/or modify this
% software under the terms of the LaTeX Project Public License
% (LPPL), version 1.3.
%
% The LPPL maintenance status of this software is
% 'author-maintained'.
%
% This software is provided 'as is', without warranty of any kind,
% either expressed or implied, including, but not limited to, the
% implied warranties of merchantability and fitness for a
% particular purpose.

\def\csq@rcsid$#1: #2 #3 #4 #5${#4 v#3}

\NeedsTeXFormat{LaTeX2e}[2005/12/01]
\ProvidesPackage{csquotes}
[\csq@rcsid $Id: csquotes.sty,v 5.1d 2011/10/22 19:17:39 lehman stable $
 context-sensitive quotations]

\def\csq@version$#1: #2.#3 ${#2#3}
\edef\csq@version{\csq@version$Revision: 5.1 $}

%% Compatibility and requirements

\RequirePackage{etoolbox}
\RequirePackage{keyval}

\@ifpackagelater{etoolbox}{2008/06/28}
  {}
  {\PackageError{csquotes}
     {Outdated 'etoolbox' package}
     {Upgrade to etoolbox v1.7 (2008/06/28) or later.\MessageBreak
      I found: '\csuse{ver@etoolbox.sty}'.\MessageBreak
      This is a fatal error. I'm aborting now.}%
   \endinput}

\@ifpackageloaded{inputenc}
  {}
  {\AtEndPreamble{%
     \@ifpackageloaded{inputenc}
       {\csq@warn@loadfirst{inputenc}}
       {}}}

\@ifpackageloaded{inputenx}
  {}
  {\AtEndPreamble{%
     \@ifpackageloaded{inputenx}
       {\csq@warn@loadfirst{inputenx}}
       {}}}

\@ifpackageloaded{ucs}
  {\let\csq@ifucs\@firstoftwo}
  {\let\csq@ifucs\@secondoftwo
   \AtEndPreamble{%
     \@ifpackageloaded{ucs}
       {\let\csq@ifucs\@firstoftwo}
       {}}}

\AtEndPreamble{%
  \@ifpackageloaded{biblatex}
    {\@ifpackagelater{biblatex}{2009/05/30}
       {}
       {\csq@error
          {Outdated 'biblatex' package}
          {Upgrade to biblatex v0.8d (2009/05/30) or later.\MessageBreak
           I found: '\csuse{ver@biblatex.sty}'}}}
    {}}

%% Category codes

\def\csq@catcodes{\do\~\do\&\do\:\do\"\do\<\do\>}
\def\do#1{\catcode\number`#1=\the\catcode`#1\relax}
\edef\csq@catcodes{\csq@catcodes}
\let\do\noexpand

\catcode`\~=\active
\catcode`\&=3
\@makeother\:
\@makeother\"
\@makeother\<
\@makeother\>

%% General

\newtoggle{csq@tempsw}
\newtoggle{csq@quiet}
\newtoggle{csq@active}
\newtoggle{csq@block}
\newtoggle{csq@parbox}
\newtoggle{csq@parthreshold}
\newbool{csdisplay}

\newcount\csq@reset
\newcount\csq@gtype
\newcount\csq@glevel
\newcount\csq@qlevel
\newcount\csq@maxlvl
\newcount\csq@tshold

\providecommand{\@gobblethree}[3]{}
\providecommand{\@gobblefive}[5]{}
\providecommand{\@gobbletwo@optarg}[2][]{}

% {<item>}{<list>}{<separator>}

\def\csq@addto@list#1{%
  \expandafter\csq@addto@list@i\csname\string#1\endcsname}
\def\csq@addto@list@i#1#2#3{%
  \begingroup
  \@tempswatrue
  \def#3##1{\ifnum`#1=`##1\relax\@tempswafalse\fi}#2%
  \expandafter\endgroup\if@tempswa
    \appto#2{#3#1}%
  \fi}

% {<macro>}

\def\csq@everypar#1{%
  \let\csq@theeverypar#1%
  \ifx\csq@theeverypar\@empty
  \else
    \csq@everypar@i
  \fi}

\def\csq@everypar@i{%
  \leavevmode
  \let\csq@new@everypar\everypar
  \csq@ltx@everypar=\expandafter{\the\everypar}%
  \csq@new@everypar={\the\csq@ltx@everypar\csq@theeverypar}%
  \let\everypar\csq@ltx@everypar
  \let\csq@everypar@i\relax}

\newtoks\csq@ltx@everypar

% Miscellaneous tests

\newcommand*{\ifblockquote}{\iftoggle{csq@block}}

\def\csq@ifsafeactives{%
  \ifx\if@safe@actives\iftrue
    \expandafter\@firstoftwo
  \else
    \expandafter\@secondoftwo
  \fi}

\def\csq@iftypeset{%
  \ifx\protect\@typeset@protect
    \expandafter\@firstoftwo
  \else
    \expandafter\@secondoftwo
  \fi}

\def\csq@ifstrings{%
  \ifx\protect\string
    \expandafter\@firstoftwo
  \else
    \expandafter\@secondoftwo
  \fi}

\def\csq@ifnested{%
  \iftoggle{csq@block}
    {\@firstoftwo}
    {\ifnumgreater\csq@qlevel\z@}}

% Parsers for UTF-8

\def\csq@string#1{\csq@string@i#1&}
\def\csq@string@i#1#2&{%
  \string#1\ifblank{#2}{}{\csq@string@i#2&}}

\def\csq@number#1{\csq@number@i#1&}
\def\csq@number@i#1#2&{%
  \number`#1 \ifblank{#2}{}{.\csq@number@i#2&}}

\def\csq@utfprint#1{u8:\csq@utfprint@i#1&}
\def\csq@utfprint@i#1#2&{%
  \number`#1 \ifblank{#2}{}{:\csq@utfprint@i#2&}}

% Grouping control

\protected\def\csq@bqgroup{%
  \bgroup\leavevmode
  \csq@glevel\currentgrouplevel
  \csq@gtype\currentgrouptype}

\protected\def\csq@eqgroup{%
  \ifnum\csq@gtype=\currentgrouptype
    \ifnum\csq@glevel=\currentgrouplevel
    \else
      \csq@err@glevel
    \fi
  \else
    \csq@err@gtype
  \fi
  \egroup}

\AtEndDocument{%
  \ifnum\csq@qlevel>\z@
    \csq@err@gleft
  \fi}

%% User feedback

\protected\def\csq@warning@loose#1{%
  \csq@warning{#1}\@gobbletwo}
\protected\def\csq@warning@strict#1{%
  \csq@error}
\let\csq@warnorerr\csq@warning@loose

\protected\def\csq@error#1#2{%
  \PackageError{csquotes}{#1}{#2.}}

\protected\def\csq@warning#1{%
  \PackageWarning{csquotes}{#1}}

\protected\def\csq@info#1{%
  \iftoggle{csq@quiet}
    {}
    {\PackageInfo{csquotes}{#1\csq@noline}}}
\let\csq@noline\@gobble
\AtBeginDocument{\let\csq@noline\@empty}

\protected\def\csq@logdebug#1{%
  \begingroup
  \def\MessageBreak{^^J(csquotes) \@spaces\@spaces\@spaces\space}%
  \set@display@protect
  \immediate\write\m@ne{Package csquotes Debug: #1\on@line.}%
  \endgroup}

\let\csq@debug\@gobble

% Errors

\protected\def\csq@errormark{%
  \rule[0.25ex]{1.25ex}{1.25ex}}

\protected\def\csq@eqerror{%
  \csq@eqgroup
  \csq@errormark}

\protected\def\csq@mismatch#{%
  \csq@errormark
  \csq@err@mismatch}

\protected\def\csq@err@mismatch#1{%
  \csq@error
    {Unbalanced groups or invalid nesting}
    {#1}}

\protected\def\csq@err@mmode#1{%
  \csq@error
    {'\string#1' invalid in math mode}
    {This command may not be used in math mode}}

\protected\def\csq@err@undef#1{%
  \csq@error
    {'\string#1' not defined}
    {This command or environment environment appears to
     be\MessageBreak undefined}}

\protected\def\csq@err@opt#1{%
  \csq@error
    {Option '#1' invalid}
    {The option you have supplied is invalid. See the csquotes
     manual\MessageBreak for valid option keys and values}}

\protected\def\csq@err@sfcodes#1{%
  \csq@error
    {'\string#1' not available}
    {'\string#1' may not be used here because the\MessageBreak
     punctuation tracker is not working at this point}}

\protected\def\csq@err@glevel{%
  \csq@mismatch{%
    I have detected a group level mismatch. Verify that all
    groups\MessageBreak and all active quotes are properly
    balanced and nested. If you\MessageBreak continue, I
    will write a summary of all previously opened
    groups\MessageBreak to the transcript file}%
  \showgroups}

\protected\def\csq@err@gtype{%
  \csq@mismatch{%
    I have detected a group type mismatch. Verify that all
    groups\MessageBreak and all active quotes are properly
    balanced and nested. If you\MessageBreak continue, I
    will write a summary of all previously opened
    groups\MessageBreak to the transcript file}%
  \showgroups}

\protected\def\csq@err@gleft{%
  \csq@err@mismatch{%
    Still \number\csq@qlevel\space quote\ifnum\csq@qlevel>\@ne s\fi
    \space open. If you continue, I will write a summary\MessageBreak
    of all previously opened groups to the transcript file}%
  \showgroups}

\protected\def\csq@err@alloc{%
  \csq@error
    {Invalid argument}
    {One of the arguments you have supplied is already allocated
     as\MessageBreak active quote or delimiter}}

\protected\def\csq@err@char{%
  \csq@error
    {Invalid argument}
    {Only single characters with category code 12 or 13 may
     be\MessageBreak allocated as active quotes. Numbers,
     punctuation marks, and\MessageBreak characters which
     are part of LaTeX's syntax or reserved\MessageBreak
     for a specific purpose are invalid}}

\protected\def\csq@err@utf{%
  \csq@error
    {Invalid argument}
    {Only valid UTF-8 sequences representing a single
     character\MessageBreak may be allocated as active quotes}}

\protected\def\csq@err@nbquote{%
  \csq@mismatch{%
    You have nested a \@backslashchar blockquote. Block quotation
    commands\MessageBreak may only be used on quotation level 0}}%

\protected\def\csq@err@patch#1{%
  \csq@error
    {Patching #1 failed}
    {This is an internal issue typically caused by a
     conflict\MessageBreak between csquotes and some
     other package. Modifying\MessageBreak the package
     loading order may fix the problem}}

\protected\def\csq@err@ucs{%
  \csq@error
    {ucs package not supported}
    {The ucs package is not supported. If you want to use
     UTF-8\MessageBreak encoded active quotes, try
     '\string\usepackage[utf8]{inputenc}'.\MessageBreak
     If you continue now, I will reject all UTF-8 encoded
     arguments\MessageBreak as invalid}}

% Warnings

\protected\def\csq@warn@loadfirst#1{%
  \csq@warnorerr
    {Load '#1' before 'csquotes'}
    {'#1' package loaded too late}
    {Always load '#1' before 'csquotes'}}

\protected\def\csq@warn@multilang#1{%
  \csq@warnorerr
    {No multilingual support.\MessageBreak #1}
    {#1}
    {Multilingual support does not seem to be available.\MessageBreak
     Try loading the 'babel' or the 'polyglossia' package}}

\protected\def\csq@warn@style#1{%
  \csq@warnorerr
    {No style for language '#1'.\MessageBreak
     Using fallback style}
    {No style for language '#1'}
    {Define a style or alias for this language first}}

\protected\def\csq@warn@location#1{%
  \csq@warnorerr
    {'\string#1' invalid at this point.\MessageBreak
     Ignoring command}
    {'\string#1' invalid at this point}
    {This command may not be used at this particular
     point.\MessageBreak See the manual of the 'csquotes'
     package for details}}

\protected\def\csq@warn@sfcodes#1{%
  \csq@warnorerr
    {No space factor codes for '#1' encoding.\MessageBreak
     Punctuation tracker may fail}
    {Punctuation tracker may fail at this point}
    {No space factor codes for '#1' encoding.
     See \string\DeclareQuoteGlyph\MessageBreak
     in the 'csquotes' manual for details}}

%% Outer quotations

\protected\def\csq@oqmark{%
  \csq@bqgroup
  \ifnum\csq@qlevel>\z@
    \csq@mismatch{%
      Level 1 quote invalid at this point.
      The current level is \number\csq@qlevel}%
    \advance\csq@qlevel\@ne
    \let\csq@oqmark\csq@eqerror
  \else
    \csq@qlevel\@ne
    \let\csq@oqmark\csq@qclose
    \expandafter\csq@qopen
  \fi}

%% Inner quotations

\protected\def\csq@iqmark{%
  \csq@bqgroup
  \ifnum\csq@qlevel>\@ne
    \csq@mismatch{%
      Level 2 quote invalid at this point.
      The current level is \number\csq@qlevel}%
    \advance\csq@qlevel\@ne
    \let\csq@iqmark\csq@eqerror
  \else
    \csq@qlevel\tw@
    \let\csq@iqmark\csq@qclose
    \expandafter\csq@qopen
  \fi}

%% Nestable quotations

\protected\def\csq@oqopen{%
  \csq@bqgroup
  \csq@oqopen@i}

\def\csq@oqopen@i{%
  \advance\csq@qlevel\@ne
  \csq@qopen}

\protected\def\csq@iqopen{%
  \csq@bqgroup
  \csq@iqopen@i}

\def\csq@iqopen@i{%
  \ifnum\csq@qlevel=\z@
    \advance\csq@qlevel\tw@
  \else
    \advance\csq@qlevel\@ne
  \fi
  \csq@qopen}

%% Opening marks

\def\csq@qopen{%
  \ifnum\csq@qlevel>\csq@maxlvl
    \csq@mismatch{%
      Level \number\csq@qlevel\space quote invalid at this point.
      The maximum level is \number\csq@maxlvl}%
  \else
    \csq@resetstyle
    \csq@init
    \csq@addkern@open
    \ifodd\csq@qlevel
      \let\csq@kernchar@i\csq@thequote@oopen
      \csq@thequote@oopen
    \else
      \let\csq@kernchar@i\csq@thequote@iopen
      \csq@thequote@iopen
    \fi
    \csq@setmarker@open
    \expandafter\csq@fixkern
  \fi}

%% Closing marks

\protected\def\csq@qclose{%
  \csq@qclose@i{}}

\def\csq@qclose@i{%
  \ifnum\csq@qlevel=\z@
    \csq@mismatch{%
      Cannot close any quote. The current level is 0}%
  \else
    \ifnum\csq@qlevel>\csq@maxlvl
      \csq@eqerror
    \else
      \expandafter\expandafter
      \expandafter\csq@qclose@ii
    \fi
  \fi}

\def\csq@qclose@ii#1{%
  \ifdim\lastkern=\csq@omitmarker
    #1\csq@eqgroup
  \else
    \csq@addkern@close
    \ifodd\csq@qlevel
      \csq@thequote@oclose
      \let\csq@kernchar@i\csq@thequote@oclose
    \else
      \csq@thequote@iclose
      \let\csq@kernchar@i\csq@thequote@iclose
    \fi
    \ifnum\csq@qlevel>\@ne
      \csq@setmarker@close
    \fi
    \ifblank{#1}{}{\expandafter#1}%
    \expandafter\csq@eqgroup
      \expandafter\def
      \expandafter\csq@kernchar@i
      \expandafter{\csq@kernchar@i}%
    \expandafter\csq@fixkern
  \fi}

%% Style initialization

\def\csq@init{%
  \csq@setsfcodes
  \ifodd\csq@qlevel
    \csq@thequote@oinit
    \csq@everypar\csq@thequote@omiddle
  \else
    \csq@thequote@iinit
    \csq@everypar\csq@thequote@imiddle
  \fi
  \csq@init@kern{open}{o}{i}%
  \csq@init@kern{close}{i}{o}}

\def\csq@init@kern#1#2#3{%
  \begingroup
  \settowidth{\@tempdima}{%
    \csuse{csq@thequote@#2#1}%
    \csuse{csq@thequote@#3#1}}%
  \settowidth{\@tempdimb}{%
    \csuse{csq@thequote@#2#1}\unkern
    \csuse{csq@thequote@#3#1}}%
  \ifdim\@tempdima=\@tempdimb
    \let\csq@tempa\endgroup
  \else
    \edef\csq@tempa{\endgroup
      \csdef{csq@thekern@#1}{%
        \the\dimexpr\@tempdima-\@tempdimb\relax}}%
  \fi
  \csq@tempa}

\def\blx@hook@parboxrestore{%
  \let\csq@theeverypar\@empty
  \csq@qlevel\z@
  \toggletrue{csq@parbox}%
  \togglefalse{csq@block}}

\protected\def\blx@parboxrestore{%
  \ifx\protect\noexpand % \@outputpage
  \else
    \blx@hook@parboxrestore
  \fi}

\appto\@parboxrestore{\blx@parboxrestore}

%% Restore kerning

\def\csq@fixkern{%
  \expandafter\expandafter\expandafter
  \expandafter\expandafter\expandafter
  \expandafter\csq@fixkern@i}

\def\csq@fixkern@i{%
  \futurelet\csq@kernchar@ii\csq@fixkern@ii}

\def\csq@fixkern@ii{%
  \ifcat a\noexpand\csq@kernchar@ii
    \expandafter\csq@fixkern@iii
  \else
    \ifcat 1\noexpand\csq@kernchar@ii
      \expandafter\expandafter
      \expandafter\csq@fixkern@iii
    \fi
  \fi}

\def\csq@fixkern@iii{%
  \begingroup
  \settowidth{\@tempdima}{%
    \csq@kernchar@i\csq@kernchar@ii}%
  \settowidth{\@tempdimb}{%
    \csq@kernchar@i\kern\z@\csq@kernchar@ii}%
  \ifdim\@tempdima=\@tempdimb
  \else
    \addtolength{\@tempdima}{-\@tempdimb}%
    \penalty\@M\hskip\@tempdima\relax
  \fi
  \endgroup}

%% Detect and kern adjoining quotes

\def\csq@kernmarker{13sp}
\def\csq@omitmarker{17sp}
\let\csq@themarker\csq@kernmarker
\def\csq@thekern@open{\csq@thequote@kern}
\def\csq@thekern@close{\csq@thequote@kern}
\def\csq@thequote@kern{0.1em}

\def\csq@setmarker@open{%
  \penalty\@M
  \hskip-\csq@themarker\relax
  \hskip\csq@themarker\relax}

\def\csq@setmarker@close{%
  \kern-\csq@themarker\relax
  \kern\csq@themarker\relax}

\def\csq@addkern@open{%
  \ifdim\lastskip=\csq@kernmarker
    \unskip\unskip\unpenalty
    \unkern % EC fix
    \ifdim\csq@thekern@open=\z@
    \else
      \penalty\@M\hskip\csq@thekern@open\relax
    \fi
  \fi}

\def\csq@addkern@close{%
  \ifdim\lastkern=\csq@kernmarker
    \unkern\unkern
    \ifdim\csq@thekern@close=\z@
    \else
      \penalty\@M\hskip\csq@thekern@close\relax
    \fi
  \fi}

%% Punctuation

% 1001       apostrophe (biblatex only)
% 1002       abbreviation dot (biblatex only)
% 1003/1250  comma
% 1004/1500  semicolon
% 1005/2000  colon
% 1006/3000  period
% 1007/3001  exclamation mark
% 1008/3002  question mark
% 1009       suppress punctuation (biblatex only)

\mathchardef\csq@sf@comma=1003
\mathchardef\csq@sf@semicolon=1004
\mathchardef\csq@sf@colon=1005
\mathchardef\csq@sf@period=1006
\mathchardef\csq@sf@exclam=1007
\mathchardef\csq@sf@question=1008
\mathchardef\csq@sf@threshold@low=1002
\mathchardef\csq@sf@threshold@term=1005
\mathchardef\csq@sf@threshold@high=1009

\def\csq@setsfcodes{%
  \ifcsdef{csq@sfcodes@\f@encoding}
    {\csuse{csq@sfcodes@\f@encoding}}
    {\csq@warn@sfcodes\f@encoding}%
  \sfcode`\)=\z@
  \sfcode`\]=\z@
  \ifnum\sfcode`\.>2000
    \csq@setencodes
  \else
    \csq@setfrcodes
  \fi
  \let\frenchspacing\csq@setfrcodes
  \let\nonfrenchspacing\csq@setencodes
  \let\csq@setsfcodes\relax}

\def\csq@ifsfcodes{%
  \ifnumequal\csq@sf@question
    {\ifcsdef{csq@sfactor@\the\sfcode`\?}
       {\csuse{csq@sfactor@\the\sfcode`\?}}
       {\sfcode`\?}}}

\def\csq@setfrcodes{%
  \ifnum\sfcode`\A=\@m
  \else
    \csq@setazcodes
  \fi
  \sfcode`\,=1003
  \sfcode`\;=1004
  \sfcode`\:=1005
  \sfcode`\.=1006
  \sfcode`\!=1007
  \sfcode`\?=1008
}

\def\csq@setencodes{%
  \sfcode`\,=1250
  \sfcode`\;=1500
  \sfcode`\:=2000
  \sfcode`\.=3000
  \sfcode`\!=3001
  \sfcode`\?=3002
}

\begingroup
\let\csq@setazcodes\@empty
\def\csq@tempa{%
  \xdef\csq@setazcodes{\csq@setazcodes\sfcode\the\@tempcnta=\@m}
  \ifnum\@tempcnta<\@tempcntb
    \advance\@tempcnta\@ne
    \expandafter\csq@tempa
  \fi}
\@tempcnta`\A
\@tempcntb`\Z
\csq@tempa
\ifnum\inputlineno=\m@ne\else
  \@tempcnta"80
  \@tempcntb"9C
  \csq@tempa
  \@tempcnta"C0
  \@tempcntb"DF
  \csq@tempa
\fi
\endgroup

\csdef{csq@sfactor@1250}{1003}
\csdef{csq@sfactor@1500}{1004}
\csdef{csq@sfactor@2000}{1005}
\csdef{csq@sfactor@3000}{1006}
\csdef{csq@sfactor@3001}{1007}
\csdef{csq@sfactor@3002}{1008}

\def\csq@spacefactor{%
  \ifhmode
    \ifcsdef{csq@sfactor@\the\spacefactor}
      {\csuse{csq@sfactor@\the\spacefactor}}
      {\the\spacefactor}%
  \else
    1000%
  \fi}

% {<true>}{<false>}

\newcommand*{\ifpunct}{%
  \csq@ifsfcodes
    {\ifnumgreater\csq@spacefactor\csq@sf@threshold@low
       {\ifnumless\csq@spacefactor\csq@sf@threshold@high}
       {\@secondoftwo}}
    {\csq@err@sfcodes\ifpunct
     \@secondoftwo}}

% {<text>}{<true>}{<false>}

\newrobustcmd*{\iftextpunct}[1]{%
  \csq@ifpuncttest{#1}{\ifpunct}}

% {<true>}{<false>}

\newcommand*{\ifterm}{%
  \csq@ifsfcodes
    {\ifnumgreater\csq@spacefactor\csq@sf@threshold@term
       {\ifnumless\csq@spacefactor\csq@sf@threshold@high}
       {\@secondoftwo}}
    {\csq@err@sfcodes\ifterm
     \@secondoftwo}}

% {<text>}{<true>}{<false>}

\newrobustcmd*{\iftextterm}[1]{%
  \csq@ifpuncttest{#1}{\ifterm}}

% {<character>}{<true>}{<false>}

\newrobustcmd*{\ifpunctmark}[1]{%
  \csq@ifsfcodes
    {\ifbool{hmode}
       {\ifnumequal{\sfcode`#1}\spacefactor}
       {\@secondoftwo}}
    {\csq@err@sfcodes\ifpunctmark
     \@secondoftwo}}

% {<text>}{<character>}{<true>}{<false>}

\newrobustcmd*{\iftextpunctmark}[2]{%
  \csq@ifpuncttest{#1}{\ifpunctmark{#2}}}

\def\csq@ifpuncttest#1#2{%
  \begingroup
  \setbox\@tempboxa=\hbox{%
    \csq@ifsfcodes\relax\csq@setsfcodes
    #1#2
      {\aftergroup\@firstoftwo}
      {\aftergroup\@secondoftwo}}%
  {\endgroup\@firstoftwo}
  {\endgroup\@secondoftwo}}

%% Multilingual interface

\def\csq@setstyle#1{%
  \begingroup
  \let\if@safe@actives\iftrue
  \ifcsdef{csq@qstyle@#1}
    {\edef\csq@tempa{\endgroup
       \def\noexpand\csq@currentstyle{#1}%
       \noexpand\csuse{csq@qstyle@#1}}%
     \csq@tempa}
    {\csq@warnorerr
       {Quote style '#1' not defined.\MessageBreak Ignoring command}
       {Quote style '#1' not defined}
       {Define the style or alias first}
     \endgroup}}

\def\csq@resetstyle{%
  \ifnum\csq@reset=\@ne
    \ifx\csq@currentstyle\languagename
    \else
      \ifcsundef{csq@qstyle@\languagename}
        {\csq@warn@style\languagename
         \csq@setstyle{fallback}}
        {\csq@setstyle{\languagename}}%
    \fi
  \fi}

\def\csq@savelang{%
  \ifdef\csq@mainlang
    {}
    {\edef\csq@mainlang{\languagename}}}

\def\csq@resetlang{%
  \ifdef\csq@mainlang
    {\csuse{otherlanguage*}{\csq@mainlang}%
     \let\csq@resetlang\relax}
    {}}

\protected\long\def\csq@switchlang#1{%
  \ifdef\csq@mainlang
    {\begingroup
     \csuse{otherlanguage*}{\csq@mainlang}%
     #1%
     \csuse{endotherlanguage*}%
     \endgroup}
    {#1}}

% \lowercase: workaround for page headers of book.cls et al.

\def\csq@lang#1{%
  \csq@savelang
  \lowercase{\csuse{otherlanguage*}{#1}}}
\def\csq@endlang{%
  \csuse{endotherlanguage*}}

\def\csq@nolang#1{%
  \begingroup
  \lowercase{\def\csq@tempa{#1}}%
  \csq@warn@multilang{Cannot switch to language '\csq@tempa'}%
  \endgroup}

\def\csq@hyph#1{%
  \csq@savelang
  \lowercase{\csq@hyphenrules{#1}}}
\let\csq@endhyph\@empty

\def\csq@nohyph#1{%
  \begingroup
  \lowercase{\def\csq@tempa{#1}}%
  \csq@warn@multilang{No hyphenation rules for '\csq@tempa'}%
  \endgroup}

\def\csq@hyphenrules#1{%
  \language\csname l@#1\endcsname\relax
  \ifcsundef{#1hyphenmins}
    {\csq@sethyphenmins\tw@\thr@@}
    {\expandafter\expandafter\expandafter\csq@sethyphenmins
       \csname#1hyphenmins\endcsname}}

\def\csq@sethyphenmins#1#2{%
  \lefthyphenmin#1\relax
  \righthyphenmin#2\relax}

\appto\csq@hook@multilang{%
  \appto\blx@hook@parboxrestore{\csq@resetlang}%
  \ifundef\l@usenglish
    {\ifundef\l@USenglish
       {}
       {\let\l@usenglish\l@USenglish}}
    {}%
  \ifundef\l@ukenglish
    {\ifundef\l@UKenglish
       {}
       {\let\l@ukenglish\l@UKenglish}}
    {}%
  \ifcase\csq@reset
  \or
  \or
    \csq@info{Enabling multilingual quotes}%
    \csq@reset\@ne
  \else
    \csq@info{Adjusting default style}%
    \ifcsdef{csq@qstyle@\csq@main@language}
      {\DeclareQuoteAlias{\csq@main@language}{default}}
      {\csq@warn@style\csq@main@language
       \DeclareQuoteAlias{fallback}{default}}%
  \fi}

\appto\csq@hook@nomultilang{%
  \ifcase\csq@reset
  \or
    \csq@warn@multilang{Cannot enable multilingual quotes}%
  \or
  \or
    \csq@warn@multilang{Cannot adjust default style}%
  \fi
  \csq@reset\z@
  \let\csq@hyph\csq@nohyph
  \let\csq@endhyph\@empty
  \let\csq@lang\csq@nolang
  \let\csq@endlang\@empty
  \let\csq@switchlang\@firstofone
  \def\csq@resetqstyle{%
    \csq@warn@multilang{Cannot enable multilingual quotes}}}

%% Markup with control sequences

% Argument parsers

% {<macro>}[<cite>][<punct>] =>
%  <macro>{\mkcitation}{<cite>}{<punct>}

\def\csq@getcargs#1{%
  \@ifnextchar[%]
    {\csq@getcargs@i{#1}}
    {\csq@getcargs@i{#1}[]}}

\long\def\csq@getcargs@i#1[#2]{%
  \@ifnextchar[%]
    {\csq@getcargs@ii{#1}{#2}}
    {\csq@getcargs@ii{#1}{#2}[]}}

\long\def\csq@getcargs@ii#1#2[#3]{%
  #1{\mkcitation}{#2}{#3}}

% {<macro>}[<pre>][<post>]{<key>}[<punct>] =>
%  <macro>{\mkccitation}{\csq@cite[<pre>][<post>]{<key>}}{<punct>}

\def\csq@getccargs#1{%
  \@ifnextchar[%]
    {\csq@getccargs@i{#1}{}}
    {\csq@getccargs@ii{#1}{}}}

\long\def\csq@getccargs@i#1#2[#3]{%
  \@ifnextchar[%]
    {\csq@getccargs@i{#1}{#2[{#3}]}}
    {\csq@getccargs@ii{#1}{#2[{#3}]}}}

\long\def\csq@getccargs@ii#1#2#3{%
  \@ifnextchar[%]
    {\csq@getccargs@iii{#1}{#2}{#3}}
    {\csq@getccargs@iii{#1}{#2}{#3}[]}}

\long\def\csq@getccargs@iii#1#2#3[#4]{%
  #1{\mkccitation}{\csq@cite#2{#3}}{#4}}

% {<macro>}<punct> => <macro>{<apunct>}<tpunct>

\protected\long\def\csq@getpunct#1{%
  \begingroup
  \def\csq@tempa{\endgroup#1}%
  \futurelet\@let@token\csq@getpunct@i}

\def\csq@getpunct@i{%
  \expandafter\csq@getpunct@ii\csq@allpunct&}

\def\csq@getpunct@ii#1{%
  \ifx#1&%
    \expandafter\csq@getpunct@v
  \fi
  \ifx#1\@let@token
    \expandafter\csq@getpunct@iii
  \fi
  \csq@getpunct@ii}

\def\csq@getpunct@iii#1\csq@getpunct@ii#2&{%
  \expandafter\csq@getpunct@iv\csq@autopunct&}

\def\csq@getpunct@iv#1{%
  \ifx#1&%
    \expandafter\csq@getpunct@vi
  \fi
  \ifx#1\@let@token
    \expandafter\csq@getpunct@vii
  \fi
  \csq@getpunct@iv}

\def\csq@getpunct@v#1\csq@getpunct@ii{\csq@tempa{}\@empty}
\def\csq@getpunct@vi#1\csq@getpunct@iv{\csq@tempa{}}
\def\csq@getpunct@vii#1\csq@getpunct@iv#2&#3{\csq@tempa{#3}\@empty}

% Punctuation

\newrobustcmd*{\DeclareAutoPunct}[1]{%
  \ifblank{#1}
    {\def\csq@autopunct{}}
    {\def\csq@autopunct{#1}}}

\let\csq@autopunct\@empty
\def\csq@allpunct{.,;:!?}

\AfterEndPreamble{% babel
  \begingroup
  \makeatletter
  \endlinechar\m@ne
  \edef\csq@tempa{%
    \noexpand\scantokens{%
      \gdef\noexpand\csq@autopunct{\csq@autopunct}%
      \gdef\noexpand\csq@allpunct{\csq@allpunct}}}%
  \csq@tempa
  \endgroup}

% Plain quotes

\newrobustcmd*{\enquote}{%
  \@ifstar{\csq@quote@ii{}{}}{\csq@quote@i{}{}}}

% {<init>}{<endinit>}{<text>}

\long\def\csq@quote@i#1#2#3{%
  \csq@bqgroup#1\csq@oqopen@i#3\csq@qclose@i{#2}}
\long\def\csq@quote@ii#1#2#3{%
  \csq@bqgroup#1\csq@iqopen@i#3\csq@qclose@i{#2}}

% Plain quotes + language switching

\newrobustcmd*{\foreignquote}{%
  \@ifstar\csq@fquote@ii\csq@fquote@i}

\def\csq@fquote@i#1{\csq@quote@i{\csq@lang{#1}}{\csq@endlang}}
\def\csq@fquote@ii#1{\csq@quote@ii{\csq@lang{#1}}{\csq@endlang}}

\newrobustcmd*{\hyphenquote}{%
  \@ifstar\csq@hquote@ii\csq@hquote@i}

\def\csq@hquote@i#1{\csq@quote@i{\csq@hyph{#1}}{\csq@endhyph}}
\def\csq@hquote@ii#1{\csq@quote@ii{\csq@hyph{#1}}{\csq@endhyph}}

% PDF strings

\long\def\csq@pdf@quote#1{%
  \if#1*\relax
    \expandafter\@firstoftwo
  \else
    \expandafter\@secondoftwo
  \fi
    {\csq@pdf@quote@ii}
    {\csq@pdf@quote@i{#1}}}

\long\def\csq@pdf@quote@i#1{%
  \csq@pdf@ooqmark #1\csq@pdf@coqmark}
\long\def\csq@pdf@quote@ii#1{%
  \csq@pdf@oiqmark #1\csq@pdf@ciqmark}

\long\def\csq@pdf@fquote#1{%
  \if#1*\relax
    \expandafter\@firstoftwo
  \else
    \expandafter\@secondoftwo
  \fi
    {\expandafter\csq@pdf@quote@ii\@gobble}
    {\csq@pdf@quote@i}}

\appto\csq@hook@hyperref{%
  \let\enquote\csq@pdf@quote
  \let\foreignquote\csq@pdf@fquote
  \let\hyphenquote\csq@pdf@fquote}

% Text quotes

\newrobustcmd*{\textquote}{%
  \@ifstar
    {\csq@getcargs{\csq@tquote{}{}{\csq@iqopen@i}}}
    {\csq@getcargs{\csq@tquote{}{}{\csq@oqopen@i}}}}

% {<init>}{<endinit>}{<qopen>}{<citehook>}{<cite>}{<punct>}{<text>}

\long\def\csq@tquote#1#2#3#4#5#6#7{%
  \csq@getpunct{\csq@tquote@i{#1}{#2}{#3}{#4}{#5}{#6}{#7}}}

% {<init>}{<endinit>}{<qopen>}{<citehook>}{<cite>}{<punct>}{<text>}{<apunct>}<tpunct>

\long\def\csq@tquote@i#1#2#3#4#5#6#7#8#9{%
  \begingroup
  \csq@setsfcodes
  \edef\csq@tempa{%
    \unexpanded{%
      \mktextquote
      {#3}%
      {#7}%
      {\csq@qclose@i{#2}}%
      {#6}{#8}}%
    {\ifblank{#5}
       {}
       {\unexpanded{\csq@switchlang{#4{#5}}}}}}%
  \csq@bqgroup#1\csq@tempa#9%
  \endgroup}

% {<qopen>}{<text>}{<qclose>}{<punct>}{<apunct>}{<cite>}

\newcommand{\mktextquote}[6]{#1#2#4#3#6#5}

% Text quotes + language switching

\newrobustcmd*{\foreigntextquote}{%
  \@ifstar\csq@ftquote@ii\csq@ftquote@i}

\def\csq@ftquote@i#1{%
  \csq@getcargs{\csq@tquote{\csq@lang{#1}}{\csq@endlang}{\csq@oqopen@i}}}
\def\csq@ftquote@ii#1{%
  \csq@getcargs{\csq@tquote{\csq@lang{#1}}{\csq@endlang}{\csq@iqopen@i}}}

\newrobustcmd*{\hyphentextquote}{%
  \@ifstar\csq@htquote@ii\csq@htquote@i}

\def\csq@htquote@i#1{%
  \csq@getcargs{\csq@tquote{\csq@hyph{#1}}{\csq@endhyph}{\csq@oqopen@i}}}
\def\csq@htquote@ii#1{%
  \csq@getcargs{\csq@tquote{\csq@hyph{#1}}{\csq@endhyph}{\csq@iqopen@i}}}

% Integrated text quotes

\newrobustcmd*{\textcquote}{%
  \@ifstar
    {\csq@getccargs{\csq@tquote{}{}{\csq@iqopen@i}}}
    {\csq@getccargs{\csq@tquote{}{}{\csq@oqopen@i}}}}

% Integrated text quotes + language switching

\newrobustcmd*{\foreigntextcquote}{%
  \@ifstar\csq@ftcquote@ii\csq@ftcquote@i}

\def\csq@ftcquote@i#1{%
  \csq@getccargs{\csq@tquote{\csq@lang{#1}}{\csq@endlang}{\csq@oqopen@i}}}
\def\csq@ftcquote@ii#1{%
  \csq@getccargs{\csq@tquote{\csq@lang{#1}}{\csq@endlang}{\csq@iqopen@i}}}

\newrobustcmd*{\hyphentextcquote}{%
  \@ifstar\csq@htcquote@ii\csq@htcquote@i}

\def\csq@htcquote@i#1{%
  \csq@getccargs{\csq@tquote{\csq@hyph{#1}}{\csq@endhyph}{\csq@oqopen@i}}}
\def\csq@htcquote@ii#1{%
  \csq@getccargs{\csq@tquote{\csq@hyph{#1}}{\csq@endhyph}{\csq@iqopen@i}}}

% PDF strings

\appto\csq@hook@hyperref{%
  \def\textquote{\pdfstringdefWarn\textquote}%
  \def\foreigntextquote{\pdfstringdefWarn\foreigntextquote}%
  \def\hyphentextquote{\pdfstringdefWarn\hyphentextquote}%
  \def\textcquote{\pdfstringdefWarn\textcquote}%
  \def\foreigntextcquote{\pdfstringdefWarn\foreigntextcquote}%
  \def\hyphentextcquote{\pdfstringdefWarn\hyphentextcquote}}

% Block quotes

\newrobustcmd*{\blockquote}{%
  \csq@getcargs{\csq@bquote{}{}}}

% {<init>}{<endinit>}{<citehook>}{<cite>}{<punct>}{<text>}

\long\def\csq@bquote#1#2#3#4#5#6{%
  \csq@ifnested
    {\csq@err@nbquote}
    {\csq@getpunct{%
       \ifbool{inner}
         {\csq@bquote@ii}
	 {\ifbool{csdisplay}
	    {\csq@bquote@i}
	    {\iftoggle{csq@parbox}\csq@bquote@ii\csq@bquote@i}}%
	 {#1}{#2}{#3}{#4}{#5}{#6}}}}

% {<init>}{<endinit>}{<citehook>}{<cite>}{<punct>}{<text>}{<apunct>}<tpunct>

\long\def\csq@bquote@i#1#2#3#4#5#6{%
  \begingroup
  \blockquote@prehook
  \togglefalse{csq@tempsw}%
  \setbox\@tempboxa=\vbox{%
    \csuse{csq@bcount@\csq@thresholdtype}%
    \parindent\z@
    \blockquote@parsehook
    #1#6#5#2\endgraf\expandafter}\expandafter
  \@tempcnta\number\prevgraf\relax
  \iftoggle{csq@tempsw}
    {\csq@debug{%
       \@backslashchar blockquote has \number\@tempcnta\space
       \csq@thresholdtype\space and manual breaks.\MessageBreak
       Setting as display}}
    {\ifnumgreater\@tempcnta\csq@tshold
       {\toggletrue{csq@tempsw}}
       {}%
     \csq@debug{%
       \@backslashchar blockquote has \number\@tempcnta\space
       \csq@thresholdtype. Threshold is \number\csq@tshold.\MessageBreak
       Setting \iftoggle{csq@tempsw}{as display}{inline}}}%
  \blockquote@posthook
  \iftoggle{csq@tempsw}
    {\aftergroup\@firstoftwo}
    {\aftergroup\@secondoftwo}%
  \endgroup
  \csq@bquote@iii\csq@bquote@ii{#1}{#2}{#3}{#4}{#5}{#6}}

\def\csq@bcount@lines{%
  \iftoggle{csq@parthreshold}
    {\def\par{\global\toggletrue{csq@tempsw}\@@par}%
     \let\newline\par
     \let\\\par}
    {}%
  \parfillskip\z@\@plus1fil\relax}

\def\csq@bcount@words{%
  \iftoggle{csq@parthreshold}
    {\def\par{\global\toggletrue{csq@tempsw}\space}%
     \let\newline\par
     \let\\\par}
    {\let\par\space
     \let\newline\space
     \let\\\space}%
  \let\nobreakspace\space
  \let~\space
  \hsize\z@
  \hyphenpenalty\@M
  \exhyphenpenalty\csq@splitcomp
  \relpenalty\@M
  \binoppenalty\@M
  \let\allowbreak\relax
  \hfuzz\maxdimen}

\newcommand*{\blockquote@prehook}{%
  \def\@elt##1{\global\value{##1}\the\value{##1}\relax}%
  \edef\csq@tempa{\cl@@ckpt}%
  \let\@elt\relax
  \@fileswfalse}

\newcommand*{\blockquote@posthook}{%
  \csq@tempa}

\newcommand*{\blockquote@parsehook}{%
  \let\csq@nbgobble\@gobble
  \let\csq@bquote\@gobblefive
  \let\csq@warnorerr\@gobblethree
  \let\csq@error\@gobbletwo
  \let\csq@warning\@gobble
  \let\csq@info\@gobble
  \def\textelp{\@ifstar\@gobble\@gobble}%
  \let\textins\textelp
  \let\marginpar\@gobbletwo@optarg
  \let\label\@gobble
  \let\index\@gobble
  \let\glossary\@gobble}

\newrobustcmd*{\BlockquoteDisable}{%
  \gappto\blockquote@parsehook}

\let\csq@nbgobble\@firstofone

% {<init>}{<endinit>}{<citehook>}{<cite>}{<punct>}{<text>}{<apunct>}<tpunct>

\def\csq@bquote@ii#1#2{\csq@tquote@i{#1}{#2}{\csq@oqopen@i}}

% {<init>}{<endinit>}{<citehook>}{<cite>}{<punct>}{<text>}{<apunct>}<tpunct>

\long\def\csq@bquote@iii#1#2#3#4#5#6#7#8{%
  \begin{\csq@blockenvironment}%
  \toggletrue{csq@block}%
  \csq@setsfcodes
  \edef\csq@tempa{%
    \unexpanded{%
      \mkblockquote
      {#6}%
      {#5}{#7}}%
    {\ifblank{#4}
       {}
       {\unexpanded{\csq@switchlang{#3{#4}}}}}}%
  #1\csq@tempa#8#2%
  \end{\csq@blockenvironment}}

% {<text>}{<punct>}{<apunct>}{<cite>}

\newcommand{\mkblockquote}[4]{#1#2#4#3}

% Block quotes + language switching

\newrobustcmd*{\foreignblockquote}[1]{%
  \csq@getcargs{\csq@bquote{\csq@lang{#1}}{\csq@endlang}}}

\newrobustcmd*{\hyphenblockquote}[1]{%
  \csq@getcargs{\csq@bquote{\csq@hyph{#1}}{\csq@endhyph}}}

\newrobustcmd*{\hybridblockquote}[1]{%
  \csq@getcargs{%
    \csq@bquote
      {\iftoggle{csq@block}{\csq@lang}{\csq@hyph}{#1}}
      {\iftoggle{csq@block}{\csq@endlang}{\csq@endhyph}}}}

% Integrated block quotes

\newrobustcmd*{\blockcquote}{%
  \csq@getccargs{\csq@bquote{}{}}}

% Integrated block quotes + language switching

\newrobustcmd*{\foreignblockcquote}[1]{%
  \csq@getccargs{\csq@bquote{\csq@lang{#1}}{\csq@endlang}}}

\newrobustcmd*{\hyphenblockcquote}[1]{%
  \csq@getccargs{\csq@bquote{\csq@hyph{#1}}{\csq@endhyph}}}

\newrobustcmd*{\hybridblockcquote}[1]{%
  \csq@getccargs{%
    \csq@bquote
      {\iftoggle{csq@block}{\csq@lang}{\csq@hyph}{#1}}
      {\iftoggle{csq@block}{\csq@endlang}{\csq@endhyph}}}}

% PDF strings

\appto\csq@hook@hyperref{%
  \def\blockquote{\pdfstringdefWarn\blockquote}%
  \def\foreignblockquote{\pdfstringdefWarn\foreignblockquote}%
  \def\hyphenblockquote{\pdfstringdefWarn\hyphenblockquote}%
  \def\blockcquote{\pdfstringdefWarn\blockcquote}%
  \def\foreignblockcquote{\pdfstringdefWarn\foreignblockcquote}%
  \def\hyphenblockcquote{\pdfstringdefWarn\hyphenblockcquote}}

% Display quotes

\newenvironment*{displayquote}
  {\csq@getcargs{\csq@bdquote{}{}}}
  {\csq@edquote}

% {<init>}{<endinit>}{<citehook>}{<cite>}{<punct>}

\def\csq@bdquote#1#2#3#4#5{%
  \csuse{\csq@blockenvironment}%
  \toggletrue{csq@block}%
  \csq@setsfcodes
  #1\ifblank{#4}
    {\def\csq@tempb{\mkenddispquote{#5}{}#2}%
     \mkbegdispquote{#5}{}}
    {\def\csq@tempb{\mkenddispquote{#5}{\csq@switchlang{#3{#4}}}#2}%
     \mkbegdispquote{#5}{\csq@switchlang{#3{#4}}}}%
  \ignorespaces}

\def\csq@edquote{%
  \unspace\csq@tempb
  \csuse{end\csq@blockenvironment}}

\providerobustcmd*{\unspace}{%
  \ifbool{hmode}
    {\ifdimgreater\lastskip\z@
       {\unskip\unspace}
       {\ifnumgreater\lastpenalty\z@
	  {\unpenalty\unspace}
	  {}}}
    {}}

% {<punct>}{<cite>}

\newcommand{\mkbegdispquote}[2]{}
\newcommand{\mkenddispquote}[2]{#1#2}

% Display quotes + language switching

\newenvironment*{foreigndisplayquote}[1]
  {\csq@getcargs{\csq@bdquote{\csq@lang{#1}}{\csq@endlang}}}
  {\csq@edquote}

\newenvironment*{hyphendisplayquote}[1]
  {\csq@getcargs{\csq@bdquote{\csq@hyph{#1}}{\csq@endhyph}}}
  {\csq@edquote}

% Integrated display quotes

\newenvironment*{displaycquote}
  {\csq@getccargs{\csq@bdquote{}{}}}
  {\csq@edquote}

% Integrated display quotes + language switching

\newenvironment*{foreigndisplaycquote}[1]
  {\csq@getccargs{\csq@bdquote{\csq@lang{#1}}{\csq@endlang}}}
  {\csq@edquote}

\newenvironment*{hyphendisplaycquote}[1]
  {\csq@getccargs{\csq@bdquote{\csq@hyph{#1}}{\csq@endhyph}}}
  {\csq@edquote}

% Hooks

\newcommand{\mkcitation}[1]{\space(#1)}
\newcommand{\mkccitation}[1]{\space#1}

%% Markup with active characters

\let\csq@dospecials\@empty
\let\csq@doutfspecials\@empty

\def\csq@do@dospecial#1#2{%
  \ifnum\catcode`#1=\active
    \csq@info{Redefining character \string#1}%
    \csq@letspecial{#1}{csq@special@\number`#1}%
  \else
    \csq@info{Making character \string#1 active}%
    \csq@letspecial{#1}{csq@special@\number`#1}%
    \catcode`#1=\active
  \fi}

\def\csq@do@undospecial#1#2{%
  \ifnum#2=\active
    \csq@info{Resetting character \string#1}%
    \csq@letspecial{#1}{csq@saved@\number`#1}%
  \else
    \csq@info{Resetting catcode of \string#1}%
    \catcode`#1=#2\relax
  \fi}

\def\csq@do@verbspecial#1#2{%
  \csq@info{Redefining character \string#1}%
  \ifnum`#1<128\relax
    \csq@edefspecial{#1}{\string#1}%
  \else
    \csq@letspecial{#1}{csq@saved@\number`#1}%
  \fi}

\def\csq@do@doutfspecial#1{%
  \csq@info{Redefining character \csq@utfprint{#1}}%
  \csletcs{u8:\csq@string{#1}}{csq@special@\csq@number{#1}}}

\def\csq@do@undoutfspecial#1{%
  \csq@info{Resetting character \csq@utfprint{#1}}%
  \csletcs{u8:\csq@string{#1}}{csq@saved@\csq@number{#1}}}

\def\csq@do@delspecial#1#2{%
  \csq@info{Deallocating character \string#1}%
  \csundef{csq@special@\number`#1}%
  \csundef{csq@saved@\number`#1}%
  \csundef{csq@string@\number`#1}%
  \csundef{csq@textdef@\number`#1}%
  \csundef{csq@xtxtdef@\number`#1}%
  \csundef{csq@pdfdef@\number`#1}}

\def\csq@do@delutfspecial#1{%
  \csq@info{Deallocating character \csq@utfprint{#1}}%
  \csundef{csq@special@\csq@number{#1}}%
  \csundef{csq@saved@\csq@number{#1}}%
  \csundef{csq@string@\csq@number{#1}}%
  \csundef{csq@textdef@\csq@number{#1}}%
  \csundef{csq@xtxtdef@\csq@number{#1}}%
  \csundef{csq@pdfdef@\csq@number{#1}}}

\def\csq@mkenable{%
  \let\do\csq@do@dospecial
  \csq@dospecials
  \let\do\csq@do@doutfspecial
  \csq@doutfspecials
  \let\do\noexpand
  \toggletrue{csq@active}}

\def\csq@mkdisable{%
  \iftoggle{csq@active}
    {\let\do\csq@do@undospecial
     \csq@dospecials
     \let\do\csq@do@undoutfspecial
     \csq@doutfspecials
     \let\do\noexpand
     \togglefalse{csq@active}}
    {}}

\def\csq@mkverbatim{%
  \iftoggle{csq@active}
    {\let\do\csq@do@verbspecial
     \csq@dospecials
     \let\do\csq@do@undoutfspecial
     \csq@doutfspecials
     \let\do\noexpand}
    {}}

\def\csq@mkdelete{%
  \csq@mkdisable
  \let\do\csq@do@delspecial
  \csq@dospecials
  \let\do\csq@do@delutfspecial
  \csq@doutfspecials
  \let\do\noexpand
  \let\csq@dospecials\@empty
  \let\csq@doutfspecials\@empty
  \let\csq@mkpdfstrings\@empty}

\let\csq@mkpdfstrings\@empty
\appto\csq@hook@hyperref{\csq@mkpdfstrings}

\ifdef\inpenc@prehook
  {\AtBeginDocument{%
     \addto@hook\inpenc@prehook{%
        \csq@info{Input encoding change}%
        \csq@mkdelete}}}
  {}

% Regular specials

% {<char>}{<textdef>}{<pdfdef1>}{<pdfdef2>}

\def\csq@addspecial#1#2#3#4{%
  \csq@validate{#1}
    {\csq@addspecial@i@s{#1}{\csqQQ}{#2}{#3}{#4}}
    {\csq@addspecial@i@u{#1}{\csqQQ}{#2}{#3}{#4}}}

% {<char>}{<macro>}{<textdef>}{<pdfdef1>}{<pdfdef2>}

\def\csq@addspecial@i@s#1#2#3#4#5{%
  \csq@info{Allocating character \string#1}%
  \csedef{csq@special@\number`#1}{\noexpand#2{\number`#1}}%
  \ifnum\catcode`#1=\active
    \cslet{csq@saved@\number`#1}{#1}%
  \else
    \csdef{csq@saved@\number`#1}{#1}%
  \fi
  \csedef{csq@string@\number`#1}{\string#1}%
  \csdef{csq@textdef@\number`#1}{#3}%
  \ifblank{#5}
    {\csdef{csq@pdfdef@\number`#1}{#4}}
    {\appto\csq@mkpdfstrings{\csq@defpspecial{#1}{#4}{#5}}}%
  \eappto\csq@dospecials{\noexpand\do{\string#1}{\the\catcode`#1}}%
  \ifnum`#1<128\relax
    \csq@addto@list{#1}{\dospecials}{\do}%
    \csq@addto@list{#1}{\@sanitize}{\@makeother}%
  \fi}

% {<char>}{<macro>}{<textdef>}{<pdfdef1>}{<pdfdef2>}

\def\csq@addspecial@i@u#1#2#3#4#5{%
  \csq@info{Allocating character \csq@utfprint{#1}}%
  \csedef{csq@special@\csq@number{#1}}{%
    \noexpand#2{\csq@number{#1}}}%
  \ifcsundef{u8:\csq@string{#1}}
    {\csq@error
       {\csq@utfprint{#1} not supported by inputenc}
       {This UTF-8 sequence does not seem to be supported by the
        inputenc\MessageBreak package}%
     \csdef{csq@saved@\csq@number{#1}}{}}
    {\csletcs{csq@saved@\csq@number{#1}}{u8:\csq@string{#1}}}%
  \csedef{csq@string@\csq@number{#1}}{\csq@string{#1}}%
  \csdef{csq@textdef@\csq@number{#1}}{#3}%
  \ifblank{#5}
    {\csdef{csq@pdfdef@\csq@number{#1}}{#4}}
    {\appto\csq@mkpdfstrings{\csq@defupspecial{#1}{#4}{#5}}}%
  \eappto\csq@doutfspecials{\noexpand\do{\csq@string{#1}}}}

% Block specials

% {<char1>}{<delim>}{<char2>}{<textdef>}

\def\csq@addbspecial#1#2#3#4{%
  \csq@validate{#1}
    {\csq@addbspecial@i@s{#1}{#2}{#3}{#4}}
    {\csq@addbspecial@i@u{#1}{#2}{#3}{#4}}}

\def\csq@addbspecial@i@s#1#2#3#4{%
  \begingroup
  \def\csq@tempa{\endgroup\csq@addspecial@i@s{#1}{\csqBQ}{}}%
  \eappto\csq@tempa{%
    {\expandafter\noexpand\csname csq@saved@\number`#1\endcsname
     \noexpand\pdfstringdefWarn{\string#1}}{}}%
  \csq@tempa
  \csq@validate{#2}
    {\csq@addbspecial@ii@s{\number`#1}{#2}{#3}{#4}}
    {\csq@addbspecial@ii@u{\number`#1}{#2}{#3}{#4}}}

\def\csq@addbspecial@i@u#1#2#3#4{%
  \begingroup
  \def\csq@tempa{\endgroup\csq@addspecial@i@u{#1}{\csqBQ}{}}%
  \eappto\csq@tempa{%
    {\expandafter\noexpand\csname csq@saved@\csq@number{#1}\endcsname
     \noexpand\pdfstringdefWarn{\csq@utfprint{#1}}}{}}%
  \csq@tempa
  \csq@validate{#2}
    {\csq@addbspecial@ii@s{\csq@number{#1}}{#2}{#3}{#4}}
    {\csq@addbspecial@ii@u{\csq@number{#1}}{#2}{#3}{#4}}}

\def\csq@addbspecial@ii@s#1#2#3#4{%
  \csq@addspecial@i@s{#2}{\csqBQsep}{}{}{}%
  \begingroup
  \let\csq@tempa\@empty
  \def\csq@tempb{{#1}}%
  \uccode`\~=`#2\relax
  \uppercase{\appto\csq@tempb{{~}}}%
  \appto\csq@tempb{{#3}{#4}}%
  \csq@validate{#3}
    {\expandafter\def\expandafter\csq@tempa
     \expandafter{\expandafter\csq@addbspecial@iii@s\csq@tempb}}
    {\expandafter\def\expandafter\csq@tempa
     \expandafter{\expandafter\csq@addbspecial@iii@u\csq@tempb}}%
  \expandafter\endgroup\csq@tempa}

\def\csq@addbspecial@ii@u#1#2#3#4{%
  \csq@addspecial@i@u{#2}{\csqBQsep}{}{}{}%
  \csq@validate{#3}
    {\csq@addbspecial@iii@s{#1}{#2}{#3}{#4}}
    {\csq@addbspecial@iii@u{#1}{#2}{#3}{#4}}}

\def\csq@addbspecial@iii@s#1#2#3#4{%
  \csq@addspecial@i@s{#3}{\csqBQend}{}{}{}%
  \begingroup
  \def\csq@tempa{{#1}{#2}}%
  \uccode`\~=`#3\relax
  \uppercase{\appto\csq@tempa{~}}%
  \appto\csq@tempa{{#4}}%
  \expandafter\endgroup
  \expandafter\csq@addbspecial@iv\csq@tempa}

\def\csq@addbspecial@iii@u#1#2#3#4{%
  \csq@addspecial@i@u{#3}{\csqBQend}{}{}{}%
  \csq@addbspecial@iv{#1}{#2}{#3}{#4}}

\def\csq@addbspecial@iv#1#2#3#4{%
  \expandafter\csq@defbspecial
  \expandafter{\csname csq@textdef@#1\endcsname}{#2}{#3}{#4}%
  \expandafter\csq@defxbspecial
  \expandafter{\csname csq@xtxtdef@#1\endcsname}{#4}}

% Specials

\newcommand*{\csqQQ}[1]{%
  \csq@ifsafeactives
    {\csuse{csq@string@#1}}
    {\csq@iftypeset
       {\ifbool{mmode}
          {\csuse{csq@saved@#1}}
          {\csuse{csq@textdef@#1}}}
       {\csq@ifstrings
          {\csuse{csq@string@#1}}
          {\noexpand\csqQQ{#1}}}}}

\newcommand*{\csqBQ}[1]{%
  \csq@ifsafeactives
    {\csuse{csq@string@#1}}
    {\csq@iftypeset
       {\ifbool{mmode}
          {\csuse{csq@saved@#1}}
          {\csq@ifnested
             {\csq@err@nbquote}
             {\csq@nbgobble{\csuse{csq@textdef@#1}}}}}
       {\csq@ifstrings
          {\csuse{csq@string@#1}}
          {\noexpand\csqBQbeg{#1}}}}}

\newcommand*{\csqBQbeg}[1]{%
  \csq@ifsafeactives
    {\csuse{csq@string@#1}}
    {\csq@iftypeset
       {\ifbool{mmode}
          {\csuse{csq@saved@#1}}
          {\csq@ifnested
             {\csq@err@nbquote}
             {\csq@nbgobble{\csuse{csq@xtxtdef@#1}}}}}
       {\csq@ifstrings
          {\csuse{csq@string@#1}}
          {\noexpand\csqBQbeg{#1}}}}}

\newcommand*{\csqBQsep}[1]{%
  \csq@ifsafeactives
    {\csuse{csq@string@#1}}
    {\csq@iftypeset
       {\csuse{csq@saved@#1}}
       {\csq@ifstrings
          {\csuse{csq@string@#1}}
          {\noexpand\csqBQsep{#1}}}}}

\newcommand*{\csqBQend}[1]{%
  \csq@ifsafeactives
    {\csuse{csq@string@#1}}
    {\csq@iftypeset
       {\csuse{csq@saved@#1}}
       {\csq@ifstrings
          {\csuse{csq@string@#1}}
          {\noexpand\csqBQend{#1}}}}}

\appto\csq@hook@hyperref{%
  \def\csqQQ#1{\csuse{csq@pdfdef@#1}}%
  \def\csqBQ#1{\csuse{csq@pdfdef@#1}}%
  \def\csqBQbeg#1{\csuse{csq@pdfdef@#1}}%
  \def\csqBQsep#1{\csuse{csq@saved@#1}}%
  \def\csqBQend#1{\csuse{csq@saved@#1}}}

% Define specials

% {<char>}{<def>}

\def\csq@edefspecial#1#2{%
  \begingroup
  \uccode`\~=`#1\relax
  \uppercase{\endgroup\edef~}{#2}}

% {<char>}{<csname>}

\def\csq@letspecial#1#2{%
  \begingroup
  \uccode`\~=`#1\relax
  \uppercase{\def\csq@tempa{\endgroup\let~}}%
  \expandafter\csq@tempa\csname#2\endcsname}

% {<macro>}{<delim>}{<char2>}{<def>}

\def\csq@defbspecial#1#2#3#4{%
  \long\def#1##1#3{\csq@bspecial@i{##1}{#2}{#4}}}

% {<text>}{<delim>}{<macro>}

\long\def\csq@bspecial@i#1#2#3{%
  \long\def\csq@bspecial@ii##1#2##2&{%
    \ifblank{##2}
      {#3{}{}{#1}}
      {\csq@bspecial@iii#1&}}%
  \long\def\csq@bspecial@iii##1#2##2&{%
    #3{##2}{}{##1}}%
  \csq@bspecial@ii#1#2&}

% {<macro>}{<def>}

\def\csq@defxbspecial#1#2{%
  \long\def#1##1\csqBQend##2{\csq@xbspecial@i{##1}{#2}}}

% {<text>}{<macro>}

\long\def\csq@xbspecial@i#1#2{%
  \long\def\csq@xbspecial@ii##1\csqBQsep##2&{%
    \ifblank{##2}
      {#2{}{}{#1}}
      {\csq@xbspecial@iii#1&}}%
  \long\def\csq@xbspecial@iii##1\csqBQsep##2##3&{%
    #2{##3}{}{##1}}%
  \csq@xbspecial@ii#1\csqBQsep&}

% {<char>}{<pdfomark>}{<pdfcmark>}

\def\csq@defpspecial#1#2#3{%
  \begingroup
  \uccode`\~=`#1\relax
  \uppercase{\endgroup\def~##1~}{#2##1#3}}

% {<char>}{<pdfomark>}{<pdfcmark>}

\def\csq@defupspecial#1#2#3{%
  \expandafter\def\csname u8:\csq@string{#1}\endcsname##1#1{#2##1#3}}

% Validate user input

% {<char>}{<macro>}{<utfmacro>}

\def\csq@validate#1#2#3{%
  \csq@ifutfchar{#1}
    {\csq@ifvalidutf{#1}
       {\ifcsundef{csq@special@\csq@number{#1}}
           {#3}
           {\csq@err@alloc}}
       {\csq@err@utf}}
    {\csq@ifvalidchar{#1}
       {\ifcsundef{csq@special@\number`#1}
          {#2}
          {\csq@err@alloc}}
       {\csq@err@char}}}

% {<char>}{<true>}{<false>}

\def\csq@ifutfchar#1{%
  \ifundef\@inpenc@undefined
    {\@secondoftwo}
    {\csq@ifutfenc}%
  {\csq@ifsingle{#1}
     {\ifnum`#1<128\relax
        \expandafter\@secondoftwo
      \else
        \csq@err@utf
        \expandafter\@gobbletwo
      \fi}
     {\@firstoftwo}}
  {\csq@ifsingle{#1}
     {\@secondoftwo}
     {\csq@err@char
      \@gobbletwo}}}

\ifundef\inputencodingname
  {\def\csq@ifutfenc{%
     \csq@ifucs
       {\csq@err@ucs\@secondoftwo}
       {\begingroup
        \def\@inpenc@undefined@##1{\def\inputencodingname{##1}}%
        \@inpenc@undefined
        \ifdefstring\inputencodingname{utf8}
	  {\aftergroup\@firstoftwo}
	  {\aftergroup\@secondoftwo}%
        \endgroup}}}
  {\def\csq@ifutfenc{%
     \csq@ifucs
       {\csq@err@ucs\@secondoftwo}
       {\ifdefstring\inputencodingname{utf8}}}}

% {<char>}{<true>}{<false>}

\long\def\csq@ifsingle#1{%
  \ifblank{#1}
    {\@secondoftwo}
    {\expandafter\csq@ifsingle@i
     \string#1&&\@secondoftwo\@firstoftwo:}}
\long\def\csq@ifsingle@i#1#2#3&#4#5#6:{#5}

% {<char>}{<true>}{<false>}

\def\csq@ifvalidchar#1{%
  \begingroup
  \@tempswafalse
  \ifnum\active=\catcode`#1\relax
    \@tempswatrue
  \else\ifnum12=\catcode`#1\relax
    \@tempswatrue
  \fi\fi
  \if@tempswa
    \csq@ifvalidchar@i{#1}%
  \fi
  \if@tempswa
    \aftergroup\@firstoftwo
  \else
    \aftergroup\@secondoftwo
  \fi
  \endgroup}

\def\csq@ifvalidchar@i#1{%
  \def\break\fi##1\relax{\fi\@tempswafalse}%
  \def\do##1{\ifnum`##1=`#1\relax\break\fi}%
  \csq@resrvdchars\relax}

\def\csq@resrvdchars{%
  \do\[\do\]\do\*\do\@\do\~\do\-\do\`\do\'\do\.\do\,\do\;\do\:%
  \do\!\do\?\do\0\do\1\do\2\do\3\do\4\do\5\do\6\do\7\do\8\do\9}

% {<char>}{<true>}{<false>}

\def\csq@ifvalidutf#1{%
  \ifblank{#1}{\@secondoftwo}{\csq@ifvalidutf@i#1&}}

\def\csq@ifvalidutf@i#1#2&{%
  \ifblank{#2}
    {\@secondoftwo}% 0x00-0x7F handled elsewhere
    {\csq@ifutfstart{#1}{\csq@ifvalidutf@ii#2&}{\@secondoftwo}}}

\def\csq@ifvalidutf@ii#1#2&{%
  \csq@ifutfnext{#1}
    {\ifblank{#2}{\@firstoftwo}{\csq@ifvalidutf@ii#2&}}
    {\@secondoftwo}}

% 0xC0-0xFD, 0x80-0xBF, 0x80-0xBF, ...

\def\csq@ifutfstart#1{%
  \ifnum`#1>191\relax
    \ifnum`#1<254\relax
      \expandafter\expandafter
      \expandafter\@firstoftwo
    \else
      \expandafter\expandafter
      \expandafter\@secondoftwo
    \fi
  \else
    \expandafter\@secondoftwo
  \fi}

\def\csq@ifutfnext#1{%
  \ifnum`#1>127\relax
    \ifnum`#1<192\relax
      \expandafter\expandafter
      \expandafter\@firstoftwo
    \else
      \expandafter\expandafter
      \expandafter\@secondoftwo
    \fi
  \else
    \expandafter\@secondoftwo
  \fi}

\def\csq@isvalid#1#2#3{#2}

% User interface

\newrobustcmd*{\MakeOuterQuote}[1]{%
  \csq@addspecial{#1}{\csq@oqmark}
    {\csq@pdf@ooqmark}{\csq@pdf@coqmark}}

\newrobustcmd*{\MakeInnerQuote}[1]{%
  \csq@addspecial{#1}{\csq@iqmark}
    {\csq@pdf@oiqmark}{\csq@pdf@ciqmark}}

\newrobustcmd*{\MakeAutoQuote}{%
  \@ifstar
    {\csq@mkaquote\csq@iqopen}
    {\csq@mkaquote\csq@oqopen}}
\def\csq@mkaquote#1#2#3{%
  \csq@addspecial{#2}{#1}{\csq@pdf@ooqmark}{}%
  \csq@addspecial{#3}{\csq@qclose}{\csq@pdf@coqmark}{}}

\newrobustcmd*{\MakeForeignQuote}{%
  \@ifstar
    {\csq@mkfquote\csq@iqopen@i}
    {\csq@mkfquote\csq@oqopen@i}}
\def\csq@mkfquote#1#2#3#4{%
  \csq@addspecial{#3}
    {\csq@bqgroup\csq@lang{#2}#1}
    {\csq@pdf@ooqmark}{}%
  \csq@addspecial{#4}
    {\csq@qclose@i{\csq@endlang}}
    {\csq@pdf@coqmark}{}}

\newrobustcmd*{\MakeHyphenQuote}{%
  \@ifstar
    {\csq@mkhquote\csq@iqopen@i}
    {\csq@mkhquote\csq@oqopen@i}}
\def\csq@mkhquote#1#2#3#4{%
  \csq@addspecial{#3}
    {\csq@bqgroup\csq@hyph{#2}#1}
    {\csq@pdf@ooqmark}{}%
  \csq@addspecial{#4}
    {\csq@qclose@i{\csq@endhyph}}
    {\csq@pdf@coqmark}{}}

\newrobustcmd*{\MakeBlockQuote}[3]{%
  \csq@addbspecial{#1}{#2}{#3}{\csq@bquote{}{}{\mkcitation}}}

\newrobustcmd*{\MakeForeignBlockQuote}[4]{%
  \csq@addbspecial{#2}{#3}{#4}%
    {\csq@bquote{\csq@lang{#1}}{\csq@endlang}{\mkcitation}}}

\newrobustcmd*{\MakeHyphenBlockQuote}[4]{%
  \csq@addbspecial{#2}{#3}{#4}%
    {\csq@bquote{\csq@hyph{#1}}{\csq@endhyph}{\mkcitation}}}

\newrobustcmd*{\MakeHybridBlockQuote}[4]{%
  \csq@addbspecial{#2}{#3}{#4}%
    {\csq@bquote
       {\iftoggle{csq@block}{\csq@lang}{\csq@hyph}{#1}}
       {\iftoggle{csq@block}{\csq@endlang}{\csq@endhyph}}
       {\mkcitation}}}

\newrobustcmd*{\EnableQuotes}{}
\newrobustcmd*{\DisableQuotes}{}
\newrobustcmd*{\VerbatimQuotes}{}
\newrobustcmd*{\DeleteQuotes}{\csq@mkdelete}

\AtBeginDocument{%
  \protected\def\EnableQuotes{\csq@mkenable}%
  \protected\def\DisableQuotes{\csq@mkdisable}%
  \protected\def\VerbatimQuotes{\csq@mkverbatim}}

% Author interface

\newrobustcmd*{\@enablequotes}{%
  \toggletrue{csq@quiet}%
  \csq@mkenable
  \togglefalse{csq@quiet}}
\newrobustcmd*{\@disablequotes}{%
  \toggletrue{csq@quiet}%
  \csq@mkdisable
  \togglefalse{csq@quiet}}
\newrobustcmd*{\@verbatimquotes}{%
  \toggletrue{csq@quiet}%
  \csq@mkverbatim
  \togglefalse{csq@quiet}}
\newrobustcmd*{\@deletequotes}{%
  \toggletrue{csq@quiet}%
  \csq@mkdelete
  \togglefalse{csq@quiet}}

%% Switch quote styles manually

\newrobustcmd*{\setquotestyle}{%
  \@ifstar
    {\csq@resetqstyle}
    {\@ifnextchar[%]
       {\csq@setqstyle}
       {\csq@setqstyle[]}}}

\def\csq@setqstyle[#1]#2{%
  \ifnum\csq@reset>\z@
    \csq@info{Disabling multilingual quotes}%
    \csq@reset\z@
  \fi
  \ifblank{#1}
    {\DeclareQuoteAlias{#2}{default}}
    {\DeclareQuoteAlias{#2/#1}{default}}}

\def\csq@resetqstyle{%
  \csq@info{Enabling multilingual quotes}%
  \csq@reset\@ne}

\AtEndPreamble{%
  \def\csq@setqstyle[#1]#2{%
    \ifnum\csq@reset=\@ne
      \csq@info{Disabling multilingual quotes}%
      \csq@reset\z@
    \fi
    \ifblank{#1}
      {\csq@setstyle{#2}}
      {\csq@setstyle{#2/#1}}}}

%% Define quote styles

\newrobustcmd*{\DeclareQuoteStyle}[2][]{%
  \begingroup
  \let\if@safe@actives\iftrue
  \ifblank{#1}
    {\edef\csq@tempa{#2}}
    {\edef\csq@tempa{#2/#1}}%
  \ifcsundef{csq@qstyle@\csq@tempa}
    {}
    {\csq@info{Redefining quotation style '\csq@tempa'}}%
  \@ifnextchar[%]
    {\csq@declareqstyle@i}
    {\csq@declareqstyle@i[]}}

\def\csq@declareqstyle@i[#1]{%
  \csgdef{csq@qstyle@\csq@tempa}{%
    \def\csq@thequote@oinit{%
      \let\csq@themarker\csq@kernmarker#1}}%
  \@ifnextchar[%]
    {\csq@declareqstyle@ii}
    {\csq@declareqstyle@ii[]}}

\def\csq@declareqstyle@ii[#1]#2{%
  \csgappto{csq@qstyle@\csq@tempa}{%
    \def\csq@thequote@iinit{#1}%
    \def\csq@thequote@oopen{#2}}%
  \@ifnextchar[%]
    {\csq@declareqstyle@iii}
    {\csq@declareqstyle@iii[]}}

\def\csq@declareqstyle@iii[#1]#2{%
  \csgappto{csq@qstyle@\csq@tempa}{%
    \def\csq@thequote@omiddle{#1}%
    \def\csq@thequote@oclose{#2}}%
  \@ifnextchar[%]
    {\csq@declareqstyle@iv}
    {\csq@declareqstyle@iv[]}}

\def\csq@declareqstyle@iv[#1]#2{%
  \ifblank{#1}
    {\def\csq@thequote@kern{\z@}}
    {\def\csq@thequote@kern{#1}}%
  \csxappto{csq@qstyle@\csq@tempa}{%
    \def\noexpand\csq@thequote@kern{\csq@thequote@kern}}%
  \csgappto{csq@qstyle@\csq@tempa}{%
    \def\csq@thequote@iopen{#2}}%
  \@ifnextchar[%]
    {\csq@declareqstyle@v}
    {\csq@declareqstyle@v[]}}

\def\csq@declareqstyle@v[#1]#2{%
  \csgappto{csq@qstyle@\csq@tempa}{%
    \def\csq@thequote@imiddle{#1}%
    \def\csq@thequote@iclose{#2}}%
  \endgroup}

\@onlypreamble\DeclareQuoteStyle

%% Define quote aliases

\newrobustcmd*{\DeclareQuoteAlias}[3][]{%
  \begingroup
  \let\if@safe@actives\iftrue
  \ifblank{#1}
    {\edef\csq@tempa{#2}}
    {\edef\csq@tempa{#2/#1}}%
  \ifcsundef{csq@qstyle@\csq@tempa}
    {\csq@error
       {Quote style not defined}
       {Define the style or alias '\csq@tempa' first}}
    {\ifcsundef{csq@qstyle@#3}
       {}
       {\csq@info{Redefining alias '#3' -> '\csq@tempa'}}%
     \csxdef{csq@qstyle@#3}{%
       \noexpand\csuse{csq@qstyle@\csq@tempa}}}%
  \endgroup}

\@onlypreamble\DeclareQuoteAlias

%% Define quotes for PDF strings

\newrobustcmd*{\DeclarePlainStyle}[4]{%
  \def\csq@pdf@ooqmark{#1}%
  \def\csq@pdf@coqmark{#2}%
  \def\csq@pdf@oiqmark{#3}%
  \def\csq@pdf@ciqmark{#4}}

\@onlypreamble\DeclarePlainStyle

%% Define package options

\newrobustcmd*{\DeclareQuoteOption}[1]{%
  \define@key{csq}{#1}{\DeclareQuoteAlias[##1]{#1}{#1}}}

\AtEndOfPackage{%
  \protected\def\DeclareQuoteOption#1{%
    \csq@warn@location\DeclareQuoteOption}}

%% Space factor codes

\newrobustcmd*{\DeclareQuoteGlyph}[2]{%
  \csxappto{csq@sfcodes@#1}{\sfcode\detokenize{#2}=\z@}}

%% Set defaults

\newrobustcmd*{\SetBlockThreshold}[1]{%
  \csq@tshold=#1\relax}

\newrobustcmd*{\SetBlockEnvironment}[1]{%
  \ifcsundef{#1}
    {\csq@err@undef{#1}}
    {\def\csq@blockenvironment{#1}}}

\newrobustcmd*{\SetCiteCommand}[1]{%
  \ifundef#1%
    {\csq@err@undef{#1}}
    {\def\csq@cite{#1}}}

%% Interface for biblatex

\newrobustcmd*{\@setquotesfcodes}{\csq@setsfcodes}

\newcommand*{\@quotelevel}{}
\let\@quotelevel\csq@qlevel

\newcommand*{\@quotereset}{}
\let\@quotereset\csq@reset

\newcommand*{\@ifquotemarker}{%
  \ifdim\lastskip=\csq@kernmarker\relax
    \expandafter\@firstoftwo
  \else
    \expandafter\@secondoftwo
  \fi}

%% Author interface to auto quotes

\newrobustcmd*{\openautoquote}{%
  \ifbool{mmode}
    {\csq@err@mmode\openautoquote}
    {\csq@oqopen}}

\newrobustcmd*{\closeautoquote}{%
  \ifbool{mmode}
    {\csq@err@mmode\closeautoquote}
    {\csq@qclose}}

\newrobustcmd*{\openinnerquote}{%
  \ifbool{mmode}
    {\csq@err@mmode\openinnerquote}
    {\csq@iqopen}}

\newrobustcmd*{\closeinnerquote}{%
  \ifbool{mmode}
    {\csq@err@mmode\closeinnerquote}
    {\csq@qclose}}

\appto\csq@hook@hyperref{%
  \def\openautoquote{\csq@pdf@ooqmark}%
  \def\closeautoquote{\csq@pdf@coqmark}%
  \def\openinnerquote{\csq@pdf@oiqmark}%
  \def\closeinnerquote{\csq@pdf@ciqmark}}

%% Author interface to internal marks 

\newrobustcmd*{\initoquote}{%
  \csq@resetstyle
  \csq@qlevel\@ne
  \csq@init}

\newrobustcmd*{\initiquote}{%
  \csq@resetstyle
  \csq@qlevel\tw@
  \csq@init}

\newrobustcmd*{\textooquote}{%
  \csq@resetstyle
  \csq@addkern@open
  \let\csq@kernchar@i\csq@thequote@oopen
  \csq@thequote@oopen
  \csq@setmarker@open
  \csq@fixkern}

\newrobustcmd*{\textmoquote}{%
  \csq@resetstyle
  \csq@thequote@omiddle}

\newrobustcmd*{\textcoquote}{%
  \ifdim\lastkern=\csq@omitmarker
  \else
    \csq@resetstyle
    \csq@addkern@close
    \csq@thequote@oclose
    \let\csq@kernchar@i\csq@thequote@oclose
    \csq@setmarker@close
    \expandafter\csq@fixkern
  \fi}

\newrobustcmd*{\textoiquote}{%
  \csq@resetstyle
  \csq@addkern@open
  \let\csq@kernchar@i\csq@thequote@iopen
  \csq@thequote@iopen
  \csq@setmarker@open
  \csq@fixkern}

\newrobustcmd*{\textmiquote}{%
  \csq@resetstyle
  \csq@thequote@imiddle}

\newrobustcmd*{\textciquote}{%
  \ifdim\lastkern=\csq@omitmarker
  \else
    \csq@resetstyle
    \csq@addkern@close
    \csq@thequote@iclose
    \let\csq@kernchar@i\csq@thequote@iclose
    \csq@setmarker@close
    \expandafter\csq@fixkern
  \fi}

%% Ellipses

\newrobustcmd*{\textelp}{%
  \begingroup
  \@ifstar
    {\@tempswatrue\csq@textelp}
    {\@tempswafalse\csq@textelp}}

\long\def\csq@textelp#1{%
  \ifblank{#1}
    {\endgroup\mktextelp}
    {\expandafter\endgroup\if@tempswa
       \expandafter\mktextinselp
     \else
       \expandafter\mktextelpins
     \fi
     {#1}}}

\newrobustcmd*{\textins}{%
  \@ifstar\mktextmod\mktextins}

\newcommand{\mktextelp}{[\textellipsis\unkern]}
\newcommand{\mktextelpins}[1]{[\textellipsis\unkern] [#1]}
\newcommand{\mktextinselp}[1]{[#1] [\textellipsis\unkern]}
\newcommand{\mktextins}[1]{[#1]}
\newcommand{\mktextmod}[1]{[#1]}

%% Auxiliary commands for some styles

% French

\newrobustcmd*{\initfrenchquotes}{%
  \let\csq@themarker\csq@omitmarker}

\newrobustcmd*{\mkfrenchopenquote}[1]{%
  \leavevmode#1\@frenchquotespace}

\newrobustcmd*{\mkfrenchclosequote}[1]{%
  \leavevmode\@frenchquotespace#1}

\newcommand*{\@frenchquotespace}{%
  \penalty\@M
  \hskip 0.8\fontdimen2\font
   plus  0.3\fontdimen3\font
   minus 0.3\fontdimen4\font}

\AtEndPreamble{%
  \@ifpackageloaded{polyglossia}
    {\@ifpackagelater{polyglossia}{2009/11/20}
       {\let\@frenchquotespace\@empty}
       {}}
    {}}

% German

\newrobustcmd*{\fixligatures}{%
  \ifhmode
    \ifnum\spacefactor>3000
      \relax
    \else
      \ifnum\spacefactor=1007
        \relax
      \else
        \ifnum\spacefactor=1008
          \relax
        \fi
      \fi
    \fi
  \fi}

% Special styles

\DeclareQuoteStyle{debug}
  {\textbf{[\number\@quotelevel]}}
  [\textbf{[\number\@quotelevel]}]
  {\textbf{[\number\@quotelevel]}}
  {\textbf{[\number\@quotelevel]}}
  [\textbf{[\number\@quotelevel]}]
  {\textbf{[\number\@quotelevel]}}

\DeclareQuoteStyle{fallback}
  {\textbf{?}}
  {\textbf{?}}
  {\textbf{?}}
  {\textbf{?}}

%% Package options

\newrobustcmd*{\ExecuteQuoteOptions}{\setkeys{csq}}
\@onlypreamble\ExecuteQuoteOptions

% Core options

\define@key{csq}{strict}[true]{%
  \ifstrequal{#1}{true}
    {\csq@info{Enabling strict warnings}%
     \let\csq@warnorerr\csq@warning@strict}
    {\csq@info{Disabling strict warnings}%
     \let\csq@warnorerr\csq@warning@loose}}

\define@key{csq}{debug}[true]{%
  \ifstrequal{#1}{true}
    {\let\csq@debug\csq@logdebug}
    {\let\csq@debug\@gobble}}

\define@key{csq}{autopunct}[true]{%
  \ifstrequal{#1}{true}
    {\let\csq@autopunct\csq@allpunct}
    {\let\csq@autopunct\@empty}}

\define@key{csq}{style}{%
  \csq@opt@autostyle@false
  \DeclareQuoteAlias{#1}{default}}

\define@key{csq}{autostyle}[true]{%
  \ifcsdef{csq@opt@autostyle@#1}
    {\csuse{csq@opt@autostyle@#1}}
    {\csq@err@opt{autostyle=#1}}}
\def\csq@opt@autostyle@false{%
  \csq@info{Disabling multilingual quotes}%
  \csq@reset\z@}
\def\csq@opt@autostyle@true{%
  \csq@info{Enabling multilingual quotes}%
  \csq@reset\@ne}
\def\csq@opt@autostyle@try{%
  \csq@reset\tw@}
\def\csq@opt@autostyle@once{%
  \csq@reset\thr@@}
\def\csq@opt@autostyle@tryonce{%
  \csq@reset4\relax}

\define@key{csq}{babel}[true]{%
  \csq@info{%
    Option 'babel' depreciated.\MessageBreak
    Using 'autostyle'}%
  \setkeys{csq}{autostyle=#1}}

\define@key{csq}{maxlevel}{%
  \ifnumless{#1}\tw@
    {\csq@err@opt{maxlevel=#1}}
    {\csq@maxlvl#1\relax}}

\define@key{csq}{threshold}{%
  \SetBlockThreshold{#1}}

\define@key{csq}{thresholdtype}[lines]{%
  \ifcsdef{csq@bcount@#1}%
    {\def\csq@thresholdtype{#1}}
    {\csq@err@opt{thresholdtype=#1}}}

\define@key{csq}{parthreshold}[true]{%
  \settoggle{csq@parthreshold}{#1}}

\define@key{csq}{splitcomp}[true]{%
  \ifstrequal{#1}{true}
    {\let\csq@splitcomp\z@}
    {\let\csq@splitcomp\@M}}

\define@key{csq}{csdisplay}[true]{%
  \setbool{csdisplay}{#1}}

\define@key{csq}{version}{%
  \ifdef\csq@getversion
    {}
    {\input{csq-compat.def}}%
  \csq@getversion{#1}}

% Initialize

\setkeys{csq}{thresholdtype=lines,parthreshold,splitcomp=false}

%% Initial setup

% Provide 'quote' environment

\ifundef\quote
  {\csq@info{%
     The 'quote' environment appears to be undefined.\MessageBreak
     I'm defining a typical 'quote' environment now}
   \def\quote{%
     \list{}{\rightmargin\leftmargin}%
     \item\relax}
   \def\endquote{\endlist}}
  {}

% Deferred last minute setup

\AtEndPreamble{%
  \ifnumgreater\csq@reset\z@
    {\csq@info{Checking for multilingual support..}%
     \@ifpackageloaded{polyglossia}
       {\csq@info{... found 'polyglossia' package}%
	\csq@warning
	  {Using preliminary 'polyglossia' interface.\MessageBreak
           Some of the multilingual features may not\MessageBreak
	   work as expected\@gobble}%
	\def\csq@main@language{\xpg@main@language}%
	\csq@hook@multilang}
       {\@ifpackageloaded{babel}
	  {\csq@info{... found 'babel' package}%
           \def\csq@main@language{\bbl@main@language}%
           \csq@hook@multilang}
	  {\csq@info{... none found}%
           \csq@hook@nomultilang}}}
    {\@ifpackageloaded{polyglossia}
       {}
       {\@ifpackageloaded{babel}
	  {}
	  {\csq@hook@nomultilang}}}%
  \undef\csq@hook@multilang
  \undef\csq@hook@nomultilang
  \@ifpackageloaded{hyperref}
    {\expandafter\pdfstringdefDisableCommands
     \expandafter{\csq@hook@hyperref}}
    {}%
  \undef\csq@hook@hyperref
  \appto\@noligs{\@verbatimquotes}%
  \@ifpackageloaded{verbatim}
    {\addto@hook\every@verbatim{\@verbatimquotes}}
    {}%
  \@ifpackageloaded{fancyvrb}
    {\appto\FV@CatCodes{\@verbatimquotes}}
    {}%
  \@ifpackageloaded{endnotes}
    {\BlockquoteDisable{%
       \renewcommand{\endnote}[2][]{%
         \ifblank{#1}
           {\endnotemark\relax}
           {\endnotemark[#1]}}%
       \renewcommand{\endnotetext}[2][]{}%
       \let\addtoendnotes\@gobble}}
    {}%
  \ifdef\collect@body % amsmath
    {\pretocmd\collect@body{\@disablequotes}
       {}
       {\csq@err@patch{'amsmath' package}}}
    {}}

\AtBeginDocument{%
  \csq@setstyle{default}%
  \csq@mkenable}

% Restore catcodes

\csq@catcodes
\undef\csq@catcodes

% Load predefined styles

\input{csquotes.def}

% Load configuration file

\csq@info{Trying to load configuration file 'csquotes.cfg'..}
\InputIfFileExists{csquotes.cfg}
  {\csq@info{... configuration file loaded successfully}}
  {\csq@info{... configuration file not used}}

% Process options

\DeclareOption*{%
  \begingroup
  \edef\csq@tempa{\endgroup
    \noexpand\setkeys{csq}{\CurrentOption}}%
  \csq@tempa}

\ProcessOptions*

\endinput

==> etoolbox.sty.tex <==
% $Id: etoolbox.sty,v 2.1 2011/01/03 19:14:10 lehman stable $

% Copyright (c) 2007-2011 Philipp Lehman.
%
% Permission is granted to copy, distribute and/or modify this
% software under the terms of the LaTeX Project Public License
% (LPPL), version 1.3.
%
% The LPPL maintenance status of this software is
% 'author-maintained'.
%
% This software is provided 'as is', without warranty of any kind,
% either expressed or implied, including, but not limited to, the
% implied warranties of merchantability and fitness for a
% particular purpose.

\def\etb@rcsid$#1: #2 #3 #4 #5${#4 v#3}

\NeedsTeXFormat{LaTeX2e}
\ProvidesPackage{etoolbox}
[\etb@rcsid $Id: etoolbox.sty,v 2.1 2011/01/03 19:14:10 lehman stable $
 e-TeX tools for LaTeX]

\begingroup
\@ifundefined{eTeXversion}
  {\PackageError{etoolbox}
     {Not running under e-TeX}
     {This package requires e-TeX. Try compiling the document
      with\MessageBreak 'elatex' instead of 'latex'. When using
      pdfTeX, try 'pdfelatex'\MessageBreak instead of 'pdflatex'.
      This is a fatal error. I'm aborting now.}%
   \aftergroup\endinput}
  {}
\endgroup

\RequirePackage{etex}

\def\etb@catcodes{\do\&\do\|\do\:\do\-\do\=\do\<\do\>}
\def\do#1{\catcode\number`#1=\the\catcode`#1\relax}
\edef\etb@catcodes{\etb@catcodes}
\let\do\noexpand
\AtEndOfPackage{\etb@catcodes\undef\etb@catcodes}

\catcode`\&=3
\catcode`\|=3
\@makeother\:
\@makeother\-
\@makeother\=
\@makeother\<
\@makeother\>

\protected\def\etb@error{\PackageError{etoolbox}}
\protected\def\etb@warning{\PackageWarning{etoolbox}}
\protected\def\etb@info{\PackageInfo{etoolbox}}
\newcount\etb@tempcnta

% {<cstoken>}[<arguments>][<optarg default>]{<definition>}

\newcommand*{\newrobustcmd}{}
\protected\def\newrobustcmd{\@star@or@long\etb@new@command}

\def\etb@new@command#1{\@testopt{\etb@newcommand#1}0}

\def\etb@newcommand#1[#2]{%
  \@ifnextchar[%]
    {\etb@xargdef#1[#2]}
    {\ifx\l@ngrel@x\relax
       \let\l@ngrel@x\protected
     \else
       \protected\def\l@ngrel@x{\protected\long}%
     \fi
     \@argdef#1[#2]}}

\long\def\etb@xargdef#1[#2][#3]#4{%
  \@ifdefinable#1{%
    \expandafter\protected
    \expandafter\def
    \expandafter#1%
    \expandafter{%
      \expandafter\@testopt
      \csname\string#1\endcsname{#3}}%
    \expandafter\@yargdef\csname\string#1\endcsname\tw@{#2}{#4}}}

% {<cstoken>}[<arguments>][<optarg default>]{<definition>}

\newrobustcmd*{\renewrobustcmd}{\@star@or@long\etb@renew@command}

\def\etb@renew@command#1{%
  \ifundef{#1}
     {\etb@error{\string#1 undefined}\@ehc}
     {}%
  \let\@ifdefinable\@rc@ifdefinable
  \etb@new@command#1}

% {<cstoken>}[<arguments>][<optarg default>]{<definition>}

\newrobustcmd*{\providerobustcmd}{\@star@or@long\etb@provide@command}

\def\etb@provide@command#1{%
  \ifundef{#1}
    {\def\reserved@a{\etb@new@command#1}}
    {\def\reserved@a{\etb@renew@command\reserved@a}}%
  \reserved@a}

% {<csname>}

\newrobustcmd*{\csshow}[1]{%
  \begingroup\expandafter\endgroup
  \expandafter\show\csname#1\endcsname}

% {<cstoken>}{<true>}{<false>}

\newcommand{\ifdef}[1]{%
  \ifdefined#1%
    \expandafter\@firstoftwo
  \else
    \expandafter\@secondoftwo
  \fi}

% {<cstoken>}{<true>}{<false>}

\newcommand{\ifundef}[1]{%
  \ifdefined#1%
    \ifx#1\relax
      \expandafter\expandafter
      \expandafter\@firstoftwo
    \else
      \expandafter\expandafter
      \expandafter\@secondoftwo
    \fi
  \else
    \expandafter\@firstoftwo
  \fi}

% {<csname>}{<true>}{<false>}

\newcommand*{\ifcsdef}[1]{%
  \ifcsname#1\endcsname
    \expandafter\@firstoftwo
  \else
    \expandafter\@secondoftwo
  \fi}

% {<csname>}{<true>}{<false>}

\newcommand*{\ifcsundef}[1]{%
  \ifcsname#1\endcsname
    \expandafter\ifx\csname#1\endcsname\relax
      \expandafter\expandafter
      \expandafter\@firstoftwo
    \else
      \expandafter\expandafter
      \expandafter\@secondoftwo
    \fi
  \else
    \expandafter\@firstoftwo
  \fi}

% {<cstoken>}{<true}{<false>}

\newcommand{\ifdefmacro}{}
\long\edef\ifdefmacro#1{%
  \noexpand\expandafter\noexpand\etb@ifdefmacro
  \noexpand\meaning#1\detokenize{macro}:&}
\edef\etb@ifdefmacro{%
  \def\noexpand\etb@ifdefmacro##1\detokenize{macro}:##2&}
\etb@ifdefmacro{\notblank{#2}}

% {<csname>}{<true>}{<false>}

\newcommand*{\ifcsmacro}[1]{%
  \ifcsdef{#1}
    {\expandafter\ifdefmacro\csname#1\endcsname}
    {\@secondoftwo}}

% {<cstoken>}{<true}{<false>}

\newcommand{\ifdefprefix}[1]{%
  \ifdefmacro{#1}
    {\etb@ifdefprefix{#1}}
    {\@secondoftwo}}
\long\edef\etb@ifdefprefix#1{%
  \noexpand\expandafter\noexpand\etb@ifdefprefix@i
  \noexpand\meaning#1\detokenize{macro}:&}
\edef\etb@ifdefprefix@i{%
  \def\noexpand\etb@ifdefprefix@i##1\detokenize{macro}:##2&}
\etb@ifdefprefix@i{\notblank{#1}}

% {<csname>}{<true>}{<false>}

\newcommand*{\ifcsprefix}[1]{%
  \ifcsdef{#1}
    {\expandafter\ifdefprefix\csname#1\endcsname}
    {\@secondoftwo}}

% {<cstoken>}{<true}{<false>}

\newcommand{\ifdefparam}{}
\long\edef\ifdefparam#1{%
  \noexpand\expandafter\noexpand\etb@ifdefparam
  \noexpand\meaning#1\detokenize{macro}:->&}
\edef\etb@ifdefparam{%
  \def\noexpand\etb@ifdefparam##1\detokenize{macro}:##2->##3&}
\etb@ifdefparam{\notblank{#2}}

% {<csname>}{<true>}{<false>}

\newcommand*{\ifcsparam}[1]{%
  \ifcsdef{#1}
    {\expandafter\ifdefparam\csname#1\endcsname}
    {\@secondoftwo}}

% {<cstoken>}{<true}{<false>}

\newcommand{\ifdefprotected}{}
\long\edef\ifdefprotected#1{%
  \noexpand\expandafter\noexpand\etb@ifdefprotected
  \noexpand\meaning#1\string\protected&}
\edef\etb@ifdefprotected{%
  \def\noexpand\etb@ifdefprotected##1\string\protected##2&}
\etb@ifdefprotected{\notblank{#2}}

% {<csname>}{<true>}{<false>}

\newcommand*{\ifcsprotected}[1]{%
  \ifcsdef{#1}
    {\expandafter\ifdefprotected\csname#1\endcsname}
    {\@secondoftwo}}

% {<cstoken>}{<true}{<false>}

\newrobustcmd{\ifdefltxprotect}[1]{%
  \begingroup
  \edef\etb@resrvda{%
    \noexpand\protect\expandafter\noexpand
    \csname\expandafter\@gobble\string#1 \endcsname}%
  \expandafter\endgroup\ifx#1\etb@resrvda
    \expandafter\@firstoftwo
  \else
    \expandafter\@secondoftwo
  \fi}

% {<csname>}{<true>}{<false>}

\newrobustcmd*{\ifcsltxprotect}[1]{%
  \ifcsdef{#1}
    {\expandafter\ifdefltxprotect\csname#1\endcsname}
    {\@secondoftwo}}

% {<cstoken>}{<true>}{<false>}

\newcommand{\ifdefempty}[1]{%
  \ifundef{#1}
    {\@secondoftwo}
    {\ifdefmacro{#1}
       {\ifdefparam{#1}
	  {\@secondoftwo}
	  {\etb@ifdefempty{#1}}}
       {\@secondoftwo}}}

\def\etb@ifdefempty#1{%
  \expandafter\expandafter
  \expandafter\ifblank
  \expandafter\expandafter
  \expandafter{%
  \expandafter\strip@prefix\meaning#1}}

% {<csname>}{<true>}{<false>}

\newcommand*{\ifcsempty}[1]{%
  \ifcsundef{#1}
    {\@secondoftwo}
    {\expandafter\ifdefparam\csname#1\endcsname
       {\@secondoftwo}
       {\expandafter\etb@ifdefempty\csname#1\endcsname}}}

% {<cstoken>}{<true>}{<false>}

\newcommand{\ifdefvoid}[1]{%
  \ifundef{#1}
    {\@firstoftwo}
    {\ifdefmacro{#1}
       {\ifdefparam{#1}
	  {\@secondoftwo}
	  {\etb@ifdefempty{#1}}}
       {\@secondoftwo}}}

% {<csname>}{<true>}{<false>}

\newcommand*{\ifcsvoid}[1]{%
  \ifcsundef{#1}
    {\@firstoftwo}
    {\expandafter\ifdefparam\csname#1\endcsname
       {\@secondoftwo}
       {\expandafter\etb@ifdefempty\csname#1\endcsname}}}

% {<cstoken1>}{<cstoken2>}{<true>}{<false>}

\newcommand{\ifdefequal}[2]{%
  \ifundef{#1}
    {\@secondoftwo}
    {\ifundef{#2}
       {\@secondoftwo}
       {\ifx#1#2%
          \expandafter\@firstoftwo
        \else
          \expandafter\@secondoftwo
        \fi}}}

% {<csname1>}{<csname2>}{<true>}{<false>}

\newcommand*{\ifcsequal}[2]{%
  \ifcsundef{#1}
    {\@secondoftwo}
    {\ifcsundef{#2}
       {\@secondoftwo}
       {\expandafter\ifx
        \csname#1\expandafter\endcsname
        \csname#2\endcsname
          \expandafter\@firstoftwo
        \else
          \expandafter\@secondoftwo
        \fi}}}

% {<cstoken1>}{<cstoken2>}{<true>}{<false>}

\newrobustcmd{\ifdefstrequal}[2]{%
  \ifdefmacro{#1}
    {\ifdefmacro{#2}
       {\begingroup
	\edef\etb@tempa{\expandafter\strip@prefix\meaning#1}%
	\edef\etb@tempb{\expandafter\strip@prefix\meaning#2}%
	\ifx\etb@tempa\etb@tempb
	  \aftergroup\@firstoftwo
	\else
	  \aftergroup\@secondoftwo
	\fi
	\endgroup}
       {\@secondoftwo}}
    {\@secondoftwo}}

% {<csname1>}{<csname2>}{<true>}{<false>}

\newcommand*{\ifcsstrequal}[2]{%
  \ifcsundef{#1}
    {\@secondoftwo}
    {\ifcsundef{#2}
       {\@secondoftwo}
       {\expandafter\ifdefstrequal
        \csname#1\expandafter\endcsname
	\csname#2\endcsname}}}

% {<cstoken>}{<string>}{<true>}{<false>}

\newrobustcmd{\ifdefstring}[2]{%
  \ifdefmacro{#1}
    {\begingroup
     \edef\etb@tempa{\expandafter\strip@prefix\meaning#1}%
     \edef\etb@tempb{\detokenize{#2}}%
     \ifx\etb@tempa\etb@tempb
       \aftergroup\@firstoftwo
     \else
       \aftergroup\@secondoftwo
     \fi
     \endgroup}
    {\@secondoftwo}}

% {<csname>}{<string>}{<true>}{<false>}

\newrobustcmd{\ifcsstring}[2]{%
  \ifcsundef{#1}
    {\@secondoftwo}
    {\expandafter\ifdefstring\csname#1\endcsname{#2}}}

% {<cstoken>}{<true}{<false>}

\newcommand{\ifdefcounter}[1]{\etb@ifcounter#1&}
\long\def\etb@ifcounter#1#2&{%
  \ifx\count#1%
    \expandafter\@secondoftwo
  \else
    \expandafter\etb@ifcounter@i\meaning#1:%
  \fi}
\edef\etb@ifcounter@i#1:#2\fi{\noexpand\fi
  \noexpand\etb@ifcounter@ii#1\string\count&}
\edef\etb@ifcounter@ii{%
  \def\noexpand\etb@ifcounter@ii##1\string\count##2&}
\etb@ifcounter@ii{\ifblank{#1}}

% {<csname>}{<true>}{<false>}

\newcommand*{\ifcscounter}[1]{%
  \ifcsdef{#1}
    {\expandafter\ifdefcounter\csname#1\endcsname}
    {\@secondoftwo}}

% {<name>}{<true>}{<false>}

\newcommand*{\ifltxcounter}[1]{%
  \ifcsdef{c@#1}
    {\expandafter\ifdefcounter\csname c@#1\endcsname}
    {\@secondoftwo}}

% {<cstoken>}{<true}{<false>}

\newcommand{\ifdeflength}[1]{\etb@iflength#1&}
\long\def\etb@iflength#1#2&{%
  \ifx\skip#1%
    \expandafter\@secondoftwo
  \else
    \expandafter\etb@iflength@i\meaning#1:%
  \fi}
\edef\etb@iflength@i#1:#2\fi{\noexpand\fi
  \noexpand\etb@iflength@ii#1\string\skip&}
\edef\etb@iflength@ii{%
  \def\noexpand\etb@iflength@ii##1\string\skip##2&}
\etb@iflength@ii{\ifblank{#1}}

% {<csname>}{<true>}{<false>}

\newcommand*{\ifcslength}[1]{%
  \ifcsdef{#1}
    {\expandafter\ifdeflength\csname#1\endcsname}
    {\@secondoftwo}}

% {<cstoken>}{<true}{<false>}

\newcommand{\ifdefdimen}[1]{\etb@ifdimen#1&}
\long\def\etb@ifdimen#1#2&{%
  \ifx\dimen#1%
    \expandafter\@secondoftwo
  \else
    \expandafter\etb@ifdimen@i\meaning#1:%
  \fi}
\edef\etb@ifdimen@i#1:#2\fi{\noexpand\fi
  \noexpand\etb@ifdimen@ii#1\string\dimen&}
\edef\etb@ifdimen@ii{%
  \def\noexpand\etb@ifdimen@ii##1\string\dimen##2&}
\etb@ifdimen@ii{\ifblank{#1}}

% {<csname>}{<true>}{<false>}

\newcommand*{\ifcsdimen}[1]{%
  \ifcsdef{#1}
    {\expandafter\ifdefdimen\csname#1\endcsname}
    {\@secondoftwo}}

% {<string1>}{<string2>}{<true>}{<false>}

\newrobustcmd{\ifstrequal}[2]{%
  \begingroup
  \edef\etb@tempa{\detokenize{#1}}%
  \edef\etb@tempb{\detokenize{#2}}%
  \ifx\etb@tempa\etb@tempb
    \aftergroup\@firstoftwo
  \else
    \aftergroup\@secondoftwo
  \fi
  \endgroup}

% {<string>}{<true>}{<false>}

\newcommand{\ifstrempty}[1]{%
  \expandafter\ifx\expandafter&\detokenize{#1}&%
    \expandafter\@firstoftwo
  \else
    \expandafter\@secondoftwo
  \fi}

% {<string>}{<true>}{<false>}

\newcommand{\ifblank}[1]{% from url.sty
  \etb@ifblank@i#1&&\@secondoftwo\@firstoftwo:}
\long\def\etb@ifblank@i#1#2&#3#4#5:{#4}

\newcommand{\notblank}[1]{%
  \etb@ifblank@i#1&&\@firstoftwo\@secondoftwo:}

% {<numexpr>}{<comp>}{<numexpr>}{<true>}{<false>}

\newcommand*{\ifnumcomp}[3]{%
  \ifnum\numexpr#1\relax#2\numexpr#3\relax
    \expandafter\@firstoftwo
  \else
    \expandafter\@secondoftwo
  \fi}

% {<numexpr>}{<numexpr>}{<true>}{<false>}

\newcommand*{\ifnumequal}[1]{%
  \ifnumcomp{#1}=}

\newcommand*{\ifnumgreater}[1]{%
  \ifnumcomp{#1}>}

\newcommand*{\ifnumless}[1]{%
  \ifnumcomp{#1}<}

% {<numexpr>}{<true>}{<false>}

\newcommand*{\ifnumodd}[1]{%
  \ifodd\numexpr#1\relax
    \expandafter\@firstoftwo
  \else
    \expandafter\@secondoftwo
  \fi}

% {<dimexpr>}{<comp>}{<dimexpr>}{<true>}{<false>}

\newcommand*{\ifdimcomp}[3]{%
  \ifdim\dimexpr#1\relax#2\dimexpr#3\relax
    \expandafter\@firstoftwo
  \else
    \expandafter\@secondoftwo
  \fi}

% {<dimexpr>}{<dimexpr>}{<true>}{<false>}

\newcommand*{\ifdimequal}[1]{%
  \ifdimcomp{#1}=}

\newcommand*{\ifdimgreater}[1]{%
  \ifdimcomp{#1}>}

\newcommand*{\ifdimless}[1]{%
  \ifdimcomp{#1}<}

% {<expr>}{<true>}{<false>}

\newcommand{\ifboolexpe}[1]{%
  \etb@be@beg\etb@be@bgroup#1(&\etb@be@end}

\let\etb@be@true\@empty
\def\etb@be@false{-\@ne}

\def\etb@be@beg{%
  \ifnum\numexpr\z@\ifnum\numexpr\z@}

\def\etb@be@end{%
  <\z@
    \expandafter\etb@be@false
  \fi
  <\z@
    \expandafter\@secondoftwo
  \else
    \expandafter\@firstoftwo
  \fi}

\long\def\etb@be@bgroup#1(#2&{%
  \etb@be@egroup#1)&%
  \ifblank{#2}
    {}
    {\etb@be@beg
     \etb@be@bgroup#2&}}

\long\def\etb@be@egroup#1)#2&{%
  \etb@be@and#1and&%
  \ifblank{#2}
    {}
    {\etb@be@end\etb@be@true\etb@be@false
     \etb@be@egroup#2&}}

\long\def\etb@be@and#1and#2&{%
  \etb@be@or#1or&%
  \ifblank{#2}
    {}
    {<\z@
       \expandafter\@firstofone
     \else
       \expandafter\@gobble
     \fi
     {=\z@\fi\ifnum\numexpr\m@ne}%
     \ifnum\numexpr\z@
     \etb@be@and#2&}}

\long\def\etb@be@or#1or#2&{%
  \etb@be@not#1not&%
  \ifblank{#2}
    {}
    {<\z@
       \expandafter\@secondoftwo
     \else
       \expandafter\@firstoftwo
     \fi
     {=\z@\fi\ifnum\numexpr\z@
      \ifnum\numexpr\@ne}
     {=\z@\fi\ifnum\numexpr\z@
      \ifnum\numexpr\z@}%
     \etb@be@or#2&}}

\long\def\etb@be@not#1not#2&{%
  \etb@be@togl#1togl&%
  \ifblank{#2}
    {}
    {>\z@
       \expandafter\@firstoftwo
     \else
       \expandafter\@secondoftwo
     \fi
     {\unless\ifnum\numexpr\m@ne}
     {\unless\ifnum\numexpr\z@}%
     \etb@be@not#2&}}

\long\def\etb@be@togl#1togl#2&{%
  \etb@be@bool#1bool&%
  \ifblank{#2}
    {}
    {\etb@be@togl@i#2&}}

\long\def\etb@be@togl@i#1#2&{%
  \ifcsdef{etb@tgl@#1}
    {\csname etb@tgl@#1\endcsname\etb@be@true\etb@be@false}
    {\etb@be@err{Toggle '#1' undefined}{}}%
  \etb@be@togl#2&}

\long\def\etb@be@bool#1bool#2&{%
  \etb@be@test#1test&%
  \ifblank{#2}
    {}
    {\etb@be@bool@i#2&}}

\long\def\etb@be@bool@i#1#2&{%
  \ifcsundef{if#1}
    {\etb@be@err{Boolean '#1' undefined}{}}
    {\csname if#1\endcsname
     \else
       \etb@be@false
     \fi}%
  \etb@be@bool#2&}

\long\def\etb@be@test#1test#2&{%
  \ifblank{#1}
    {}
    {\etb@be@err{The invalid part is: '\detokenize{#1}'}{}}%
  \ifblank{#2}
    {}
    {\etb@be@test@i#2&}}

\long\def\etb@be@test@i#1#2&{%
  #1\etb@be@true\etb@be@false
  \etb@be@test#2&}

\long\def\etb@be@err#1#2{%
  \expandafter\ifnum\the\numexpr
    \expandafter\ifnum\the\currentiftype=-3
      \expandafter\thr@@
    \else
      \expandafter\currentiftype
    \fi
  =\thr@@
    \expandafter\@firstoftwo
  \else
    \expandafter\@secondoftwo
  \fi
  {=\z@\fi
   \etb@be@err{#1}{#2\ifnum\numexpr\m@ne}}
  {\etb@err@expr{#1}#2}}

% {<expr>}{<true>}{<false>}

\newrobustcmd{\ifboolexpr}[1]{\etb@boolexpr{#1}}

\long\def\etb@boolexpr#1{%
  \begingroup
  \let\etb@br@neg\@firstoftwo
  \etb@tempcnta\z@
  \etb@br@beg
  \etb@br@bgroup#1(&%
  \etb@br@end
  \etb@br@eval}

\def\etb@br@beg{%
  \begingroup
  \let\etb@br@neg\@firstoftwo
  \etb@tempcnta\z@}

\def\etb@br@end{%
  \etb@br@eval\etb@br@true\etb@br@false}

\def\etb@br@eval{%
  \ifnum\etb@tempcnta<\z@
    \aftergroup\@secondoftwo
  \else
    \aftergroup\@firstoftwo
  \fi
  \endgroup}

\def\etb@br@true{%
  \advance\etb@tempcnta\etb@br@neg\z@\m@ne
  \let\etb@br@neg\@firstoftwo}

\def\etb@br@false{%
  \advance\etb@tempcnta\etb@br@neg\m@ne\z@
  \let\etb@br@neg\@firstoftwo}

\long\def\etb@br@bgroup#1(#2&{%
  \etb@br@egroup#1)&%
  \ifblank{#2}
    {}
    {\etb@br@beg
     \etb@br@bgroup#2&}}

\long\def\etb@br@egroup#1)#2&{%
  \etb@br@and#1and&%
  \ifblank{#2}
    {}
    {\etb@br@end
     \etb@br@egroup#2&}}

\long\def\etb@br@and#1and#2&{%
  \etb@br@or#1or&%
  \ifblank{#2}
    {}
    {\ifnum\etb@tempcnta<\z@
       \etb@tempcnta\m@ne
     \else
       \etb@tempcnta\z@
     \fi
     \etb@br@and#2&}}

\long\def\etb@br@or#1or#2&{%
  \etb@br@not#1not&%
  \ifblank{#2}
    {}
    {\ifnum\etb@tempcnta<\z@
       \etb@tempcnta\z@
     \else
       \etb@tempcnta\@ne
     \fi
     \etb@br@or#2&}}

\long\def\etb@br@not#1not#2&{%
  \etb@br@togl#1togl&%
  \ifblank{#2}
    {}
    {\let\etb@br@neg\@secondoftwo
     \etb@br@not#2&}}

\long\def\etb@br@togl#1togl#2&{%
  \etb@br@bool#1bool&%
  \ifblank{#2}
    {}
    {\etb@br@togl@i#2&}}

\long\def\etb@br@togl@i#1#2&{%
  \ifcsdef{etb@tgl@#1}
    {\csname etb@tgl@#1\endcsname\etb@br@true\etb@br@false}
    {\etb@err@expr{Toggle '#1' undefined}\etb@br@false}%
  \etb@br@togl#2&}

\long\def\etb@br@bool#1bool#2&{%
  \etb@br@test#1test&%
  \ifblank{#2}
    {}
    {\etb@br@bool@i#2&}}

\long\def\etb@br@bool@i#1#2&{%
  \ifcsundef{if#1}
    {\etb@err@expr{Boolean '#1' undefined}\etb@br@false}
    {\csname if#1\endcsname
       \etb@br@true
     \else
       \etb@br@false
     \fi}%
  \etb@br@bool#2&}

\long\def\etb@br@test#1test#2&{%
  \ifblank{#1}
    {}
    {\etb@err@expr{The invalid part is: '\detokenize{#1}'}}%
  \ifblank{#2}
    {}
    {\etb@br@test@i#2&}}

\long\def\etb@br@test@i#1#2&{%
  \ignorespaces#1\etb@br@true\etb@br@false
  \etb@br@test#2&}

\long\def\etb@err@expr#1{%
  \etb@error
    {Invalid boolean expression}
    {#1.}}

% {<expr>}{<code>}

\newrobustcmd{\whileboolexpr}[2]{%
  \etb@boolexpr{#1}{#2\whileboolexpr{#1}{#2}}{}}

% {<expr>}{<code>}

\newrobustcmd{\unlessboolexpr}[2]{%
  \etb@boolexpr{#1}{}{#2\unlessboolexpr{#1}{#2}}}

% {<cstoken>}

\newcommand{\expandonce}[1]{%
  \unexpanded\expandafter{#1}}

% {<csname>}

\newcommand*{\csexpandonce}[1]{%
  \expandafter\expandonce\csname#1\endcsname}

% {<code>}

\newcommand*{\protecting}{}
\def\protecting#{%
  \ifx\protect\@typeset@protect
    \etb@protecting\@firstofone
  \fi
  \ifx\protect\@unexpandable@protect
    \etb@protecting\etb@unexpandable
  \fi
  \ifx\protect\noexpand
    \etb@protecting\unexpanded
  \fi
  \ifx\protect\string
    \etb@protecting\detokenize
  \fi
  \relax\@firstofone}

\def\etb@protecting#1#2\relax\@firstofone{\fi#1}
\long\def\etb@unexpandable#1{\unexpanded{\protecting{#1}}}

% {<csname>}

\newrobustcmd*{\csdef}[1]{\expandafter\def\csname#1\endcsname}
\newrobustcmd*{\csedef}[1]{\expandafter\edef\csname#1\endcsname}
\newrobustcmd*{\csgdef}[1]{\expandafter\gdef\csname#1\endcsname}
\newrobustcmd*{\csxdef}[1]{\expandafter\xdef\csname#1\endcsname}
\newrobustcmd*{\protected@csedef}{\etb@protected\csedef}
\newrobustcmd*{\protected@csxdef}{\etb@protected\csxdef}

\def\etb@protected{%
  \let\@@protect\protect
  \let\protect\@unexpandable@protect
  \afterassignment\restore@protect}

% {<csname>}{<cstoken>}

\newrobustcmd{\cslet}[2]{%
  \expandafter\let\csname#1\endcsname#2}

% {<cstoken>}{<csname>}

\newrobustcmd{\letcs}[2]{%
  \ifcsdef{#2}
    {\expandafter\let\expandafter#1\csname#2\endcsname}
    {\undef#1}}

% {<csname>}{<csname>}

\newrobustcmd*{\csletcs}[2]{%
  \ifcsdef{#2}
    {\expandafter\let
     \csname#1\expandafter\endcsname
     \csname#2\endcsname}
    {\csundef{#1}}}

% {<csname>}

\newcommand*{\csuse}[1]{%
  \ifcsname#1\endcsname
    \csname#1\expandafter\endcsname
  \fi}

% {<cstoken>}

\newrobustcmd{\undef}[1]{\let#1\etb@undefined}

% {<csname>}

\newrobustcmd*{\csundef}[1]{\cslet{#1}\etb@undefined}

% {<cstoken>}{<code>}

\newrobustcmd{\appto}[2]{%
  \ifundef{#1}
    {\edef#1{\unexpanded{#2}}}
    {\edef#1{\expandonce#1\unexpanded{#2}}}}
\newrobustcmd{\eappto}[2]{%
  \ifundef{#1}
    {\edef#1{#2}}
    {\edef#1{\expandonce#1#2}}}
\newrobustcmd{\gappto}[2]{%
  \ifundef{#1}
    {\xdef#1{\unexpanded{#2}}}
    {\xdef#1{\expandonce#1\unexpanded{#2}}}}
\newrobustcmd{\xappto}[2]{%
  \ifundef{#1}
    {\xdef#1{#2}}
    {\xdef#1{\expandonce#1#2}}}

\newrobustcmd*{\protected@eappto}{\etb@protected\eappto}
\newrobustcmd*{\protected@xappto}{\etb@protected\xappto}

% {<cstoken>}{<code>}

\newrobustcmd{\preto}[2]{%
  \ifundef{#1}
    {\edef#1{\unexpanded{#2}}}
    {\edef#1{\unexpanded{#2}\expandonce#1}}}
\newrobustcmd{\epreto}[2]{%
  \ifundef{#1}
    {\edef#1{#2}}
    {\edef#1{#2\expandonce#1}}}
\newrobustcmd{\gpreto}[2]{%
  \ifundef{#1}
    {\xdef#1{\unexpanded{#2}}}
    {\xdef#1{\unexpanded{#2}\expandonce#1}}}
\newrobustcmd{\xpreto}[2]{%
  \ifundef{#1}
    {\xdef#1{#2}}
    {\xdef#1{#2\expandonce#1}}}

\newrobustcmd*{\protected@epreto}{\etb@protected\epreto}
\newrobustcmd*{\protected@xpreto}{\etb@protected\xpreto}

% {<csname>}{<code>}

\newrobustcmd*{\csappto}[1]{\expandafter\appto\csname#1\endcsname}
\newrobustcmd*{\cseappto}[1]{\expandafter\eappto\csname#1\endcsname}
\newrobustcmd*{\csgappto}[1]{\expandafter\gappto\csname#1\endcsname}
\newrobustcmd*{\csxappto}[1]{\expandafter\xappto\csname#1\endcsname}
\newrobustcmd*{\protected@cseappto}{\etb@protected\cseappto}
\newrobustcmd*{\protected@csxappto}{\etb@protected\csxappto}

% {<csname>}{<code>}

\newrobustcmd*{\cspreto}[1]{\expandafter\preto\csname#1\endcsname}
\newrobustcmd*{\csepreto}[1]{\expandafter\epreto\csname#1\endcsname}
\newrobustcmd*{\csgpreto}[1]{\expandafter\gpreto\csname#1\endcsname}
\newrobustcmd*{\csxpreto}[1]{\expandafter\xpreto\csname#1\endcsname}
\newrobustcmd*{\protected@csepreto}{\etb@protected\csepreto}
\newrobustcmd*{\protected@csxpreto}{\etb@protected\csxpreto}

% {<cstoken>}{<numexpr>}

\newrobustcmd*{\numdef}[2]{%
  \ifundef#1{\let#1\z@}{}%
  \edef#1{\the\numexpr#2}}
\newrobustcmd*{\numgdef}[2]{%
  \ifundef#1{\let#1\z@}{}%
  \xdef#1{\the\numexpr#2}}

% {<csname>}{<numexpr>}

\newrobustcmd*{\csnumdef}[1]{%
  \expandafter\numdef\csname#1\endcsname}
\newrobustcmd*{\csnumgdef}[1]{%
  \expandafter\numgdef\csname#1\endcsname}

% {<cstoken>}{<dimexpr>}

\newrobustcmd*{\dimdef}[2]{%
  \ifundef#1{\let#1\z@}{}%
  \edef#1{\the\dimexpr#2}}
\newrobustcmd*{\dimgdef}[2]{%
  \ifundef#1{\let#1\z@}{}%
  \xdef#1{\the\dimexpr#2}}

% {<csname>}{<dimexpr>}

\newrobustcmd*{\csdimdef}[1]{%
  \expandafter\dimdef\csname#1\endcsname}
\newrobustcmd*{\csdimgdef}[1]{%
  \expandafter\dimgdef\csname#1\endcsname}

% {<cstoken>}{<glueexpr>}

\newrobustcmd*{\gluedef}[2]{%
  \ifundef#1{\let#1\z@skip}{}%
  \edef#1{\the\glueexpr#2}}
\newrobustcmd*{\gluegdef}[2]{%
  \ifundef#1{\let#1\z@skip}{}%
  \xdef#1{\the\glueexpr#2}}

% {<csname>}{<glueexpr>}

\newrobustcmd*{\csgluedef}[1]{%
  \expandafter\gluedef\csname#1\endcsname}
\newrobustcmd*{\csgluegdef}[1]{%
  \expandafter\gluegdef\csname#1\endcsname}

% {<cstoken>}{<muexpr>}

\newrobustcmd*{\mudef}[2]{%
  \ifundef#1{\def#1{0mu}}{}%
  \edef#1{\the\muexpr#2}}
\newrobustcmd*{\mugdef}[2]{%
  \ifundef#1{\let#1\z@}{}%
  \xdef#1{\the\muexpr#2}}

% {<csname>}{<muexpr>}

\newrobustcmd*{\csmudef}[1]{%
  \expandafter\mudef\csname#1\endcsname}
\newrobustcmd*{\csmugdef}[1]{%
  \expandafter\mugdef\csname#1\endcsname}

% {<counter>}{<numexpr>}

\newrobustcmd*{\defcounter}[2]{%
  \ifcsundef{c@#1}
    {\etb@noglobal\@nocounterr{#1}}%
    {\csname c@#1\endcsname\numexpr#2\relax}}

% {<length>}{<glueexpr>}

\newrobustcmd*{\deflength}[2]{%
  \ifundef{#1}
    {\etb@noglobal\etb@err@nolen{#1}}%
    {#1\glueexpr#2\relax}}

\protected\def\etb@err@nolen#1{%
  \etb@error{Length '\string#1' undefined}\@eha}

% {<name>}

\newrobustcmd*{\newbool}[1]{%
  \expandafter\@ifdefinable\csname if#1\endcsname{%
    \expandafter\newif\csname if#1\endcsname}}

% {<name>}

\newrobustcmd*{\providebool}[1]{%
  \ifcsundef{if#1}
    {\expandafter\newif\csname if#1\endcsname}
    {\begingroup
     \edef\@tempa{\expandafter\meaning\csname if#1\endcsname}%
     \ifx\@tempa\etb@isfalse
     \else
       \ifx\@tempa\etb@istrue
       \else
         \etb@error{\@backslashchar if#1 not a boolean}\@eha
       \fi
     \fi
     \endgroup}}

% {<name>}{<true>|<false>}

\newrobustcmd*{\setbool}[2]{%
  \ifcsundef{if#1}
    {\etb@noglobal\etb@err@nobool{#1}}
    {\ifcsundef{#1#2}
       {\etb@noglobal\etb@err@boolval{#2}}
       {\csname#1#2\endcsname}}}

% {<name>}

\newrobustcmd*{\booltrue}[1]{%
  \ifcsundef{if#1}
    {\etb@noglobal\etb@err@nobool{#1}}
    {\csname#1true\endcsname}}

% {<name>}

\newrobustcmd*{\boolfalse}[1]{%
  \ifcsundef{if#1}
    {\etb@noglobal\etb@err@nobool{#1}}
    {\csname#1false\endcsname}}

\edef\etb@istrue{\meaning\iftrue}
\edef\etb@isfalse{\meaning\iffalse}
\protected\def\etb@noglobal{\let\relax\relax}

% {<name>}{<true}{<false>}

\newcommand*{\ifbool}[1]{%
  \ifcsundef{if#1}
    {\etb@err@nobool{#1}\@gobbletwo}
    {\csname if#1\endcsname
       \expandafter\@firstoftwo
     \else
       \expandafter\@secondoftwo
     \fi}}

% {<name>}{<not true}{<not false>}

\newcommand*{\notbool}[1]{%
  \ifcsundef{if#1}
    {\etb@err@nobool{#1}\@gobbletwo}
    {\csname if#1\endcsname
       \expandafter\@secondoftwo
     \else
       \expandafter\@firstoftwo
     \fi}}

\protected\def\etb@err@nobool#1{%
  \etb@error{Boolean '\@backslashchar if#1' undefined}\@eha}

\def\etb@err@boolval#1{%
  \etb@error
    {Invalid boolean value '#1'}
    {Valid boolean values are 'true' and 'false'.}}

% {<name>}

\newrobustcmd*{\newtoggle}[1]{%
  \ifcsdef{etb@tgl@#1}
    {\etb@error{Toggle '#1' already defined}\@eha}
    {\cslet{etb@tgl@#1}\@secondoftwo}}

% {<name>}

\newrobustcmd*{\providetoggle}[1]{%
  \ifcsdef{etb@tgl@#1}
    {}
    {\cslet{etb@tgl@#1}\@secondoftwo}}

% {<name>}{<true>|<false>}

\newrobustcmd*{\settoggle}[2]{%
  \ifcsdef{etb@tgl@#1}
    {\ifcsdef{etb@toggle#2}
       {\csletcs{etb@tgl@#1}{etb@toggle#2}}
       {\etb@noglobal\etb@err@boolval{#2}}}
    {\etb@noglobal\etb@err@notoggle{#1}}}

% {<name>}

\newrobustcmd*{\toggletrue}[1]{%
  \ifcsdef{etb@tgl@#1}
    {\cslet{etb@tgl@#1}\etb@toggletrue}
    {\etb@noglobal\etb@err@notoggle{#1}}}

% {<name>}

\newrobustcmd*{\togglefalse}[1]{%
  \ifcsdef{etb@tgl@#1}
    {\cslet{etb@tgl@#1}\etb@togglefalse}
    {\etb@noglobal\etb@err@notoggle{#1}}}

\let\etb@toggletrue\@firstoftwo
\let\etb@togglefalse\@secondoftwo

% {<name>}{<true}{<false>}

\newcommand*{\iftoggle}[1]{%
  \ifcsdef{etb@tgl@#1}
    {\csname etb@tgl@#1\endcsname}
    {\etb@err@notoggle{#1}\@gobbletwo}}

% {<name>}{<not true}{<not false>}

\newcommand*{\nottoggle}[1]{%
  \ifcsdef{etb@tgl@#1}
    {\csname etb@tgl@#1\endcsname\@secondoftwo\@firstoftwo}
    {\etb@err@notoggle{#1}\@gobbletwo}}

\protected\def\etb@err@notoggle#1{%
  \etb@error{Toggle '#1' undefined}\@eha}

% {<cstoken>}{<true}{<false>}

\protected\def\etb@ifscanable#1{%
  \begingroup
  \edef\etb@resrvda{%
    \def\noexpand\etb@resrvda####1\detokenize{macro}:####2->####3&{%
      ####1\def\string\etb@resrvda####2{####3}}%
    \edef\noexpand\etb@resrvda{\noexpand\etb@resrvda\meaning#1&}}%
  \etb@resrvda
  \makeatletter
  \scantokens\expandafter{\etb@resrvda}%
  \expandafter\endgroup\ifx#1\etb@resrvda
    \expandafter\@firstoftwo
  \else
    \expandafter\@secondoftwo
  \fi}

% {<cstoken>}{<search>}{<true}{<false>}

\protected\long\def\etb@ifpattern#1#2{%
  \begingroup
  \edef\etb@resrvda{%
    \def\noexpand\etb@resrvda####1\detokenize{#2}####2&{%
      \endgroup\noexpand\noexpand\noexpand\ifblank{####2}}%
    \edef\noexpand\etb@resrvda{\noexpand\etb@resrvda
      \expandafter\strip@prefix\meaning#1\detokenize{#2}&}%
    \noexpand\etb@resrvda}
  \etb@resrvda\@secondoftwo\@firstoftwo}

% {<string>}{<true}{<false>}

\protected\long\def\etb@ifhashcheck#1{%
  \begingroup
  \edef\etb@resrvda{\detokenize{#1}}%
  \expandafter\endgroup
  \expandafter\etb@ifhashcheck@i\meaning\etb@resrvda&}

\edef\etb@ifhashcheck@i#1&{%
  \noexpand\expandafter
  \noexpand\etb@ifhashcheck@ii
  \noexpand\strip@prefix#1\string#\string#&}

\edef\etb@ifhashcheck@ii{%
  \def\noexpand\etb@ifhashcheck@ii##1\string#\string###2&}
\etb@ifhashcheck@ii{\ifblank{#2}}

% {<cstoken>}

\newrobustcmd*{\robustify}[1]{%
  \ifundef{#1}
    {\etb@error{\string#1 undefined}\@eha}
    {\ifdefmacro{#1}
       {\ifdefltxprotect{#1}
          {\letcs\etb@resrvda{\expandafter\@gobble\string#1 }%
           \@tempswatrue}
          {\let\etb@resrvda#1%
           \@tempswafalse}%
        \ifdefparam\etb@resrvda
          {\etb@ifscanable\etb@resrvda
             {\etb@robustify\etb@resrvda
              \let#1\etb@resrvda}
             {\etb@error{Failed to robustify \string#1}
                {The command is special and cannot be
                 handled by \string\robustify.}%
              \@tempswafalse}}
          {\protected\edef#1{\expandonce\etb@resrvda}}
        \if@tempswa
          \ifcsdef{\string#1 }
            {}
            {\csundef{\expandafter\@gobble\string#1 }}%
        \fi
        \undef\etb@resrvda}
       {\etb@error{\string#1 not a macro}\@eha}}}

\def\etb@robustify#1{%
  \begingroup
  \edef\etb@resrvdb{%
    \def\noexpand\etb@resrvdb####1\detokenize{macro}:####2->####3&{%
      \protected####1\def\string#1\space####2{####3}}%
    \edef\noexpand\etb@resrvdb{%
      \noexpand\etb@resrvdb\meaning#1&}}%
  \etb@resrvdb
  \etb@patchcmd@scantoks\etb@resrvdb}

%  {<cstoken>}{<search>}{<true}{<false>}
% *{<cstoken>}{<true}{<false>}

\newrobustcmd{\ifpatchable}{%
  \etb@dbg@trce\ifpatchable
  \begingroup
  \@makeother\#%
  \@ifstar\etb@ifpatchable@i\etb@ifpatchable}

\long\def\etb@ifpatchable#1#2{%
  \endgroup
  \etb@dbg@init#1%
  \ifundef{#1}
    {\etb@dbg@fail{def}\@secondoftwo}
    {\etb@dbg@info{def}%
     \ifdefmacro{#1}
       {\etb@dbg@info{mac}%
        \etb@ifscanable{#1}
          {\etb@ifhashcheck{#2}
             {\etb@dbg@info{tok}%
              \etb@ifpattern#1{#2}
                 {\etb@dbg@info{pat}%
                  \etb@dbg@info{pos}\@firstoftwo}
                 {\etb@dbg@fail{pat}\@secondoftwo}}
             {\etb@dbg@fail{hsh}\@secondoftwo}}
          {\etb@dbg@fail{tok}\@secondoftwo}}
       {\etb@dbg@fail{mac}\@secondoftwo}}}

\long\def\etb@ifpatchable@i#1{%
  \endgroup
  \etb@dbg@init#1%
  \ifundef{#1}
    {\etb@dbg@fail{def}\@secondoftwo}
    {\etb@dbg@info{def}%
     \ifdefmacro{#1}
       {\etb@dbg@info{mac}%
        \ifdefparam{#1}
          {\etb@dbg@info{prm}%
           \etb@ifscanable{#1}
             {\etb@dbg@info{tok}%
              \etb@dbg@info{pos}\@firstoftwo}
             {\etb@dbg@fail{tok}\@secondoftwo}}
          {\etb@dbg@info{prl}%
           \ifdefprotected{#1}
             {\etb@dbg@info{pro}}
             {}%
           \etb@dbg@info{pos}\@firstoftwo}}
       {\etb@dbg@fail{mac}\@secondoftwo}}}

% [<prefix>]{<cstoken>}{<search>}{<replace>}{<success>}{<failure>}

\newrobustcmd*{\patchcmd}{%
  \etb@dbg@trce\patchcmd
  \begingroup
  \@makeother\#%
  \etb@patchcmd}

\newcommand{\etb@patchcmd}[4][########1]{%
  \etb@ifpatchable#2{#3}
    {\etb@dbg@succ{ret}%
     \begingroup
     \edef\etb@resrvda{%
       \def\noexpand\etb@resrvda####1\detokenize{macro:}####2->####3&{%
         #1\def\string\etb@resrvda\space####2{\noexpand\etb@resrvdb####3&}}%
       \def\noexpand\etb@resrvdb####1\detokenize{#3}####2&{%
         ####1\detokenize{#4}####2}%
       \edef\noexpand\etb@resrvda{%
         \noexpand\etb@resrvda\meaning#2&}}%
     \etb@resrvda
     \etb@patchcmd@scantoks\etb@resrvda
     \let#2\etb@resrvda
     \undef\etb@resrvda
     \@firstoftwo}
    {\@secondoftwo}}

\def\etb@patchcmd@scantoks#1{%
  \edef\etb@resrvda{\endgroup
    \unexpanded{\makeatletter\scantokens}{#1}%
    \catcode\number`\@=\the\catcode`\@\relax}%
  \etb@resrvda}

% {<cstoken>}{<code>}{<success>}{<failure>}

\newrobustcmd*{\apptocmd}{%
  \etb@dbg@trce\apptocmd
  \begingroup
  \@makeother\#%
  \etb@hooktocmd\etb@append}

\newrobustcmd*{\pretocmd}{%
  \etb@dbg@trce\pretocmd
  \begingroup
  \@makeother\#%
  \etb@hooktocmd\etb@prepend}

\long\def\etb@hooktocmd#1#2#3{%
  \endgroup
  \etb@dbg@init#2%
  \ifundef{#2}
    {\etb@dbg@fail{def}\@secondoftwo}
    {\etb@dbg@info{def}%
     \ifdefmacro{#2}
       {\etb@dbg@info{mac}%
        \ifdefparam{#2}
          {\etb@dbg@info{prm}%
           \etb@ifscanable{#2}
             {\etb@ifhashcheck{#3}
                {\etb@dbg@info{tok}%
                 \etb@dbg@succ{ret}%
                 \etb@hooktocmd@i#1#2{#3}%
                 \@firstoftwo}
                {\etb@dbg@fail{hsh}\@secondoftwo}}
             {\etb@dbg@fail{tok}\@secondoftwo}}
          {\etb@dbg@info{prl}%
           \ifdefprotected{#2}
             {\etb@dbg@info{pro}%
              \etb@dbg@succ{red}%
              \protected}
             {\etb@dbg@succ{red}}%
           \edef#2{#1{\expandonce#2}{\unexpanded{#3}}}%
           \@firstoftwo}}
       {\etb@dbg@fail{mac}\@secondoftwo}}}

\long\def\etb@hooktocmd@i#1#2#3{%
  \begingroup
  \edef\etb@resrvda{%
    \def\noexpand\etb@resrvda####1\detokenize{macro}:####2->####3&{%
      ####1\def\string\etb@resrvda\space####2{#1{####3}{\detokenize{#3}}}}%
    \edef\noexpand\etb@resrvda{%
      \noexpand\etb@resrvda\meaning#2&}}%
  \etb@resrvda
  \etb@patchcmd@scantoks\etb@resrvda
  \let#2\etb@resrvda
  \undef\etb@resrvda}

\long\def\etb@append#1#2{#1#2}
\long\def\etb@prepend#1#2{#2#1}

\newrobustcmd*{\tracingpatches}{%
  \etb@info{Enabling tracing}%
  \input{etoolbox.def}%
  \global\let\tracingpatches\relax}
\@onlypreamble\tracingpatches

\let\etb@dbg@trce\@gobble
\let\etb@dbg@init\@gobble
\let\etb@dbg@info\@gobble
\let\etb@dbg@succ\@gobble
\let\etb@dbg@fail\@gobble

% {<numeral>}

\newcommand{\rmntonum}[1]{%
  \ifblank{#1}
    {}
    {\expandafter\etb@rti@end\number\numexpr
     \expandafter\etb@rti@prs\detokenize{#1}&\relax}}

\def\etb@rti@prs#1#2{%
  \ifx&#1%
    \expandafter\@firstoftwo
  \else
    \expandafter\@secondoftwo
  \fi
  {#1#2}
  {\ifx&#2%
     \expandafter\@firstoftwo
   \else
     \expandafter\@secondoftwo
   \fi
   {\etb@rti@chk#1+\etb@rti@num#1#2}
   {\etb@rti@chk#1\etb@rti@chk#2%
    \ifnum\etb@rti@num#1<\etb@rti@num#2 %
      \expandafter\@firstoftwo
    \else
      \expandafter\@secondoftwo
    \fi
    {+\etb@rti@num#2-\etb@rti@num#1\etb@rti@prs}
    {+\etb@rti@num#1\etb@rti@prs#2}}}}

\def\etb@rti@chk#1{%
  \ifcsname etb@rmn@#1\endcsname
  \else
    \expandafter\etb@rti@brk
  \fi}

\def\etb@rti@brk#1&{+\z@&-1}
\def\etb@rti@end#1&#2\relax{\ifblank{#2}{#1}{#2}}
\def\etb@rti@num#1{\csname etb@rmn@#1\endcsname}

\chardef\etb@rmn@i=1
\chardef\etb@rmn@I=1
\chardef\etb@rmn@v=5
\chardef\etb@rmn@V=5
\chardef\etb@rmn@x=10
\chardef\etb@rmn@X=10
\chardef\etb@rmn@l=50
\chardef\etb@rmn@L=50
\chardef\etb@rmn@c=100
\chardef\etb@rmn@C=100
\mathchardef\etb@rmn@d=500
\mathchardef\etb@rmn@D=500
\mathchardef\etb@rmn@m=1000
\mathchardef\etb@rmn@M=1000

% {<numeral>}{<true>}{<false>}

\newcommand{\ifrmnum}[1]{%
  \ifblank{#1}
    {\@secondoftwo}
    {\expandafter\etb@ifr@prs\detokenize{#1}\relax}}

\def\etb@ifr@prs#1{%
  \ifx\relax#1%
    \expandafter\@firstoftwo
  \else
    \ifcsname etb@rmn@#1\endcsname
      \expandafter\expandafter
      \expandafter\etb@ifr@prs
    \else
      \expandafter\expandafter
      \expandafter\etb@ifr@brk
    \fi
  \fi}

\def\etb@ifr@brk#1\relax{\@secondoftwo}

% <*>{<command>}{<separator>}

\newrobustcmd*{\DeclareListParser}{%
  \@ifstar
    {\etb@defparser\etb@defparser@arg}
    {\etb@defparser\etb@defparser@do}}

\def\etb@defparser#1#2#3{%
  \@ifdefinable#2{#1{#2}{#3}}}

\def\etb@defparser@do#1#2{%
  \begingroup
  \edef\@tempa{\endgroup
    \long\def\noexpand#1####1{%
      \expandafter\noexpand
      \csname etb@lst@\expandafter\@gobble\string#1\endcsname
      \space####1\noexpand#2&}%
    \long\csdef{etb@lst@\expandafter\@gobble\string#1}####1\noexpand#2####2&{%
      \noexpand\etb@listitem\noexpand\do{####1}%
      \noexpand\ifblank{####2}
        {\noexpand\listbreak}
        {\expandafter\noexpand
         \csname etb@lst@\expandafter\@gobble\string#1\endcsname
	 \space####2}&}}%
  \@tempa}

\def\etb@defparser@arg#1#2{%
  \begingroup
  \edef\@tempa{\endgroup
    \long\def\noexpand#1####1####2{%
      \expandafter\noexpand
      \csname etb@lst@\expandafter\@gobble\string#1\endcsname
      {####1}\space####2\noexpand#2&}%
    \long\csdef{etb@lst@\expandafter\@gobble\string#1}####1####2\noexpand#2####3&{%
      \noexpand\etb@listitem{####1}{####2}%
      \noexpand\ifblank{####3}
        {\noexpand\listbreak}
        {\expandafter\noexpand
         \csname etb@lst@\expandafter\@gobble\string#1\endcsname
	 {####1}\space####3}&}}%
  \@tempa}

\long\def\etb@listitem#1#2{%
  \ifblank{#2}
    {}
    {\expandafter\etb@listitem@i
     \expandafter{\@firstofone#2}{#1}}}
\long\def\etb@listitem@i#1#2{#2{#1}}

\newcommand*{\listbreak}{}
\long\def\listbreak#1&{}

% {<item1>,<item2>,...} => \do{<item1>}\do{<item2>}...

\DeclareListParser{\docsvlist}{,}

% {<handler>}{<item1>,<item2>,...} => <handler>{<item1>}<handler>{<item2>}...

\DeclareListParser*{\forcsvlist}{,}

% {<listmacro>}{<string>}

\newrobustcmd{\listadd}[2]{%
  \ifblank{#2}{}{\appto#1{#2|}}}
\newrobustcmd{\listeadd}[2]{%
  \begingroup
  \edef\etb@tempa{\endgroup\noexpand\ifblank{#2}}%
  \etb@tempa{}{\eappto#1{#2|}}}
\newrobustcmd{\listgadd}[2]{%
  \ifblank{#2}{}{\gappto#1{#2|}}}
\newrobustcmd{\listxadd}[2]{%
  \begingroup
  \edef\etb@tempa{\endgroup\noexpand\ifblank{#2}}%
  \etb@tempa{}{\xappto#1{#2|}}}

% {<listcsname>}{<string>}

\newrobustcmd{\listcsadd}[1]{%
  \expandafter\listadd\csname#1\endcsname}
\newrobustcmd{\listcseadd}[1]{%
  \expandafter\listeadd\csname#1\endcsname}
\newrobustcmd{\listcsgadd}[1]{%
  \expandafter\listgadd\csname#1\endcsname}
\newrobustcmd{\listcsxadd}[1]{%
  \expandafter\listxadd\csname#1\endcsname}

% {<string>}{<listmacro>}{<true>}{<false>}

\newrobustcmd{\ifinlist}[2]{%
  \begingroup
  \def\etb@tempa##1|#1|##2&{\endgroup
    \ifblank{##2}\@secondoftwo\@firstoftwo}%
  \expandafter\etb@tempa\expandafter|#2|#1|&}

\newrobustcmd{\xifinlist}[1]{%
  \begingroup
  \edef\etb@tempa{\endgroup\ifinlist{#1}}%
  \etb@tempa}

% {<string>}{<listcsname>}{<true>}{<false>}

\newrobustcmd{\ifinlistcs}[2]{%
  \expandafter\etb@ifinlistcs@i\csname #2\endcsname{#1}}
\long\def\etb@ifinlistcs@i#1#2{\ifinlist{#2}{#1}}

\newrobustcmd{\xifinlistcs}[1]{%
  \begingroup
  \edef\etb@tempa{\endgroup\ifinlistcs{#1}}%
  \etb@tempa}

% {<handler>}{<listmacro>} => <handler>{<item1>}<handler>{<item2>}...

\newcommand*{\forlistloop}[2]{%
  \expandafter\etb@forlistloop\expandafter{#2}{#1}}

\long\def\etb@forlistloop#1#2{\etb@forlistloop@i{#2}#1|&}

\long\def\etb@forlistloop@i#1#2|#3&{%
  \ifblank{#2}
    {}
    {#1{#2}}%
  \ifblank{#3}
    {\listbreak}
    {\etb@forlistloop@i{#1}#3}%
  &}

% {<handler>}{<listcsname>} => <handler>{<item1>}<handler>{<item2>}...

\newcommand*{\forlistcsloop}[2]{%
  \expandafter\expandafter\expandafter\etb@forlistloop
  \expandafter\expandafter\expandafter{\csname#2\endcsname}{#1}}

% {<listmacro>} => \do{<item1>}\do{<item2>}...

\newcommand*{\dolistloop}{\forlistloop\do}

% {<listcsname>} => \do{<item1>}\do{<item2>}...

\newcommand*{\dolistcsloop}{\forlistcsloop\do}

% {<code>}

\newrobustcmd*{\AtEndPreamble}{\gappto\@endpreamblehook}
\newcommand*{\@endpreamblehook}{}

\preto\document{%
  \endgroup
  \let\AtEndPreamble\@firstofone
  \@endpreamblehook
  \protected\def\AtEndPreamble{\@notprerr\@gobble}%
  \undef\@endpreamblehook
  \begingroup}

% {<code>}

\newrobustcmd*{\AfterPreamble}{\AtBeginDocument}
\AtEndPreamble{\let\AfterPreamble\@firstofone}

% {<code>}

\newrobustcmd*{\AfterEndPreamble}{\gappto\@afterendpreamblehook}
\newcommand*{\@afterendpreamblehook}{}

\appto\document{%
  \let\AfterEndPreamble\@firstofone
  \@afterendpreamblehook
  \protected\def\AfterEndPreamble{\@notprerr\@gobble}%
  \undef\@afterendpreamblehook
  \ignorespaces}

\AtEndDocument{\let\AfterEndPreamble\@gobble}

% {<code>}

\newrobustcmd*{\AfterEndDocument}{\gappto\@afterenddocumenthook}
\newcommand*{\@afterenddocumenthook}{}

\patchcmd\enddocument
  {\deadcycles}
  {\let\AfterEndDocument\@firstofone
   \@afterenddocumenthook
   \deadcycles}
  {}
  {\let\etb@@end\@@end
   \def\@@end{%
     \let\AfterEndDocument\@firstofone
     \@afterenddocumenthook
     \etb@@end}}

% {<environment>}{<code>}

\newrobustcmd{\AtBeginEnvironment}[1]{%
  \csgappto{@begin@#1@hook}}

\patchcmd\begin
  {\csname #1\endcsname}
  {\csuse{@begin@#1@hook}%
   \csname #1\endcsname}
  {}
  {\etb@warning{%
     Patching '\string\begin' failed!\MessageBreak
     '\string\AtBeginEnvironment' will not work\@gobble}}

% {<environment>}{<code>}

\newrobustcmd{\AtEndEnvironment}[1]{%
  \csgappto{@end@#1@hook}}

\patchcmd\end
  {\csname end#1\endcsname}
  {\csuse{@end@#1@hook}%
   \csname end#1\endcsname}
  {}
  {\etb@warning{%
     Patching '\string\end' failed!\MessageBreak
     '\string\AtEndEnvironment' will not work\@gobble}}

% {<environment>}{<code>}

\newrobustcmd{\BeforeBeginEnvironment}[1]{%
  \csgappto{@beforebegin@#1@hook}}

\pretocmd\begin
  {\csuse{@beforebegin@#1@hook}}
  {}
  {\etb@warning{%
     Patching '\string\begin' failed!\MessageBreak
     '\string\BeforeBeginEnvironment' will not work\@gobble}}

% {<environment>}{<code>}

\newrobustcmd{\AfterEndEnvironment}[1]{%
  \csgappto{@afterend@#1@hook}}

\patchcmd\end
  {\if@ignore}
  {\csuse{@afterend@#1@hook}%
   \if@ignore}
  {}
  {\etb@warning{%
     Patching '\string\end' failed!\MessageBreak
     '\string\AfterEndEnvironment' will not work\@gobble}}

\endinput

==> introduction.tex <==
\section{Introduction}
\label{sec:introduction}

With the extension satellites based positioning and navigation service, the GPS receiver encounters the problem of the signal acquisition in the challenging environments, such as indoor, on urban street and in woods with dense leaves~\cite{Tsui2001}. In these environments, the GPS signal becomes weak and can hardly be acquired by the receivers. To solve the problem, the studies on the weak GPS signal acquisition methods are widely performed. Generally, these GPS signal acquisition methods can be divided into two main categories. First, piling up GPS data is adopted to increase SNR~\cite{Psiaki01,Elders-Boll2004,Yu2007}. Second, mitigating the interference from the noise, the jamming signal and the unexpected GPS signals~\cite{Wang2011,Morton2007,Huang2011} is another approach to improving GPS signal acquisition performance; 

Coherent accumulation is a classical method of acquiring weak GPS signal acquisition. Even though the SNR increases with the extending accumulated GPS signal length, the coherently accumulated signal length does not goes beyond 10ms due to the data bit transition. To improve the SNR furthermore, Psiaki~\cite{Psiaki01} studied two non-coherent GPS signal accumulation methods, ‘full-bit’ and ‘half-bit’  GPS signal acquisition methods, which noncoherently pile up the GPS data to improve the GPS signal acquisition performance. In the condition that the carrier-to-noise (CNR) is larger than zero, the GPS signal noncoherent accumulation will generate the higher SNR. However, the accumulated GPS data duration can not be extended without limits. The noncoherent GPS signal accumulation will induce square loss; and the Doppler shift will also limit the accumulated GPS signal length extension. Thus, the GPS signal acquisition performance improvement by the noncoherent GPS signal accumulation is limited. At the direction of increasing SNR by piling up the GPS data, differential coherent accumulation method is also employed~\cite{Elders-Boll2004,Yu2007}. The differential coherent accumulation based acquisition method sums up the products of two adjacent coherent results. The GPS signal acquisition method increases the Doppler shift tolerance which is also insensitive to the data bit transition. Thus for differential coherent accumulation the constraint on the GPS signal data length extension is not so strict as the coherent accumulation which length is shorter than 10ms in usual cases. However, the shortage of the differential coherent accumulation is obvious that the SNR gain efficiency is not high enough compared with coherent accumulation method in the condition of the small Doppler shift.

Wang etc.~\cite{Wang2011} employed the noise subspace tracking algorithm to reduce the degradation from the interference which is a kind of spatial filtering method. The noise subspace tracking method depends on an antenna array to implement beam forming to mitigate the interference. Inevitably, the antenna array will increase the cost of the GPS receiver. Morton etc.~\cite{Morton2007} studied the GPS signal self-interference mitigation method by subspace projection. However, in the study of Morton, the non-orthogonality between the different GPS signal is neglected of, that is, the cross-correlation result between different pseudorandom codes is not exact zero. Huang and Pi~\cite{Huang2011} studied the interference between the different GPS signals which is called the near-far effect in GPS signal acquisition. Three different kinds of solutions to the near-far problem are proposed. Unfortunately, there is no one general method which can handle all the three kinds of the near-far problems. 

Huang etc.~\cite{Huang2009} proposed a GPS signal detection algorithm which employed Duffing chaotic oscillator to detect the weak GPS signals. The GPS signal detection algorithm utilizes the immunity to noise and sensitivity to the periodical signals. GPS signal has two periods possessed by the carrier and the pseudorandom code. Meanwhile, the noise is of no any periodicity in usual cases. The external periodical force from the periodic input signal will change the state of the chaotic oscillator by which the GPS signal is detected. However, there is a gap between the algorithm study and the hardware implementation since the chaotic oscillator based GPS signal acquisition method demands for the quite heavy computation burden. Also, Liu etc.~\cite{Liu2009} and Sahmoudi etc.~\cite{Sahmoudi2009} studied the degraded GPS signal tracking algorithm in the challenging environments with dense multipath and jamming signal. As we know, the tracking algorithm in the challenging environments makes sense only after the weak GPS signal is successfully acquired.

Indeed, the GPS signal possesses cyclostationary feature which enables the GPS receiver distinguish the expected GPS signal from the background noise and jamming signal. To the best knowledge of the author, few publications refers to utilizing the cyclostastionary feature to acquire the weak GPS signal.

In the 1950s, cyclostationary feature was proposed to characterize the statistics which is non-stationary but periodic. Since the 1980s Gardner W.A. has performed wide and deep research work on the cyclostatistics and the related applications~\cite{Gardner1975,Gardner1986,Gardner1988,Gardner1988a,Gardner1991,Gardner1992,Gardner1993}. Until now, there are huge amount of signal processing algorithms based on cyclostatistics in the various fields. However, as the author can refer, there is no publication on GPS signal detection based on the cyclostationary feature.
In this paper, the cyclostationary feature of the GPS signal is analyzed firstly; after that, the GPS signal detection method based on cyclostatistics is proposed and the detection performance is analyzed; also the initial pseudorandom code phase and the Doppler shift estimation methods are studied; in the end part of this article the simulations and experiments are carried out to test the effectiveness of the proposed GPS signal acquisition scheme.


\cite{So1994}



%Section~\ref{sec:principle_Weibull_chan_gen} discusses the CORDIC based Weibull fading channel generation method. 
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


==> numeric_simulation.tex <==
\section{Experiments and Simulations}
\label{sec:numeric_simulation}





%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{figure}[h]
\centering
\includegraphics[width=3.0in] {Fig/Sim_MSE_WL}
\setlength{\abovecaptionskip}{3pt plus 3pt minus 2pt}
\caption{MSE of the simulated fading channel versus the word length}
\label{fig: Sim MSE vs WL}
%\vspace{-0.15 in}
\end{figure}
%%%%%%%%%%%%%%%%%


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{figure}[h]
\centering
\includegraphics[width=3.0in] {Fig/Sim_MSE_T}
\setlength{\abovecaptionskip}{3pt plus 3pt minus 2pt}
\caption{MSE of the simulated fading channel versus the update period}
\label{fig: Sim MSE vs T}
%\vspace{-0.15 in}
\end{figure}
%%%%%%%%%%%%%%%%%


==> optimization_Ray_chan.tex <==
\section{Joint Optimization of Word Length and Update Rate}
\label{sec:joint optimization}

$x(t)$ denotes the unquantized real valued and time continuous Rayleigh channel. We use $\hat{x}_q(t)$ to represent quantized value and discrete time channel which features the channel generated on the emulator,
%%%%%%%%%%%%%%%%%%
\begin{equation}
x_q(t)=\sum_{n=-\infty}^{+\infty}x_q(nT)u(t-nT)
\label{eq: hat x_q def}
\end{equation}
%%%%%%%%%%%%%%%%%%
where $x_q(nT)$ denotes the Rayleigh channel data which is generated on the channel emulator at the \textit{n}-th time instance. $u(t)$ is the reconstruction function which converts the time discrete channel to the continuous one. As for the channel emulator, the value of the generated channel data keeps the same in the duration of $T$. Thus, $u(t)$ is a rectangular signal with the time duration of $T$ and the amplitude of unit one. 

Furthermore, $\epsilon(nT)$ is the quantization noise at \textit{n}-th, which is used to capture the effect of quantization error from the real value channel data to the discrete value one. Thus, the real valued data $x(nT)$ can be written as,
%%%%%%%%%%%%%%%%%%
\begin{equation}
x(nT)=x_q(nT)+\epsilon(nT).
\label{eq: x(nT) def1}
\end{equation}
%%%%%%%%%%%%%%%%%%

$\hat{x}(t)$ is used to represent continuous time channel which is reconstructed from the discrete time data $x(nT)$, $n=\cdots,1,2,3,\cdots$,
%%%%%%%%%%%%%%%%%%
\begin{equation}
\hat{x}(t)=\sum_{n=-\infty}^{+\infty}(x_q(nT)+\epsilon(nT))u(t-nT).
\label{eq: hat x(t) def1}
\end{equation}
%%%%%%%%%%%%%%%%%%

\subsection{Mean Square Error of the Generated Fading Channel}
\label{subsec: mse cal}

We define the mean square error between $x(t)$ and $\hat{x}_q(t)$ as
%%%%%%%%%%%%%%%%%%
\begin{equation}
\begin{aligned}
e^s&=E\left[\left(x(t)-\hat{x}_q(t)\right)^2\right]\\
&=E\left[\left(x(t)-\sum_{n=-\infty}^{+\infty}\left(x(nT)-\epsilon(nT)\right)u(t-nT)\right)^2\right]\\
&=E\left[\left(x(t)-\sum_{n=-\infty}^{+\infty}x(nT)u(t-nT)\right)^2\right]\\
&~~~+E\left[\left(\sum_{n=-\infty}^{+\infty}\epsilon(nT)u(t-nT)\right)^2\right]\\
&~~~+E\left[2\left(x(t)-\sum_{n=-\infty}^{+\infty}x(nT)u(t-nT)\right)\right.\\
&~~~~~~~~~\left.\cdot\left(\sum_{n=-\infty}^{+\infty}\epsilon(nT)u(t-nT)\right)\right]\\
\end{aligned}
\label{eq: mse def1}
\end{equation}
%%%%%%%%%%%%%%%%%%

Next, we will calculate the three items in (\ref{eq: mse def1}). 
%%%%%%%%%%%%%%%%%%%%%%%%
\begin{equation}
\begin{aligned}
&E\left[\left(x(t)-\sum_{n=-\infty}^{+\infty}x(nT)u(t-nT)\right)^2\right]\\
=&E\left[\left(x(t)-\hat{x}(t)\right)^2\right]\\
=&E\left[\left(x(t)-\hat{x}(t)\right)\left(x(t-\tau)-\hat{x}(t-\tau)\right)\right]|_{\tau=0}\\
=&R_x(\tau)+R_{\hat{x}}(\tau)-R_{\hat{x}x}(t,t-\tau)-R_{x\hat{x}}(t,t-\tau)|_{\tau=0}
\end{aligned}
\label{eq: 1st item in mse}
\end{equation}
%%%%%%%%%%%%%%%%%%%%%%%%

For the Rayleigh channel generation, the autocorrelation $R_x(\tau)$ is the first kind, order zero Bessel function,
%%%%%%%%%%%%%%%%%%%%%%%%
\begin{equation}
R_x(\tau)=J_0(2\pi f_D\tau).
\label{eq: Rx(tau)}
\end{equation}
%%%%%%%%%%%%%%%%%%%%%%%%

The autocorrelation function $R_{\hat{x}}(\tau)$ is 
%%%%%%%%%%%%%%%%%%%%%%%%
\begin{equation}
R_{\hat{x}}(\tau)=\frac{1}{T^2}\int S_x(f)|U(f)|^2 e^{j2\pi f\tau}df.
\label{eq: R_hatx(tau)}
\end{equation}
%%%%%%%%%%%%%%%%%%%%%%%%
where 
%%%%%%%%%%%%%%%%%%%%%%%%
\begin{equation}
S_x(f)=\frac{1}{\pi \sqrt{f^2_D-f^2}},~~ |f|\leq f_D.
\label{eq: Sx(f) cal1}
\end{equation}
%%%%%%%%%%%%%%%%%%%%%%%%

and the proof of (\ref{eq: R_hatx(tau)}) is given by (\ref{eq: R_hatx(tau) cal})
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{figure*}[!h]
% ensure that we have normalsize text
\normalsize
% Store the current equation number.
%\setcounter{MYtempeqncnt}{\value{equation}}
%\setcounter{equation}{5}
%%%%%%%%%%%%%%%%%%%%%%%%
\begin{equation}
\hrulefill
\begin{aligned}
R_{\hat{x}}(\tau)=&E\left[\hat{x}(t)\hat{x}(t-\tau)\right]\\
=&E\left[\sum_{n_1=-\infty}^{+\infty}x(n_1T)u(t-n_1T)\sum_{n_2=-\infty}^{+\infty}x(n_2T)u(t-\tau-n_2T)\right]\\
=&E\left[\sum_{n_1=-\infty}^{+\infty}\sum_{n_2=-\infty}^{+\infty}x(n_1T)x(n_2T)u(t-n_1T)u(t-\tau-n_2T)\right]\\
=&\sum_{n_1=-\infty}^{+\infty}\sum_{n_2=-\infty}^{+\infty}R_x((n_1-n_2)T)u(t-n_1T)u(t-\tau-n_2T)\\
=&\sum_{n_1=-\infty}^{+\infty}\sum_{n_2=-\infty}^{+\infty}\iiint S_x(f)U(f_1)U^*(f_2)e^{j2\pi(f-f_1)n_1T}e^{-j2\pi(f-f_2)n_2T}e^{j2\pi(f_1-f_2)t}e^{j2\pi f_2\tau}dfdf_1df_2\\
\overset{=}{(a)}&\frac{1}{T^2}\iiint S_x(f)U(f_1)U^*(f_2)\sum_{n_1=-\infty}^{+\infty}\delta(f-f_1-\frac{n_1}{T})\sum_{n_2=-\infty}^{+\infty}\delta(f-f_2+\frac{n_2}{T})e^{j2\pi(f_1-f_2)t}e^{j2\pi f_2\tau}dfdf_1df_2\\
=&\frac{1}{T^2}\int S_x(f)|U(f)|^2 e^{j2\pi f\tau}df\\
\end{aligned}
\label{eq: R_hatx(tau) cal}
\end{equation}
%%%%%%%%%%%%%%%%%%%%%%%%
where ($a$) follows the equation
%%%%%%%%%%%%%%%%%%%%
\begin{equation}
\sum_{n_1=-\infty}^{+\infty}e^{j2\pi(f-f_1)n_1T}=\frac{1}{T}\sum_{n_1=-\infty}^{+\infty}\delta(f-f_1-\frac{n_1}{T})
\label{eq: exp sum to sum delta}
\nonumber
\end{equation}
%%%%%%%%%%%%%%%%%%%%%%%%
% Restore the current equation number.
%\setcounter{equation}{\value{MYtempeqncnt}}
% IEEE uses as a separator
\hrulefill
% The spacer can be tweaked to stop underfull vboxes.
\vspace*{4pt}
\end{figure*}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

The cross-correlation function $R_{\hat{x}x}(\tau)$ is
%%%%%%%%%%%%%%%%%%%%%%%%
\begin{equation}
R_{\hat{x}x}(\tau)=\frac{1}{T}\int S_x(f)U(f) e^{j2\pi f\tau}df,
\label{eq: R_hatx x(tau)}
\end{equation}
%%%%%%%%%%%%%%%%%%%%%%%%
which proof is given by
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{figure*}[!h]
% ensure that we have normalsize text
\normalsize
% Store the current equation number.
%\setcounter{MYtempeqncnt}{\value{equation}}
%\setcounter{equation}{5}
%%%%%%%%%%%%%%%%%%%%%%%%
\begin{equation}
\hrulefill
\begin{aligned}
R_{\hat{x}x}(t,t-\tau)=&E\left[\hat{x}(t)x(t-\tau)\right]\\
=&E\left[x(t)\sum_{n=-\infty}^{+\infty}x(nT)u(t-\tau-nT)\right]\\
%=&E\left[\sum_{n_1=-\infty}^{+\infty}\sum_{n_2=-\infty}^{+\infty}x(n_1T)x(n_2T)u(t-n_1T)u(t-\tau-n_2T)\right]\\
=&\sum_{n=-\infty}^{+\infty}R_x(t-nT)u(t-\tau-nT)\\
=&\sum_{n=-\infty}^{+\infty}\iint S_x(f)U(f_1)e^{-j2\pi(f-f_1)nT}e^{j2\pi(f-f_1)t}e^{j2\pi f_1\tau}dfdf_1\\
=&\frac{1}{T}\iint S_x(f)U(f_1)\sum_{n=-\infty}^{+\infty}\delta(f-f_1+\frac{n}{T})e^{j2\pi(f-f_1)t}e^{j2\pi f_1\tau}dfdf_1\\
=&\frac{1}{T}\int S_x(f)U(f) e^{j2\pi f\tau}df\\
\end{aligned}
\label{eq: R_hatx x(tau) cal}
\end{equation}

% Restore the current equation number.
%\setcounter{equation}{\value{MYtempeqncnt}}
% IEEE uses as a separator
\hrulefill
% The spacer can be tweaked to stop underfull vboxes.
\vspace*{4pt}
\end{figure*}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


Similarly, we give can calculate the cross-correlation function $R_{x\hat{x}}(\tau)$ by
%%%%%%%%%%%%%%%%%%%%%%%%
\begin{equation}
R_{x\hat{x}}(\tau)=\frac{1}{T}\int S_x(f)U^*(f) e^{j2\pi f\tau}df.
\label{eq: R_x hatx(tau)}
\end{equation}
%%%%%%%%%%%%%%%%%%%%%%%%

Therefore, the item of $E\left[\left(x(t)-\sum_{n=-\infty}^{+\infty}x(nT)u(t-nT)\right)^2\right]$ is determined by
 %%%%%%%%%%%%%%%%%%%%%%%%
\begin{equation}
\begin{aligned}
&E\left[\left(x(t)-\sum_{n=-\infty}^{+\infty}x(nT)u(t-nT)\right)^2\right]\\
=&\int_{-f_D}^{f_D}S_x(f)(1-2\Re\{U(f)\}+|U(f)|^2) df\\
%=&\int_{-f_D}^{f_D}S_x(f)(1-2\Re\left\{\frac{\sin(\pi fT)}{\pi fT}\right\}+|\frac{\sin(\pi fT)}{\pi fT}|^2|_{\tau=0}
\end{aligned}
\label{eq: mse 1st item cal result}
\end{equation}
%%%%%%%%%%%%%%%%%%%%%%%%

Because we assume that the Nyquist sampling requirement is satisfied, $\frac{1}{T}\geq 4f_D$, $U(f)=\frac{\sin(\pi fT)}{\pi fT}\geq 0$. The equation (\ref{eq: mse 1st item cal result}) is rewritten as
 %%%%%%%%%%%%%%%%%%%%%%%%
\begin{equation}
\begin{aligned}
&E\left[\left(x(t)-\sum_{n=-\infty}^{+\infty}x(nT)u(t-nT)\right)^2\right]\\
=&\int_{-f_D}^{f_D}S_x(f)\left(1-\frac{\sin(\pi fT)}{\pi f}\right)^2 df
\end{aligned}
\label{eq: mse 1st item cal result2}
\end{equation}
%%%%%%%%%%%%%%%%%%%%%%%%

Next, we calculate $E\left[\left(\sum_{n=-\infty}^{+\infty}\epsilon(nT)u(t-nT)\right)^2\right]$. Using the same derivation of calculating $R_{\hat{x}}(\tau)$ in (\ref{eq: R_hatx(tau) cal}), we obtain 
%%%%%%%%%%%%%%%%%%%%%%%%
\begin{equation}
\begin{aligned}
E\left[\left(\sum_{n=-\infty}^{+\infty}\epsilon(nT)u(t-nT)\right)^2\right]=\frac{1}{T^2}\int S_{\epsilon}(f)|U(f)|^2df,\\
\end{aligned}
\label{eq: mse 2st item cal result1}
\end{equation}
%%%%%%%%%%%%%%%%%%%%%%%%
where $S_{\epsilon}(f)$ is the spectrum of the quantization noise $\epsilon$.

The channel data generation on FPGA is the process of the quantization into the uniform $2^P$ levels. Therefore, the quantization noise $\epsilon$ uniformly distributes in $[\frac{-1}{2\times2^P},\frac{1}{2\times2^P}]$ and is independent to quantized data $x_q$. The variance of $x_q$ is $\frac{1}{12}\frac{1}{4^P}$. Thus, (\ref{eq: mse 2st item cal result1}) is rewritten as
%%%%%%%%%%%%%%%%%%%%%%%%
\begin{equation}
\begin{aligned}
E\left[\left(\sum_{n=-\infty}^{+\infty}\epsilon(nT)u(t-nT)\right)^2\right]=\int \frac{1}{12}\frac{1}{4^P}\left|\frac{\sin(\pi fT)}{\pi fT}\right|^2df,\\
\end{aligned}
\label{eq: mse 2st item cal result2}
\end{equation}
%%%%%%%%%%%%%%%%%%%%%%%%

Next, we calculate the third item of (\ref{eq: mse def1}),
%%%%%%%%%%%%%%%%%%
\begin{equation}
\begin{aligned}
&E\left[\left(x(t)-\sum_{n=-\infty}^{+\infty}x(nT)u(t-nT)\right)\right.\\
&~~~~~~\left.\cdot\left(\sum_{n=-\infty}^{+\infty}\epsilon(nT)u(t-nT)\right)\right]\\
=&E\left[\left(x(t)\sum_{n=-\infty}^{+\infty}\epsilon(nT)u(t-nT)\right)\right]\\
~-&E\left[\sum_{n=-\infty}^{+\infty}x(nT)u(t-nT)\sum_{n=-\infty}^{+\infty}\epsilon(nT)u(t-nT)\right]\\
=&E\left[\sum_{n=-\infty}^{+\infty}\epsilon^2(nT)u(t-nT)\right]\\
&-E\left[\left(\sum_{n=-\infty}^{+\infty}\epsilon(nT)u(t-nT)\right)^2\right]\\
=&\int \frac{1}{12}\frac{1}{4^P}\frac{\sin(\pi fT)}{\pi fT}df-\int \frac{1}{12}\frac{1}{4^P}\left|\frac{\sin(\pi fT)}{\pi fT}\right|^2df
\end{aligned}
\label{eq: mse 3rd item cal result1}
\end{equation}
%%%%%%%%%%%%%%%%%%

Based the calculation above, the mean square error between $x(t)$ and $\hat{x}_q(t)$ is 
%%%%%%%%%%%%%%%%%%
\begin{equation}
\begin{aligned}
e^s=&\int_{-f_D}^{f_D}S_x(f)\left(1-\frac{\sin(\pi fT)}{\pi f}\right)^2 df\\
+&2\int \frac{1}{12}\frac{1}{4^P}\frac{\sin(\pi fT)}{\pi fT}df-\int \frac{1}{12}\frac{1}{4^P}\left|\frac{\sin(\pi fT)}{\pi fT}\right|^2df\\
\overset{(a)}{=}&\int_{-f_D}^{f_D}S_x(f)\left(1-\frac{\sin(\pi fT)}{\pi fT}\right)^2 df+\frac{1}{12}\frac{1}{4^P}\\
\end{aligned}
\label{eq: mse result 1}
\end{equation}
%%%%%%%%%%%%%%%%%%
where ($a$) follows the facts that $\int \frac{\sin(\pi fT)}{\pi fT}df=1$ and $\int \left|\frac{\sin(\pi fT)}{\pi fT}\right|^2df=1$.

Afterwards, we will optimize the MSE $e^s$ at the constraint of the hardware resources in terms of bits per second~($\frac{P}{T}$). More specifically, we assume the hardware resource of bits per second is fixed~($\frac{P}{T}=C$ and $C$ is a constant), which indicates the computation burden for generating the fading channel. With this budget of hardware resources, we improve the fidelity of the generated channel $\hat{x}(t)$ by minimizing its mean square error $e^s$. This optimization problem is formulated by 
%%%%%%%%%%%%%%%%%%
\begin{equation}
\begin{aligned}
\text{minimize:}&~~e^s(P,~T) \\
\text{subject to}&~~\frac{P}{T}\leq C.
\end{aligned}
\label{eq: opt eq 1}
\end{equation}
%%%%%%%%%%%%%%%%%%

Based on (\ref{eq: opt eq 1}), we have the Lagrange function 
%%%%%%%%%%%%%%%%%%
\begin{equation}
\begin{aligned}
g(P,~T)=e^s(P,~T)+\lambda(\frac{P}{T}-C).
\end{aligned}
\label{eq: opt Lagrange eq}
\end{equation}
%%%%%%%%%%%%%%%%%%
where $\lambda$ is a Lagrange multiplier.

To calculate the optimized $P$ and $T$ achieving the minimum $e^s$, we calculate the zero valued partial derivatives,
%%%%%%%%%%%%%%%%%%
\begin{equation}
\left\{\begin{aligned}
&\frac{\partial g(P,~T)}{\partial P}=0 \\
&\frac{\partial g(P,~T)}{\partial T}=0
\end{aligned}
.\right.
\label{eq: opt partial derivative 1}
\end{equation}
%%%%%%%%%%%%%%%%%%

Combining (\ref{eq: opt partial derivative 1}) and the constraint $\frac{P}{T}=C$, we have
%%%%%%%%%%%%%%%%%%
\begin{equation}
\left\{\begin{aligned}
&\frac{\lambda}{T}-\frac{4^{-P}\ln4}{12}=0 \\
&\frac{\lambda P}{T^2}+\int_{-f_D}^{f_D}\left(\begin{aligned}S_x(f)\left(1-\frac{\sin\pi fT}{\pi fT}\right)\\
\times\left(\frac{\pi fT\cos\pi fT-\sin\pi fT}{\pi fT^2}\right) \end{aligned}\right)df=0\\
&\frac{P}{T}\leq C
\end{aligned}
.\right.
\label{eq: 1st derivative}
\end{equation}
%%%%%%%%%%%%%%%%%%

Let $T^*$ and $P^*$ denote the values of the channel update period and the bit width which generate the zero valued first order partial derivative of $g(\cdot)$. With $T^*$ and $P^*$, we calculate the Heissen matrix of $g(\cdot)$ which is given by
%%%%%%%%%%%%%%%%%%
\begin{equation}
J=\left.\begin{bmatrix}
\frac{\partial^2g}{\partial P^2} & \frac{\partial^2g}{\partial P\partial T}\\
\frac{\partial^2g}{\partial T\partial P} & \frac{\partial^2g}{\partial T^2}
\end{bmatrix}
\right|_{T=T^*,P=P^*}
\label{eq: Heissen matrix}
\end{equation}
%%%%%%%%%%%%%%%%%%
where the entries of $J$ are determined by
%%%%%%%%%%%%%%%%%%
\begin{equation}
\left\{\begin{aligned}
&\frac{\partial^2g}{\partial P^2}=\frac{4^{-P}\ln4}{12};~\frac{\partial^2g}{\partial P\partial T}=\frac{\partial^2g}{\partial T\partial P}=\frac{-\lambda}{T^2}\\
&\frac{\partial^2g}{\partial T^2}=\frac{2\lambda P}{T^3}-\int_{-f_D}^{f_D}S_x(f)\left(\frac{\pi fT-\pi^2 f^2T^2\sin\pi fT-2\pi fT\cos\pi fT+2\sin\pi fT}{\pi fT^3}\right)df\\
%&=\frac{-\lambda}{T^2}\\
\end{aligned}
.\right.
\label{eq: 2nd derivative}
\end{equation}
%%%%%%%%%%%%%%%%%%


Because the clock frequency of FPGA is much higher than the maximum Doppler in the fading channel, the update rate $T$ is approximately considered as a real number. Thus, we can determine the optimum $T$ by calculating the derivatives of the continuous variables over $T$. Let $T^*$ denote the optimum $T$. However, for any given hardware platforms, including the FPGA, the numbers of the bits used for channel generation are positive integers. Therefore, the derivative calculation for the continuous variable, as shown in (\ref{eq: opt partial derivative 1}), is not fitting the calculation of the optimum word length $P$. 

To solve the problem caused by the mixture of continuous and discrete valued variables, the numerical methods are used. 

\subsection{Numerical Solution to the Optimum $T$ and $P$}
\label{subsec: num solu to T* P*}

Before the numerical investigation on the optimum update period $T$ and the bit width $P$, we need to determine the value ranges of them. According to the Nyquist sampling theorem, the update period $T$ is required to be not larger than the inverse of two times maximum Doppler, $T\leq\frac{1}{2f_D}$. And, the lower bound of $T$ is limited by the clock period of the FPGA chips. Based on the simulation results in (\ref{Huang2013}), the bit width $P$ should be no less than $8$, otherwise, the MSE of the generated channel is larger than XXX. Considering the real case of FPGA chips, the maximum value of $P$ is set as $24$. If the larger value of $P$ is selected, the FPGA will XXXXXX. Therefore, we have the range of $T$ and $P$ which are $\frac{1}{f_0}<T\leq\frac{1}{2f_D}$ and $8\leq P\leq 24$.


At each value of $P$ in $[8,~24]$, we calculate the update period $T$ which makes the first order derivative of $g(\cdot)$ versus $T$ equal to zero. One example of the first order derivative is plotted in Fig.~\ref{fig: 1st derivative}. The red star markers indicates the points at which $\frac{\partial g}{\partial T}=0$. 

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{figure}[h]
\centering
\includegraphics[width=2.0in] {Fig/FirstDerivative}
\setlength{\abovecaptionskip}{3pt plus 3pt minus 2pt}
\caption{First order derivative of $g(\cdot)$ over T for a given word length $P$}
\label{fig: 1st derivative}
%\vspace{-0.15 in}
\end{figure}
%%%%%%%%%%%%%%%%%

Let $\mathcal{T}_P^*$ denote the set of the $T$'s inducing $\frac{\partial g}{\partial T}=0$ at the bit width of $P$, $\mathcal{T}_P^*=\{T^*_{Pi}\}$, $i\in\mathbb{N}$ and $1\leq i\leq |\mathcal{T}_P^*|$, where $\left.\frac{\partial g}{\partial T}\right|_{T^*_{Pi},P}=0$. We use $\beta_P$ to represent Cartesian product between $\mathcal{T}_P^*$ and $P$. Therefore, the entry of $\beta_P$ is $(T^*_{Pi}, P)$.

We calculate the determinant of the Heissen matrix at all entries $\beta_P$. Part of the determinant calculation results are illustrated in Fig.~\ref{fig: det of Heissen matrix}. From Fig.~\ref{fig: det of Heissen matrix}, the determinants of Heissen matrix are all positive. Therefore, the entries of $\beta_P$ are all the locally minimum points. 

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{figure}[h]
\centering
\includegraphics[width=3.0in] {Fig/Det_vs_Tstar}
\setlength{\abovecaptionskip}{3pt plus 3pt minus 2pt}
\caption{Determinant of the Heissen matrix at the fixed points}
\label{fig: det of Heissen matrix}
%\vspace{-0.15 in}
\end{figure}
%%%%%%%%%%%%%%%%%

With the locally minimum points set $\beta_P$, we calculate the mean square error $e_s$ and the bit rate via (\ref{eq: mse result 1}) and $\frac{P}{T^*_{Pi}}$ respectively. Let $\mathcal{E}_{P}$ and $\mathcal{R}_{P}$ denote the set of the calculated MSE and the bit rate at $P$ respectively.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{figure}[h]
\centering
\includegraphics[width=3.0in] {Fig/MSE_vs_R}
\setlength{\abovecaptionskip}{3pt plus 3pt minus 2pt}
\caption{Minimum MSE under the constraint of the bit rate}
\label{fig: MSE vs R}
%\vspace{-0.15 in}
\end{figure}
%%%%%%%%%%%%%%%%%

In Fig.~\ref{fig: MSE vs R}, the \enquote*{MSE-R} curves for the different $P$'s are plotted. Each \enquote*{MSE-R} curve in Fig.~\ref{fig: MSE vs R} monotonically decrease and is convex. A single \enquote*{MSE-R} curve provides us the information of the optimum update period $T$ locally at $P$. To determine the optimum combination of $T$ and $P$, we plot the convex hull of the \enquote*{MSE-R} curves for all $P$'s. The dot dash curve in Fig.~\ref{fig: MSE vs R} is the convex hull. 

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{figure}[h]
\centering
\includegraphics[width=3.0in] {Fig/opt_wl_T_vs_resource}
\setlength{\abovecaptionskip}{3pt plus 3pt minus 2pt}
\caption{The optimum word length and the channel update rate}
\label{fig: opt WL and T}
%\vspace{-0.15 in}
\end{figure}
%%%%%%%%%%%%%%%%%

The convex hull in Fig.~\ref{fig: MSE vs R} indicates the minimum MSE for a given a bit rate. From each point on the convex hull, We trace back to the $T^*$ and $P^*$ which generate the convex hull. These combinations of $T^*$ and $P^*$ are the optimum update period and the bit width. In Fig.~\ref{fig: opt WL and T}, the optimum update period $T^*$ and the bit width $P^*$ are plotted. 

From Fig.~\ref{fig: opt WL and T} both the $T^*$ curve and the $P^*$ one are not continuous. This is because the bit width $P$ are natural number which is discrete valued. 




==> sec_cyc_feature.tex <==
\section{Cyclostationary Feature and Cyclic Spectrum of GPS Signal Equations}
\label{sec: cyclic feature}

The GPS signal is represented by $s(t)$. The $s(t)$ is the time period of 1\textit{ms} is given by 
%%%%%%%%%%%%%%%%%%
\begin{equation}
s(t)=\sum_{k=0}^{1022}c(k)q(t-kT_c-t_0)\cos(2\pi f_0t+\theta_0).
\label{eq: def of s(t)}
\end{equation}
%%%%%%%%%%%%%%%%%%
where $T_c$ denotes the time duration of one pseudorandom code chip. $q(t)$ is the square wave with duration, $q(t)=1$ for $0\leq t\leq T_c$, otherwise, $q(t)=0$. $t_0$ is the initial pseudorandom code phase. $f_0$ is the signal carrier frequency. $\theta_0$ is the initial phase of the carrier.

%where denotes the time duration of one pseudorandom code chip,  is the square wave with duration

\subsection{Cyclostationary feature of GPS signal}
\label{subsec: cyclic feature of GPS}

To investigate the cyclostationary feature of GPS signal, we calculate the mean and the variance of $s(t)$

In one period of C/A code, due to ergodic feature, the mean value of $s(t)$ is approximately calculated by
%%%%%%%%%%%%%%%%%%
\begin{equation}
\begin{aligned}
M_{s}&=\int_0^{T_0}s(t)dt\\
&=\int_0^{T_0}\sum_{k=0}^{1022}c(k)q(t-kT_c-t_0)\cos(2\pi f_0t+\theta_0)dt\\
&\approx 0,
\end{aligned}
\label{eq: mean of s(t)}
\end{equation}
%%%%%%%%%%%%%%%%%%
where $T_0$ denotes the period of C/A code.



==> sec_stability.tex <==
\section{Stability of the Iteration Structure}
\label{set: stability analysis}
The sum-of-sinusoid (SS) scheme is considered in our fading channel generator. In the SS method, multiple sinusoids are generated first which are then piled up to generate the Gaussian distributed random process. We generate two orthogonal Gaussian process which are denoted by $I$ and $Q$. The envelope of $I$ and $Q$ is Rayleigh distributed.

In the novel method, our contribution is that we propose the order two iterative structure to generate the sinusoids.With this iterative structure, the novel channel generator is given by
%%%%%%%%%%%%%%%%%%%%%%%
\begin{equation}
\left\{
\begin{aligned}
x[n]&=\frac{1}{L}\sqrt{\left(\sum_{l=0}^{L-1}I_l[n]\right)^2+\left(\sum_{l=0}^{L-1}Q_l[n]\right)^2}\\
I_l[n]&=2\cos\omega_lI_l[n-1]-I_l[n-2]\\
Q_l[n]&=2\cos\omega_lQ_l[n-1]-Q_l[n-2]
\end{aligned}
\right.
\label{eq: iter. chan. gen.}
\end{equation}
%%%%%%%%%%%%%%%%%%%%%%%%%%
where $l\in\{1, 2, · · · ,L\}$ and $I_l$ and $Q_l$ denote the \textit{l}-th
sinusoid used to generate the In-phase and the Quadrature
Gaussian process.

The expression of $I_l$ in the frequency domain is written as
%%%%%%%%%%%%%%%%%%%%%%%
\begin{equation}
\ddot{Y}-2B\dot{Y}+Y=0,
\label{eq: order 2 different eq}
\end{equation}
%%%%%%%%%%%%%%%%%%%%%%%%%%
where $B = \cos\omega_l$.

The eigen equation of the order two differential equation
(\ref{eq: order 2 different eq}) is given by
%%%%%%%%%%%%%%%%%%%%%%%
\begin{equation}
\lambda^2-2B\lambda+1=1.
\label{eq: eigen eq}
\end{equation}
%%%%%%%%%%%%%%%%%%%%%%%%%%

The solutions to (\ref{eq: eigen eq}) is presented by
%%%%%%%%%%%%%%%%%%%%%%%
\begin{equation}
\lambda=B\pm j\sqrt{1-B^2}.
\label{eq: solution to diff eq}
\end{equation}
%%%%%%%%%%%%%%%%%%%%%%%%%%


Based on (\ref{eq: solution to diff eq}), the absolute value of $\lambda$ is
%%%%%%%%%%%%%%%%%%%%%%%
\begin{equation}
|\lambda|=1,
\label{eq: abs of solu}
\end{equation}
%%%%%%%%%%%%%%%%%%%%%%%%%%
and the angle of the root is given by
%%%%%%%%%%%%%%%%%%%%%%%
\begin{equation}
\omega_l=\angle\lambda=\arctan\frac{\sqrt{1-B^2}}{B}.
\label{eq: angle of solu}
\end{equation}
%%%%%%%%%%%%%%%%%%%%%%%%%%

However, due to the finite number of bits, there exists the error in quantizing the constant $B$. Let $\Delta b$ denote the quantization error for $B$ and $B^*$ represents the quantized $B$,
%%%%%%%%%%%%%%%%%%%%%%%
\begin{equation}
B^*=B+\Delta b.
\label{eq: B * def}
\end{equation}
%%%%%%%%%%%%%%%%%%%%%%%%

According to~\cite{}, the quantization error $\Delta b$ is uniformly distributed in the range of $[-\frac{1}{2^{P+1}}, \frac{1}{2^{P+1}}]$ where $P$ is the bit width in the quantization. 



For fairness, we consider the largest quantization error for a given bit width $P$, that is,
%%%%%%%%%%%%%%%%%%%%%%%
\begin{equation}
\Delta b=\frac{1}{2^p}.
\label{eq: largest Delta b}
\end{equation}
%%%%%%%%%%%%%%%%%%%%%%%%


Take the \textit{P}-bits quantization for example. The maximum of $ω_l$, $l\in\{1, 2, · · · ,L\}$, is represented by \enquote*{$\overbrace{11 · · · 1}$}. In that case $B^* = B$, thus, $\Delta b = 0$. Therefore, the value of $B^*$ locates in the range of $[0, 1]$.

We substitue $B^*$ into (\ref{eq: eigen eq}) and obtain the solution which is given by
%%%%%%%%%%%%%%%%%%%%%%%
\begin{equation}
\lambda^*=B+\Delta b\pm j\sqrt{1-(B+\Delta b)^2}.
\label{eq: B * def}
\end{equation}
%%%%%%%%%%%%%%%%%%%%%%%%

The amplitude and angle of $λ^*$ are calculated by
%%%%%%%%%%%%%%%%%%%%%%%
\begin{align}
|\lambda^*|&=1\\
\omega_l^*&=\omega_l+\Delta\omega=\arctan\frac{\sqrt{1-(B+\Delta b)^2}}{B+\Delta b},
\label{eq: abs and angle of B*}
\end{align}
%%%%%%%%%%%%%%%%%%%%%%%%%
where $\Delta \omega$ denote the frequency bias in the sinusoid generation.

For the convenience of analysis, we first consider the positive $\Delta b$. In this case, it can be easily shown that $\frac{\sqrt{1-(B+\Delta b)^2}}{B+\Delta b}<\frac{\sqrt{1-B^2}}{B}$ which means $\Delta\omega<0$. Similarly, $\Delta\omega>0$, when $\Delta b<0$.


From (\ref{eq: abs and angle of B*}), the amplitude is immune to the quantization error which means the amplitude of the generated sinusoid stays on the unit one. The quantization error affects the frequency of the generated sinusoid.


The Taylor expansion of $\tan(ω_l+\Delta\omega)$ at the point $ω_l$ is given by
%%%%%%%%%%%%%%%%%%%%%%%
\begin{equation}
\tan(\omega_l+\Delta\omega)=\tan(\omega_l)+\frac{1}{\cos^2\omega_l}\Delta\omega-\frac{2\sin\omega_l}{\cos^3\omega_l}(\Delta\omega)^2+\mathcal{O}((\Delta\omega)^3).
\label{eq: Taylor expan of tan}
\end{equation}
%%%%%%%%%%%%%%%%%%%%%%%%

Because $\Delta b ≪ |ω_l|$ we can easily find that the derivative of $\tan(\theta^*)$ over the quantization error $\Delta b$ is negative. The difference between $\tan\theta^*$ and $\tan\theta$ is written as
%%%%%%%%%%%%%%%%%%%%%%%
\begin{equation}
\begin{aligned}
e_1&=\tan\theta^*-\tan\theta\\
&=\sqrt{\frac{\sin^2\omega_l-2\cos\omega_l\Delta b-(\Delta b)^2}{\cos^2\omega_l+2\cos\omega_l\Delta b+(\Delta b)^2}}-\tan\omega_l.
\end{aligned}
\label{eq: tan theta *-tan theta}
\end{equation}
%%%%%%%%%%%%%%%%%%%%%%%%

Combining (\ref{eq: Taylor expan of tan}) and (\ref{eq: tan theta *-tan theta}), we have
%%%%%%%%%%%%%%%%%%%%%%%
\begin{equation}
C_1(\Delta\omega)^2+C_2\Delta\omega+C_3=0,
\label{eq: quadratic eq}
\end{equation}
%%%%%%%%%%%%%%%%%%%%%%%%
where
%%%%%%%%%%%%%%%%%%%%%%%
\begin{equation}
\begin{array}{c}
C_1\triangleq-\frac{2\sin\omega_l}{\cos^3\omega_l},C_2\triangleq\frac{1}{\cos^2\omega_l}\\
C_3\triangleq\sqrt{\frac{\sin^2\omega_l-2\cos\omega_l\Delta b-(\Delta b)^2}{\cos^2\omega_l+2\cos\omega_l\Delta b+(\Delta b)^2}}-\tan\omega_l
\end{array}
\label{eq: C1 C2 C3}
\end{equation}
%%%%%%%%%%%%%%%%%%%%%%%%

By solving (\ref{eq: quadratic eq}), we can obtain the connection between $\Delta\omega$ and $\Delta b$. Furthermore, it is easily seen that the larger
$\Delta b$ induces the larger $\Delta\omega$. Therefore, the roots of (\ref{eq: quadratic eq}) are calculated which are given by
%%%%%%%%%%%%%%%%%%%%%%%
\begin{equation}
\Delta\omega=\left\{\begin{array}{lcr}
\frac{-C_2-\sqrt{C_2^2-4C_1C_3}}{2C_1}&\mbox{for} & \Delta b>0\\
\frac{-C_2+\sqrt{C_2^2-4C_1C_3}}{2C_1}&\mbox{for} & \Delta b\leq 0
\end{array}\right..
\label{eq: solu to Delta omega}
\end{equation}
%%%%%%%%%%%%%%%%%%%%%%%%



Therefore, the frequency shift caused by the quantization error is determined by (\ref{eq: solu to Delta omega}). Indeed, the frequency shift in the channel generation is not necessary to be removed. According to the results in~\cite{Xiao2006}, the perturbation on the designed frequency component is helpful to improve the independence of the generated channels.



Even though the uniformly distributed quantization error does not change the statistical features of the generated fading channel~\cite{Xiao2006}, the frequency overlapping or intersection for the different sinusoid components needs to be precluded. 

We can easily see that the larger number of sinusoids induces the smaller frequency gap between two sinusoids which are adjacent in frequency domain. If the number of sinusoid L is larger, the more bits are needed to quantize the channel data. Next, we investigate the relationship between $L$ and $P$.


The closest frequency gap exists between the 1 and $cos(\frac{\pi}{2L})$. The second closet frequency gap is between $cos(\frac{\pi}{2L})$ and $cos(\frac{\pi}{L})$. The two frequency gaps need to be larger than the frequency bias $\Delta\omega$. According to this requirement, we have the two inequalities as follows,
%%%%%%%%%%%%%%%%%%%%%%%
\begin{equation}
\left\{
\begin{aligned}
\frac{-C_2-\sqrt{C_2^2-4C_1C_3(\Delta b^+)}}{2C_1}\leq2\pi\left(1-\cos\frac{\pi}{2L}\right)\\
\frac{-C_2+\sqrt{C_2^2-4C_1C_3(\Delta b^-)}}{2C_1}\geq2\pi\left(\cos\frac{\pi}{L}-\cos\frac{\pi}{2L}\right)
\end{aligned}
\right.,
\label{eq: seperaty of freq}
\end{equation}
%%%%%%%%%%%%%%%%%%%%%%%%
where $C_3(\Delta b^+)$ and $C_3(\Delta b^-)$ denote the values of $C_3$ when $\Delta b$ is positive and negative respectively. 

We can easily prove that the left parts of the two inequalities in (\ref{eq: seperaty of freq}) are both the monotonic functions of $\Delta b$. When $\Delta b=\frac{1}{2^{P+1}}$, $C_3(\Delta b^+)$ reaches the maximum value. $C_3(\Delta b^-)$ achieves the minimum at $\Delta b=\frac{-1}{2^{P+1}}$. Therefore, (\ref{eq: seperaty of freq}) is transformed into the equation as follows,
%%%%%%%%%%%%%%%%%%%%%%%
\begin{equation}
\left\{
\begin{aligned}
&\frac{C_2(\frac{\pi}{2L})-\sqrt{C_2^2(\frac{\pi}{2L})-4C_1(\frac{\pi}{2L})\left(\sqrt{\frac{\sin^2\frac{\pi}{2L}-2\cos\frac{\pi}{2L}\frac{1}{2^{P+1}}-(\frac{1}{2^{P+1}})^2}{\cos^2\frac{\pi}{2L}+2\cos\frac{\pi}{2L}\frac{1}{2^{P+1}}+(\frac{1}{2^{P+1}})^2}}-\tan\frac{\pi}{2L}\right)}}{4\pi C_1(\frac{\pi}{2L})}\leq2\pi\left(1-\cos\frac{\pi}{2L}\right)\\
&\frac{C_2(\frac{\pi}{2L})+\sqrt{C_2^2(\frac{\pi}{2L})-4C_1(\frac{\pi}{2L})\left(\sqrt{\frac{\sin^2\frac{\pi}{2L}+2\cos\frac{\pi}{2L}l\frac{1}{2^{P+1}}-(\frac{1}{2^{P+1}})^2}{\cos^2\frac{\pi}{2L}-2\cos\frac{\pi}{2L}\frac{1}{2^{P+1}}+(\frac{1}{2^{P+1}})^2}}-\tan\frac{\pi}{2L}\right)}}{4\pi C_1(\frac{\pi}{2L})}\geq2\pi\left(\cos\frac{\pi}{L}-\cos\frac{\pi}{2L}\right)
\end{aligned}
\right.,
\label{eq: seperaty of freq2}
\end{equation}
%%%%%%%%%%%%%%%%%%%%%%%%
where $C_1(\frac{\pi}{2L})$ $C_2(\frac{\pi}{2L})$ denote the values of $C_1$ and $C_2$ at $\omega_l=\frac{\pi}{2L}$.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{figure}[h]
\centering
\includegraphics[width=3.0in] {Fig/DeltaOmega_vs_Omega}
\setlength{\abovecaptionskip}{3pt plus 3pt minus 2pt}
\caption{Frequency bias caused by the limited word length at the different sinusoid components}
\label{fig:Delta Omega vs omega}
%\vspace{-0.15 in}
\end{figure}
%%%%%%%%%%%%%%%%%

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{figure}[h]
\centering
\includegraphics[width=3.0in] {Fig/DeltaOmega_vs_WL}
\setlength{\abovecaptionskip}{3pt plus 3pt minus 2pt}
\caption{Frequency bias at the different limited word lengths}
\label{fig:Delta Omega vs WL}
%\vspace{-0.15 in}
\end{figure}
%%%%%%%%%%%%%%%%

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{figure}[h]
\centering
\includegraphics[width=3.0in] {Fig/up_bound_of_paths}
\setlength{\abovecaptionskip}{3pt plus 3pt minus 2pt}
\caption{Upper bound on the number of the sinusoid components in the constraint by frequency bias}
\label{fig: up bound of sins}
%\vspace{-0.15 in}
\end{figure}
%%%%%%%%%%%%%%%%%

\begin{comment}
For the given number of the sinusoids L, the smallest frequency gap between two sinusoids is
%%%%%%%%%%%%%%%%%%%%%%%
\begin{equation}
\Delta\omega_m=2\pi\left(1-\cos\frac{\pi}{2L}\right).
\label{eq: largest Delta omega}
\end{equation}
%%%%%%%%%%%%%%%%%%%%%%%%

To avoid the frequency overlapping, we need to set $\Delta\omega\leq \frac{1}{2}\Delta\omega_m$, that is
%%%%%%%%%%%%%%%%%%%%%%%
\begin{equation}
\Delta\omega\leq2\pi\left(1-\cos\frac{\pi}{2L}\right).
\label{eq: upper bound of Delta omega}
\end{equation}
%%%%%%%%%%%%%%%%%%%%%%%%

$\Delta\omega$ is a function of $\Delta b$ as shown in (\ref{eq: solu to Delta omega}). We substitute $\Delta b =\frac{1}{2^{N+1}}$ into $\Delta\omega(\Delta b)$.

Combining (\ref{eq: solu to Delta omega}), (\ref{eq: largest Delta b}) and (\ref{eq: largest Delta omega}), we obtain the connection between $L$ and $P$ which is given by
%%%%%%%%%%%%%%%%%%%%%%%
\begin{equation}
L\leq\frac{\pi}{2}\frac{1}{\arccos\left(1+\frac{C_2-\sqrt{C_2^2-4C_1\left(\sqrt{\frac{\sin^2\omega_l-2\cos\omega_l\frac{1}{2^P}-(\frac{1}{2^P})^2}{\cos^2\omega_l+2\cos\omega_l\frac{1}{2^P}+(\frac{1}{2^P})^2}}-\tan\omega_l\right)}}{4\pi C_1}\right)}
\label{eq: L leq func of P}
\end{equation}
%%%%%%%%%%%%%%%%%%%%%%%%
\end{comment}
